Topics in Supergravity Phenomenology

In the first part of the review article, we discuss the possibility of realizing "mu-split-like SUSY" scenario from a phenomenological model, which we show could be realizable locally as the large volume limit of a type IIB Swiss-Cheese Calabi-Yau orientifold involving a mobile space-time filling D3-brane localized at a nearly special Lagrangian three-cycle embedded in the "big" divisor and multiple fluxed stacks of space-time filling D7-branes wrapping the same "big" divisor. We show that the mass of one of the Higgs doublets can be produced to be of the order of 125 GeV whereas other Higgs as well as higgsino mass parameter to be very heavy- the "mu-split-like SUSY" scenario. Then we discuss the role of the heavy squarks/sleptons and the light Higgs in (i) obtaining long-lived gluinos (ii) in verifying that the NLSPs (squarks/sleptons/neutralino) decay into the LSP (gravitino) respects the BBN constraints with the lifetime of the LSP (gravitino) coming out to be of the order or larger than the age of the universe, (iii) getting gravitino relic abundance of around 0.1, and (iv) obtaining electronic EDM close to the experimental upper bounds. In second part of the review article, we obtain local M-theory uplift of Type IIB background involving non-compact (resolved) warped deformed conifold and (N) space time filling D3-branes placed on the singularity of the conifold, (M) D5-branes wrapped around compact 2-sphere, and (N_f) D7-branes wrapped around non-compact four-cycle via Strominger-Yau-Zaslow's mirror symmetry prescription and show the stability of the solution so obtained. We propose a new MQGP limit corresponding to finite-string-coupling (g_s~ 1)- large-t'Hooft-coupling regime of M-theory. Interestingly, we obtain eta/s=1/4 pi for the uplift and the diffusion constant D~1/T for types IIB/IIA backgrounds in the both limits.

==> Chapter2/chapter2-back_up.tex <==
%Satyam Shivam Sundaram
%Jai Mata Di
\chapter{Phenomenological Model: Realization of $\mu$-split SUSY Scenario}
\vskip -0.5in
{\hskip1.4in{\it ``Do there exist many worlds, or is there but a single world? This is one of the most noble and exalted questions in the study of Nature."}}

\hskip3.0in - Albertus Magnus, c. 13th Century.

\graphicspath{{Chapter2/}{Chapter2/}}
\vskip -0.5in
\section{Introduction}
Over the past few years, producing realistic models satisfying both cosmological as well as phenomenological requirements from string compactifications, has proven to be a daunting challenge. To get the phenomenological implications of BSM models, they must implicate a particular SUSY breaking mechanism and hence scale of SUSY breaking. The recently proposed split SUSY model (based on high SUSY breaking scale) inspired by the need of fine-tuning the cosmological constant, is emerging to be quite interesting from the point of view of phenomenology because of the fact that heavy scalars mostly appearing as virtual particles in most of the particle decay studies, help to resolve many diverse issue of both particle physics and cosmology \cite{HamidSplitSUSY}. Therefore, it is quite interesting to realize split SUSY scenario within the string-theoretic framework. One of the interesting string compactification schemes, which eventually gives a metastable dS minima naturally, was presented in \cite{dSetal} by considering Type IIB compactified on the orientifold of a Swiss-Cheese Calabi-Yau in the LVS limit that includes non-(perturbative) corrections and non-perturbative instanton-corrections in superpotential. Further, the possibility of generating light fermion masses as well as heavy sfermion masses by including a space-time filling mobile $D3$-brane and stack(s) of (fluxed) $D7$-branes wrapping the ``Big" divisor in the aforementioned framework \cite{ferm_masses_MS}, has interestingly pointed towards the likelihood of split SUSY-like scenario in large volume Type IIB model. Motivated by this, we extend the model to include two-Wilson line moduli\cite{Dhuria+Misra_mu_Split_SUSY}, followed by a systematic four-Wilson line moduli model\cite{gravitino_DM}, and explicitly show a possible local realization of $\mu$-split SUSY-like scenario in the large volume limit by including D3/D7-branes.

Before elaborating upon the discussion of $\mu$-split SUSY realization, in section {\bf 2}, we first provide details of a phenomenological model which could possibly be realized in a string-theoretic framework by considering, locally, the Swiss-Cheese Calabi-Yau type IIB string compactification in the large volume limit with a mobile space-time filling D3-brane restricted to a nearly special Lagrangian three-cycle in the Calabi-Yau and fluxed stacks of wrapped D7-branes. Then we summarize the construction of  four harmonic distribution one-forms localized along the mobile space-time filling $D3$-brane (restricted to the three-cycle). By calculating the intersection matrix valued in the Wilson line moduli sub-space $a_{I=1,...,h^{(0,1)}_-(\Sigma_B)}$, appearing in K\"{a}hler coordinate $T_B$, we write (the K\"{a}hler sector of the) K\"{a}hler potential that includes  four-Wilson line moduli $a_1, a_2, a_3, a_4$ and two-position moduli of a mobile space-time filling $D3$-brane restricted to the above-mentioned (nearly) SLag (corresponding to a local minimum). The estimate of the Dirac mass terms appearing in the ${\cal N}=1$ supergravity action of \cite{Wess_Bagger} calculated from superpotential and K\"{a}hler potential suggest that the fermionic superpartners of ${\cal A}_1$ and ${\cal A}_3$ correspond respectively to  the first generation leptons: $e_L$ and $e_R$, and the fermionic superpartners of ${\cal A}_2$ and ${\cal A}_4$ correspond respectively to the first generation quarks: $u_L$ and $u_R$.  We use this identification throughout  to discuss all phenomenological issues such as evaluation of soft SUSY breaking parameters as well as estimates of various three-point vertices in the context of gauged ${\cal N}=1$ supergravity action. Next, due to multiple D7-branes, we provide explicit bi-fundamental representations for the four-Wilson line moduli and two $D3$-brane position moduli (after having turned on appropriate two-form fluxes on the $D7$-brane world volume decomposing adjoint-valued matter fields into bi-fundamental matter fields) and speculate about the possible modification in the relevant ${\cal N}=1$ chiral coordinate in the presence of the same. It is also shown that the (effective) physical Yukawas change only by ${\cal O}(1)$ under an RG-flow from the string scale down to the EW scale. The discussion of phenomenological results  governing signatures of $\mu$-split SUSY in this framework are  appended in sections {\bf 3}-{\bf 5}.  Section {\bf 3} has details of calculations of various soft SUSY breaking parameters.  In section {\bf 4}, we describe the fact that it is possible to obtain $125\ GeV$ mass for one of the Higgs doublets at EW scale. Section {\bf 5} discuss evaluation of neutralino/chargino mass matrix. In section {\bf 6}, we present a detailed study of gluino decay life time at tree-level as well as at one-loop level in the context of ${\cal N}=1$ gauged SUGRA.  Finally we
summarize the chapter in section {\bf 7}.
 \vskip -0.5in
\section{The Model}
 Let us first briefly describe our model for which we present evidence that
it could be locally realized as a large volume $D3/D7$ Swiss-Cheese setup in
 \cite{gravitino_DM}. For an ${\cal N}=1$ compactification, we will take the phenomenological K\"{a}hler potential of our model to be:
\begin{eqnarray}
\label{K_pheno}
& & \hskip -0.5in K_{\rm Pheno} = - ln\left[-i(\tau-{\bar\tau})\right]
-ln\left(-i\int_{CY_3}\Omega\wedge{\bar\Omega}\right)\nonumber\\
& & \hskip -0.5in - 2\ ln\Biggl[a_B(\sigma_B + {\bar\sigma}_B - \gamma K_{\rm geom})^{\frac{3}{2}} - (\sum_{i}a_{S,i}(\sigma_{S,i} + {\bar\sigma}_{S,i} - \gamma K_{\rm geom}))^{\frac{3}{2}} + {\cal O}(1) {\cal V}\Biggr],
 \end{eqnarray}
where the divisor volumes $\sigma_\alpha$ are expressible in terms of ``K\"{a}hler" coordinates $T_\alpha, {\cal M}_{\cal I}$
\begin{eqnarray}
\label{sigma}
& & \sigma_\alpha\sim T_\alpha -\left[ i{\cal K}_{\alpha bc}c^b{\cal B}^c
+ i C^{{\cal M}_{\cal I}{\bar{\cal M}}_{\bar {\cal J}}}_\alpha({\cal V})Tr\left({\cal M}_{\cal I}{\cal M}^\dagger_{\bar {\cal J}}\right)\right],
\end{eqnarray}
$\alpha=\left(B,\{S,i\}\right)$ and ${\cal M}_{\cal I}$ being
  $SU(3_c)\times SU(2)_L$  bifundamental  matter field $a_{{\cal I}=2}$, $SU(3_c)\times U(1)_R$ bifundamental matter field
$a_{{\cal I}=4}$, $SU(2)_L\times U(1)_L$ bifundamental matter field $a_{{\cal I}=1}$,
$U(1)_L\times U(1)_R$ bifundamental matter field $a_{{\cal I}=3}$ along with
$SU(2)_L\times U(1)_L$ bifundamental $\tilde{z}_{1,2}$
 with the intersection matrix:
$ C^{a_I{\bar a}_{\bar J}}_\alpha\sim \delta^B_\alpha C^{I{\bar J}}_\alpha, C^{a_I\bar {\tilde{z}}_{\bar j}}_\alpha=0$, $\rho_{S,B}, {\cal G}^a = c^a - \tau b^a$ being complex axionic
fields ($\alpha,a$ running over the real dimensionality of a sub-space of the internal manifold's cohomology complex),  and the phenomenological  superpotential is given as under:
\begin{equation}
\label{W_pheno}
 W_{\rm Pheno}\sim\left(z_1^{18} + z_2^{18}\right)^{n^s}
e^{-n^s vol(\Sigma_S) - (\alpha_S z_1^2 + \beta_S z_2^2 + \gamma_S z_1z_2)},
\end{equation}
\noindent where the bi-fundamental $\tilde{z}_i$ in $K$ will be equivalent to the $z_{1,2}\in\mathbb C$ in $W$. It is
expected that ${\cal M}_{\cal I}, T_{S,B}, {\cal G}^a$ will constitute the ${\cal N}=1$ chiral coordinates. The
 intersection matrix elements $\kappa_{S/B ab}$ and the volume-dependent $C^{{\cal M}_{\cal I}{\bar{\cal M}}_{\bar {\cal  J}}}_\alpha({\cal V})$, are chosen in such a way that at a local (meta-stable) minimum:
 \begin{eqnarray}
 \label{extremum_i}
& &  \langle \sigma_S\rangle \sim \langle (T_S + {\bar T}_S)\rangle  - i C^{\tilde{z}_i\bar {\tilde{z}}_{\bar j}}({\cal V}) Tr\left(\langle\tilde{z}_i\rangle \langle \bar {\tilde{z}}_{\bar j}\rangle\right)\sim {\cal O}(1)
\nonumber\\
& &  \langle \sigma_B\rangle \sim \langle (T_B + {\bar T}_B)\rangle  - i C^{\tilde{z}_i\bar {\tilde{z}}_{\bar j}}({\cal V}) Tr\left(\langle\tilde{z}_i\rangle \langle\bar {\tilde{z}}_{\bar j}\rangle\right)
- i C^{a_I{\bar a}_{\bar J}}({\cal V}) Tr\left(\langle a_I\rangle \langle{\bar a}_{\bar J}\rangle\right)\sim e^{f \langle \sigma_S\rangle},\nonumber\\
& &
 \end{eqnarray}
 where $f$ is a fraction not too small as compared to 1, and the stabilized values of $T_\alpha$ around the meta-stable local minimum:
 \begin{equation}
 \label{extremum_ii}
 \langle\Re e T_S\rangle,\langle\Re e T_B\rangle\sim {\cal O}(1).
 \end{equation}
 In the context of ${\cal N}=1$ type IIB orientifolds, in (\ref{extremum_i}), $\alpha,a$ index respectively involutively even, odd sectors of $h^{1,1}(CY_3)$ under a holomorphic, isometric involution.
If the volume ${\cal V}$ of the internal manifold is large in string length units, one sees that one obtains a hierarchy between the stabilized values $\langle\Re e\tau_{S,B}\rangle$ but not $\langle\Re e T_{S,B}\rangle$.

We now argue how to realize (\ref{K_pheno}) - (\ref{extremum_ii}), locally, in string theory.
Consider type IIB compactified on the orientifold of a Swiss-Cheese Calabi-Yau
in the LVS limit that includes non-(perturbative) $\alpha^{\prime}$ corrections
 and non-perturbative instanton-corrections in superpotential. For phenomenological purposes, we will consider a space-time filling $D3$-brane
and multiple fluxed stacks of space-time filling $D7$-branes wrapping a single
four-cycle, the big divisor, with different choice of small
two-form fluxes turned on the different two-cycles homologously non-trivial from the point of view of this four-cycle's
Homology (for the purpose of decomposing initially adjoint-valued matter fields
to bi-fundamental matter fields, for generating the SM gauge groups and
to effect gauge-coupling unification at the string scale). Then  $z_{1,2}$ get identified with the $D3$-brane's position moduli,
$\tau$ is the axion-dilaton modulus and ${\cal G}^a$ are NS-NS and RR two-form axions complexified by the axion-dilaton modulus.
% In the orientifold-limit of F-theory, one considers an
%orientifold of the Calabi-Yau involving a holomorphic isometric involution.

From Sen's orientifold-limit-of-F-theory point of view  corresponding to type IIB compactified on a Calabi-Yau three fold $Z$-orientifold with $O3/O7$ planes, one requires an elliptically fibered Calabi-Yau four-fold $X_4$ (with projection $\pi$) over a 3-fold $B_3(\equiv CY_3-$orientifold)  where $B_3$ can be taken to be  an $n$-twisted ${\mathbb {CP}}^1$-fibration over ${\mathbb {CP}}^2$ such that pull-back of the divisors in $CY_3$ automatically satisfy Witten's unit-arithmetic genus condition \cite{DDF}.  For $n=6$ \cite{DDF}, the Calabi-Yau three-fold $Z$ then turns out to be a unique Swiss-Cheese Calabi Yau  in ${ \mathbb{WCP}}^4_{[1,1,1,6,9]}[x_1:x_2:x_3:x_4:x_5]$ given by a smooth degree-18 hypersurface in ${ \mathbb{WCP}}^4[1,1,1,6,9]$; the exceptional divisor corresponding to resolution of a ${\mathbb  Z}_3$-singularity $x_1=x_2=x_3=0$, via the monomial-divisor map, is encoded as the $\phi x_1^6x_2^6x_3^6 (\phi$ being an involutively odd complex structure modulus) polynomial deformation in the defining hypersurface. Henceforth, we will be working in the non-singular coordinate patch $x_2=1$ in the large volume limit of the Swiss-Cheese Calabi-Yau.

The closed string moduli-dependent K\"{a}hler potential, includes perturbative (using \cite{BBHL}) and non-perturbative (using \cite{Grimm}) $\alpha^\prime$-corrections. Written out in (discrete subgroup of) $SL(2,{\bf Z})$(expected to survive orientifolding)-covariant form, the perturbative corrections are proportional to $\chi(CY_3)$ and non-perturbative $\alpha^\prime$ corrections are weighted by $\{n^0_\beta\}$, the genus-zero Gopakumar-Vafa invariants that count the number of genus-zero rational curves $\beta\in H_2^-(CY_3,{\bf Z})$. In fact, the closed string moduli-dependent contributions are dominated by the genus-zero Gopakumar-Vafa invariants which using Castelnuovo's theory of moduli spaces can be shown to be extremely large for compact projective varieties \cite{Klemm_GV} such as the one used.

Based on the study initiated in \cite{ferm_masses_MS,Dhuria+Misra_mu_Split_SUSY}, one of us (AM), inspired by the Donaldson's algorithm - see \cite{Donaldson_i} -  had obtained in \cite{review-iii}, an estimate of a nearly Ricci-flat Swiss Cheese metric for points finitely separated from $\Sigma_B$ based on the ansatz as given in \cite{gravitino_DM}. Using this ansatz, one sees that $h^{11}\sim h^{z_4^2{\bar z}_4^2}{\cal V}^{\frac{2}{3}}$.
%For consistency, we should therefore obtain $h^{z_4^2{\bar z}_4^2}\sim {\cal V}^{-\frac{1}{3}}$. This has been assumed in (\ref{eq:K}) and will be verified below to correspond to one allowed value of $h^{z_4^2{\bar z}_4^2}$ that would yield an approximately Ricci-flat metric (up to within 10$\%$).
Using (\ref{eq:K}), one can show that:
\begin{equation}
\label{eq:R11bar_i}
R_{z_i{\bar z}_j}\sim\frac{\sum_{n=0}^8a_n\left(h^{z_4^2{\bar z}_4^2}\right)^n {\cal V}^{\frac{n}{3}}}{\left(1+{\cal O}(1)h^{z_4^2{\bar z}_4^2} {\cal V}^{\frac{1}{3}}\right)^2{\cal V}^{\frac{1}{18}}\left(\sum_{n=0}^3b_n\left(h^{z_4^2{\bar z}_4^2}\right)^n {\cal V}^{\frac{n}{3}}\right)^2}.
\end{equation}
Solving numerically: $\sum_{n=0}^8a_n\left(h^{z_4^2{\bar z}_4^2}\right)^n {\cal V}^{\frac{n}{3}}=0$, as was assumed, one (of the eight values of) $h^{z_4^2{\bar z}_4^2}$, up to a trivial K\"{a}hler transformation, turns out to be ${\cal V}^{-\frac{1}{3}}, {\cal V}\sim 10^6$. Curiously, from GLSM-based analysis, we had seen in \cite{D3_D7_Misra_Shukla} that on $\Sigma_B(z_4=0)$, the argument of the logarithm received the most dominant contribution from the FI-parameter $r_2\sim{\cal V}^{\frac{1}{3}}$ which using this value of $h^{z_4^2{\bar z}_4^2}$, is in fact, precisely what one obtains even now. Using this value of $h^{z_4^2{\bar z}_4^2}$, one obtains: $R_{z_i{\bar z}_4},R_{z_4{\bar z}_4}\sim10^{-1}$. Further, as has been assumed that the metric components $g_{z_{1,2}{\bar z}_4}$ are negligible as compared to $g_{z_i{\bar z}_j}$ - this was used in \cite{ferm_masses_MS} in showing the completeness of the basis spanning $H^{1,1}_-$ for a large volume holomorphic isometric involution restricted to (\ref{eq:near_slag_i}),
 $z_1\rightarrow-z_1,z_{2,3}\rightarrow z_{2,3}$, which is now born out explicitly, wherein the latter turn out to about 10$\%$ of the former. One does not need the aforementioned restriction on the geometric Swiss-Cheese metric for large volume involutions restricted to (\ref{eq:near_slag_i}), of the following type. In the $x_2\neq0$-coordinate patch, the defining degree-18 hypersurface in ${\mathbb {WCP}}^4_{1,1,1,6,9}[x_1:x_2:x_3:x_4:x_5]$ can be written as: $1 + z_1^{18} + z_2^{18} + z_3^3 - \psi z_1z_2z_3z_4 - \phi z_1^6z_2^6 = 0, z_1=\frac{x_1}{x_2}, z_2=\frac{x_3}{x_2}, z_3=\frac{x_4}{x_1^6}, z_4=\frac{x_5}{x_1^9}$. The same can be rewritten as: $\left(i z_4\right)^2 - \psi z_1z_2z_3z_4 =  z_3^3 + \phi z_1^6z_2^6 - z_1^{18} - z_2^{18}$. This is can therefore be thought of as the following Weierstrass variety:
 $\begin{array}{rrc}T^2(z_3,z_4(z_3)) & \rightarrow&{\mathbb {WCP}}^4_{1,1,1,6,9}(z_1,z_2,z_3)\\
 & & \downarrow\pi \\
 & & {\mathbb CP}^2(z_1,z_2)\\
  \end{array}$. Now, assuming that the complex structure modulus $\psi$ has been stabilized to an infinitesimal value so that one can disregard the polynomial deformation proportional to $\psi$, and defining $\chi_{1,2}\equiv z_{1,2}^6$, this elliptic fibration structure can thought also of as:
  $\begin{array}{rrc}T^2(z_3,z_4(z_3)) & \rightarrow&{\mathbb {WCP}}^4_{1,1,1,6,9}(\chi_1,\chi_2,z_3)\\
 & & \downarrow\pi \\
 \left({\rm Complex\ curve}\right){\cal C}(\chi_1)&\longrightarrow & {\mathbb {CP}}^2(\chi_1,\chi_2)\\
 & & \downarrow\pi^\prime\\
 & & {\mathbb {CP}}^1(\chi_2)
  \end{array}$, corresponding to $\left(i z_4\right)^2\approx z_3^3 + \phi \chi_1\chi_2 - \chi_1^3 - \chi_2^3$. Alternatively, one can also think of the Weierstrass variety as:
  $\begin{array}{rrc}T^2(-\chi_1,z_4(-\chi_1)) & \rightarrow&{\mathbb {WCP}}^4_{1,1,1,6,9}(\chi_1,\chi_2,z_3)\\
 & & \downarrow\pi \\
 \left({\rm Complex\ curve}\right){\cal C}(-z_3)&\longrightarrow & {\mathbb {CP}}^2(-z_3,\chi_2)\\
 & & \downarrow\pi^\prime\\
 & & {\mathbb {CP}}^1(\chi_2)
  \end{array}$, corresponding to $\left(i z_4\right)^2\approx\left(-\chi_1\right)^3 + \phi \chi_1\chi_2 + z_3^3 - \chi_2^3$. Therefore, near (\ref{eq:near_slag_i}), one can define a large volume holomorphic involution: $\chi_1\leftrightarrow-z_3, \phi\rightarrow-\phi$(the fact that complex structure modulus $\phi$ is involutively odd, is also used in (\ref{eq:sigmas_Ts})). We will assume that in the coordinate patch
(but not globally):
$|z_1|\equiv {\cal V}^{\frac{1}{36}},\ |z_2|\equiv{\cal V}^{\frac{1}{36}},\ |z_3|\equiv{\cal V}^{\frac{1}{6}}$, the Calabi-Yau is diffeomorphic to the Swiss-Cheese $\mathbb {{WCP}}^4_{1,1,1,6,9}[18]$. The
defining hypersurface for the same is: $x_1^{18}+x_2^{18}+x_3^{18}+x_4^3+x_5^2
-18\psi\prod_{i=1}^5x_i-3\phi (x_1x_2x_3)^6=0$. This can be thought of as the following
hypersurface in an ambient complex four-fold: $P(x_1,...,x_5;\xi)=0$ after resolution
of the $\mathbb Z_3$-singularity\cite{Rummel_et_al} [the $x_4$ and $x_5$ have been switched
relative to \cite{DDF}; $n=6$ $\mathbb {CP}^1$-fibration over $\mathbb{CP}^2$ with
projective coordinates $x_{1,2,3},x_4,x_5$ of \cite{DDF} is equivalent to $n=-6$ with projective coordinates
$x_{1,2,3,},x_5,x_4$ - see \cite{Denef_Les_Houches}] with the toric data for the same given by:
$$\begin{array}{c|cccccc}
& x_1 & x_2 & x_3 & x_4 & x_5 & \xi \\ \hline
Q^1 & 1 & 1 & 1 & 6 & 0 & 9 \\
Q^2 & 0 & 0 & 0 & 1 & 1 & 2 \\
\end{array}.$$
In the coordinate patch: $x_2\neq0$(implying one is away
from the $\mathbb Z_3$-singular $(0,0,0,x_4,x_5)$ in
$\mathbb{WCP}^4_{1,1,1,6,9}[18]$), $\xi\neq0$, one sees that the following are
the gauge-invariant coordinates: $z_1=\frac{x_1}{x_2}, z_2=\frac{x_3}{x_2},
z_3=\frac{x_4^2}{x_2^3\xi}, z_4=\frac{x_5^2x_2^9}{\xi}.$
We henceforth assume
the Calabi-Yau hypersurface to be written in this coordinate patch as:
$z_1^{18} + z_2^{18} + {\cal P}(z_{1,2,3,4};\psi,\phi)=0$.
The divisor $\left\{x_5=0\right\}\cap\left\{P(x_{1,2,3,4,5};\xi)=0\right\}$
is rigid with $h^{0,0}=1$  (See \cite{Rummel_et_al})  satisfying the Witten's
unit-arithmetic genus condition, and that the Calabi-Yau volume can
be written as
${\rm vol}(CY_3)=\frac{\tau_4^{\frac{3}{2}}}{18} -
\frac{\sqrt{2}\tau_5^{\frac{3}{2}}}{9},$  implying that the `small divisor'
$\Sigma_s$ is $\left\{x_5=0\right\}\cap\left\{z_1^{18} + z_2^{18} + {\cal P}(z_{1,2,3},z_4=0;\psi,\phi)=0\right\}$
and the big divisor $\Sigma_B$ is  $\left\{x_4=0\right\}\cap\left\{z_1^{18} + z_2^{18} + {\cal P}(z_{1,2,4},z_3=0;\psi,\phi)=0\right\}.$ Alternatively, using
the toric data of \cite{candelas_et_al_11169}:
$$\begin{array}{c|cccccc}
& x_1 & x_2 & x_3 & x_4 & x_5 & \xi \\ \hline
Q^1 & 1 & 1 & 1 & 0 & 0 & -3 \\
Q^2 & 0 & 0 & 0 & -2 & -3 & -1 \\
\end{array},$$ one can verify that
$\left\{\xi=0\right\}\cap\left\{P^\prime(x_{1,2,3,4,5};\xi)=0
\right\}$ is the rigid blow-up mode with $h^{0,0}=1$ (which can be easily
verified using cohomCalg\footnote{We thank P.Shukla for verifying the same.})
and one can define gauge-invariant coordinates in the $x_2\neq0,x_4\neq0$
coordinate-patch: $z_1=\frac{x_1}{x_2}, z_2=\frac{x_3}{x_2},
z_3=\frac{(x_5x_1)^2}{x_4^3}, z_4=\frac{(x_6x_1^3)^2}{x_4}.$ \\
Interestingly, around the  three-cycle
\begin{equation}
\label{eq:near_slag_i}
C_3:|z_1|\sim {\cal V}^{\frac{1}{36}},\ |z_2|\sim{\cal V}^{\frac{1}{36}},\ |z_3|\sim{\cal V}^{\frac{1}{6}},
\end{equation}
the Calabi-Yau can be thought of,
locally, as a complex three-fold ${\cal M}_3$ which is a $T^3$(swept out by ($arg z_1$,$arg z_2$, $arg z_3$)-fibration over a large base $(|z_1|,|z_2|,|z_3|)$; precisely apt for application of mirror symmetry as three T-dualities a la S(trominger) Y(au) Z(aslow)), $C_3$ is almost a s(pecial) Lag(rangian) sub-manifold because it satisfies the requirement that  $f^*J\approx0,\ \Re e\left(f^*e^{i\theta}\Omega\right)\biggr|_{\theta=\frac{\pi}{2}}\approx {\rm vol}(C_3),\ \Im m\left(f^* e^{i\theta}\Omega\right)\biggr|_{\theta=\frac{\pi}{2}}\approx0$ where $f:C_3\rightarrow CY_3$). Let us see if these requirements hold up. Using the geometric K\"{a}hler potential  as given in \cite{gravitino_DM}, the geometric metric near $C_3$ is estimated to be:
\begin{equation}
\label{eq:geom met}
g_{i{\bar j}}\sim\frac{{\cal O}(10^{-1})}{2}\left(
\begin{array}{lll}
 \frac{1}{ \sqrt[18]{V}} & \frac{1}{ \sqrt[18]{V}} & \frac{1}{ V^{7/36}} \\
 \frac{1}{ \sqrt[18]{V}} & \frac{1}{ \sqrt[18]{V}} & \frac{1}{ V^{7/36}} \\
 \frac{1}{ V^{7/36}} & \frac{1}{ V^{7/36}} & \frac{1}{ \sqrt[3]{V}}
\end{array}
\right),
\end{equation}
The same was necessary in
explicitly demonstrating $h^{1,1}_-\neq0$ in \cite{ferm_masses_MS} for the large volume involution: $z_1\rightarrow -z_1, z_{2,3}\rightarrow z_{2,3}$. \\
$(i)$ Using (\ref{eq:geom met}), one sees that:
\begin{eqnarray}
\label{eq:J_pull back}
& & f^*(ds_6^2)\sim0.05\left[\sum_{i,j=1}^2{\cal V}^{-\frac{1}{18}}\left(dz_id{\bar z}_{\bar j}\right)+{\cal V}^{-\frac{1}{3}}|dz_3|^2\right]\Biggr|_{C_3}\nonumber\\
& & \sim 0.05\left[\sum_{i,j=1}^2d (arg z_i)d (arg{\bar z}_{\bar j}) + d (arg z_3) d (arg {\bar z}_3)\right].
\end{eqnarray}
This implies $f^*J\sim0.05$, which is small.\\
$(ii)$ In the $x_2\neq0$- coordinate patch with $z_1=\frac{x_1}{x_2}, z_2=\frac{x_3}{x_2}, z_3=\frac{x_4}{x_2^6}, z_4=\frac{x_5}{x_2^6}$, by the Griffiths residue formula, one obtains: $\Omega=\frac{dz_1\wedge dz_2\wedge dz_4}{\frac{\partial P}{\partial z_3}}=\frac{dz_1\wedge dz_2\wedge dz_4}{3z_3^2-\psi z_1z_2z_4}$. The coordinate $z_4$ can be solved for using:
\begin{equation}
\label{eq:x4_i}
z_4=\frac{\psi z_1z_2z_3\pm\sqrt{\psi^2(z_1z_2z_3)^2-4(1+z_1^{18}+z_2^{18}+z_3^3-\phi (z_1z_2)^6)}}{2}\sim \psi {\cal V}^{\frac{2}{9}}\pm i{\cal V}^{\frac{1}{4}},
\end{equation}
which implies that the $T^3$ will never degenerate as the roots will never coincide:
\begin{eqnarray}
\label{eq:x4_ii}
& & dz_4\sim dz_3\left(\frac{\psi z_1z_2}{2} \pm\frac{\left(2\psi^2z_1^2z_2^2z_3 - 12 z_3^2\right)}{4\sqrt{\psi^2(z_1z_2z_3)^2-4(1+z_1^{18}+z_2^{18}+z_3^3-\phi (z_1z_2)^6)}}\right) \nonumber\\
&& \hskip 0.35in+ (...)dz_1 + (...)dz_2 \nonumber\\
&& \hskip 0.2in  \sim\left(\frac{\psi z_1z_2}{2} \pm
  1.5i\frac{z_3^2}{\sqrt{z_1^{18}+z_2^{18}+z_3^3}}\right)dz_3 +
(...)dz_1 + (...)dz_2, \nonumber\\
&&  \hskip 0.35in {\rm near}\ (\ref{eq:near_slag_i}),
|\psi|<<1,|\phi|<<1.
\end{eqnarray}
 Therefore, restricted to (\ref{eq:near_slag_i}) and substituting (\ref{eq:x4_i}) and (\ref{eq:x4_ii}) in the aforementioned expression of $\Omega$, one obtains:
\begin{eqnarray}
\label{eq:Omega}
& & \Omega\sim\frac{\left(\psi {\cal V}^{\frac{1}{18}}\pm 1.5i{\cal V}^{\frac{1}{12}}\right)}{3{\cal V}^{\frac{1}{3}}-\psi {\cal V}^{\frac{1}{18}}\left[\psi {\cal V}^{\frac{2}{9}}\pm i{\cal V}^{\frac{1}{4}}\right]}dz_1\wedge dz_2\wedge dz_3 \sim  \left(\frac{\psi{\cal V}^{-\frac{5}{18}}}{3}\pm 0.5i {\cal
    V}^{-\frac{1}{4}}\right)
dz_1\wedge dz_2\wedge dz_3.\nonumber\\
\end{eqnarray}
Hence, if one could estimate  the pull-back of the nowhere vanishing
holomorphic three-form as:
\begin{eqnarray}
\label{eq:f*Omega}
& & f^*\Omega\sim\left(\frac{\psi}{3}{\cal
    V}^{-\frac{5}{18}+\frac{1}{18}+\frac{1}{6}}+
0.5i{\cal V}^{-\frac{1}{4}+\frac{1}{18}+\frac{1}{6}}\right)d(arg
z_1)\wedge d(arg z_2)\wedge d(arg z_3)\Biggr|_{{\cal V}\sim10^6}
\nonumber\\
& & \sim\left(0.2\psi\pm0.3i\right)d(arg z_1)\wedge d(arg z_2)\wedge d(arg z_3),
\end{eqnarray}
and:
\begin{eqnarray}
\label{eq:vol C_3}
& &  {\rm vol}(C_3)\sim\sqrt{f^*g}f^*(dz_1\wedge dz_2\wedge dz_3)\sim\sqrt{(0.05)^3}{\cal V}^{\frac{2}{9}}d(arg
z_1)\wedge d(arg z_2)\wedge d(arg z_3)\Biggr|_{{\cal V}\sim10^6}\nonumber\\
& & \sim0.2d(arg z_1)\wedge d(arg z_2)\wedge d(arg z_3),
\end{eqnarray}
then relative to a phase $e^{-i\theta},\theta=\frac{\pi}{2}$,
$\Im m\left(f^*e^{-i\theta}\Omega\right)\sim 0.2\psi d(arg z_1)\wedge
d(arg z_2)\wedge d(arg z_3)$, which for $|\psi|<<1$, is close to
zero; (equivalently)$\Re\left(f^*e^{-i\theta}\Omega\right)\sim$
vol($C_3)$. This implies that $C_3$ is nearly/almost a special Lagrangian
sub-manifold
\cite{Kachru+McGreevy_slag}.

The ${\cal N}=1$ chiral co-ordinates  with the inclusion of mobile $D3$-brane
position moduli $z_{1,2}$ (which we identify with the $\Sigma_B$ coordinates) and mulitple matrix-valued $D7$-branes Wilson line moduli
${a_I}$ were guessed at in  \cite{gravitino_DM}. 
 the ${\cal N}=1$ chiral coordinates: $T_{\alpha=B,S},{\cal G}^{a=1,2},\zeta^A,z^{i=1,2}$
(See \cite{Jockers_thesis,D3_D7_Misra_Shukla} for definitions of all) - in particular:
\begin{eqnarray}
\label{eq:sigmas_Ts}
& & \sigma_\alpha\sim T_\alpha -\left( i\kappa_{\alpha bc}c^b{\cal B}^c + \kappa_\alpha + \frac{i}{(\tau - {\bar\tau})}\kappa_{\alpha bc}{\cal G}^b({\cal G}^c
- {\bar {\cal G}}^c) \right.\nonumber\\
 & & \left.+ i\delta^B_\alpha\kappa_4^2\mu_7l^2C_\alpha^{I{\bar J}}a_I{\bar a_{\bar J}} + \frac{3i}{4}\delta^B_\alpha\tau Q_{\tilde{f}} + i\mu_3l^2(\omega_\alpha)_{i{\bar j}} z^i\bigl({\bar z}^{\bar j}-\frac{i}{2}{\bar z}^{\tilde{a}}({\bar{\cal P}}_{\tilde{a}})^{\bar j}_lz^l\bigr)\right),
\end{eqnarray}
where (i) $\kappa_4$ is related to four-dimensional Newton's constant, $\mu_3$ and $\mu_7$ are $D3$ and $D7$-brane tensions; (ii) $\kappa_{\alpha ab}$'s are triple intersection integers of the CY orientifold; (iii)
 $c^a$ and $b^a$ are coefficients of RR and NS-NS two forms expanded in odd basis of $H^{(1,1)}_{{\bar\partial},-}(CY)$; (iv) $C^{I{\bar J}}_\alpha=\int_{\Sigma^B}i^*\omega_\alpha\wedge A^I\wedge A^{\bar J}$, $\omega_\alpha\in H^{(1,1)}_{{\bar\partial},+}(CY_3)$ and $A^I$ forming a basis for $H^{(0,1)}_{{\bar\partial},-}(\Sigma^B)$ - immersion map is defined as: $i:\Sigma^B\hookrightarrow CY_3$, $a_I$ is defined via a Kaluza-Klein reduction of the $U(1)$ gauge field (one-form) $A(x,y)=A_\mu(x)dx^\mu P_-(y)+a_I(x)A^I(y)+{\bar a}_{\bar J}(x){\bar A}^{\bar J}(y)$, where $P_-(y)=1$ if $y\in\Sigma^B$ and -1 if $y\in\sigma(\Sigma^B)$; (v)
 $z^{\tilde{a}}, \tilde{a}=1,...,h^{2,1}_-(CY_3),$ are $D=4$ complex structure deformations of the CY orientifold, $\left({\cal P}_{\tilde{a}}\right)^i_{\bar j}\equiv\frac{1}{||\Omega||^2}{\bar\Omega}^{ikl}\left(\chi_{\tilde{a}}\right)_{kl{\bar j}}$, i.e.,
${\cal P}:TCY_3^{(1,0)}\longrightarrow TCY_3^{(0,1)}$ via the transformation:
$z^i\stackrel{\rm c.s.\ deform}{\longrightarrow}z^i+\frac{i}{2}z^{\tilde{a}}\left({\cal P}_{\tilde{a}}\right)^i_{\bar j}{\bar z}^{\bar j}$, $z^i$ are scalar fields corresponding to geometric fluctuations of $D3$-brane inside the Calabi-Yau and defined via: $z(x)=z^i(x)\partial_i + {\bar z}^{\bar i}({\bar x}){\bar\partial}_{\bar i}$, and (vi)
 $Q_{\tilde{f}}\equiv l^2\int_{\Sigma^B}\tilde{f}\wedge\tilde{f}$, where $\tilde{f}\in\tilde{H}^2_-(\Sigma^B)\equiv{\rm coker}\left(H^2_-(CY_3)\stackrel{i^*}{\rightarrow}H^2_-(\Sigma^B)\right)$.

We estimate the intersection matrices $C_{I\bar{J}}^{B}$ in an appendix of \cite{gravitino_DM} by constructing harmonic one forms. Following the previous constructions in \cite{D3_D7_Misra_Shukla,ferm_masses_MS}, the harmonic distribution one-forms can be constructed by integrating: $dA_I=\left(P_{\Sigma_B}(z_{1,2,3})\right)^Idz_1\wedge dz_2$, with $I=1,2(done),3,4$ where
\begin{equation}
\label{eq:A I}
A_I\sim \delta\left(|z_3|-{\cal V}^{\frac{1}{6}}\right)\delta\left(|z_1|-{\cal V}^{\frac{1}{36}}\right)\delta\left(|z_2|-{\cal V}^{\frac{1}{36}}\right)\left[\omega_I(z_1,z_2)dz_1 + \tilde{\omega}_I(z_1,z_2)dz_2\right].
\end{equation}
 As the defining hypersurface of the Swiss-Cheese Calabi-Yau in $x_2\neq0$-coordinate patch
will be $z_1^{18} + z_2^{18} + ...$ which near $C_3$ (implying that the other two coordinates will scale like
${\cal V}^{\frac{1}{6}}, {\cal V}^{\frac{1}{6}} - {\cal V}^{\frac{1}{4}}$) receives the most dominant contributions from the monomials $z_1^{18}$ and
$z_2^{18}$ it is sufficient to consider ${\cal P}_{\Sigma_S}\Bigr|_{D3|_{{\rm near}\ C_3\hookrightarrow\Sigma_B}},{\cal P}_{\Sigma_B}|_{{\rm near}\ C_3\hookrightarrow\Sigma_B}\sim z_1^{18} + z_2^{18}$ with the understanding $|{\cal P}(z_{1,2,3},z_4=0;\phi,\psi)|_{C_3},|{\cal P}(z_{1,2,4},z_3;\phi,\psi)|_{C_3}<|z_1^{18}+z_2^{18}|$. One sees that $A_I$ is harmonic only on $\Sigma_B$ and not at any other generic locus in the Calabi-Yau manifold; (\ref{eq:A I}) shows that $A_I$ are distribution one-forms on $\Sigma_B$ localized along the $D3$-brane which is localized on the three-cycle $C_3$ of (\ref{eq:near_slag_i}). Writing $A_I(z_1,z_2)=\omega_I(z_1,z_2)dz_1+\tilde{\omega}_I(z_1,z_2)dz_2$,\footnote{Intuitively, these distribution one-forms could be thought of as
the holomorphic square-root of a Poincare dual of a four-cycle.} where $\omega(-z_1,z_2)=\omega(z_1,z_2)$, $\tilde{\omega}(-z_1,z_2)=-\tilde{\omega}(z_1,z_2)$ and $\partial_1\tilde{\omega}=-\partial_2\omega$, one obtains:
 \begin{eqnarray}
\label{eq:A_1234}
& & A_1|_{C_3}\sim - z_1^{18}z_2^{19}dz_1 + z_1^{19}z_2^{18}dz_2, A_2|_{C_3}\sim - z_1^{18}z_2dz_1 + z_2^{18}z_1 dz_2,\nonumber\\
& & A_3|_{C_3}\sim -z_1^{18}z_2^{37}dz_1 -z_2^{18}z_1^{37}dz_1, A_4|_{C_3}\sim -z_1^{36}z_2^{37}dz_1 + z_2^{36}z_1^{37}dz_2.
\end{eqnarray}
Utilizing above, one can calculate the intersection numbers $C_{I \bar J}$ corresponding to set of four-Wilson line moduli. The resultant contribution of various $C_{I \bar J}$'s are given in an appendix of \cite{gravitino_DM}.

Let's now look at the term quadratic in the $D3$-brane position moduli in $T_{\alpha=B,S}$ which is given by: $\left(\omega_\alpha\right)_{i{\bar j}}z^i\left({\bar z}^{\bar j} - \frac{i}{2}\left({\cal P}_{\tilde{a}}\right)^{\bar j}_{\ l}{\bar z}^{\tilde{a}}z^l\right)$, where $\left({\cal P}_{\tilde{a}}\right)^{\bar j}_{\ l}=\frac{\Omega^{{\bar j}{\bar k}{\bar m}}\left(\chi_{\tilde{a}}\right)_{{\bar k}{\bar m}l}}{||\Omega||^2}$\\
 $\sim\frac{g^{j_1{\bar j}}g^{k_1{\bar k}}g^{m_1{\bar m}}\Omega_{j_1k_1m_1}\left(\chi_{\tilde{a}}\right)_{{\bar k}{\bar m}l}}{g^{i_2{\bar i}_2}g^{j_3{\bar j}_3}g^{k_2{\bar k}_2}\Omega_{i_2j_2k_2}{\bar\Omega}_{{\bar i}_2{\bar j}_2{\bar k}_2}}$.
As $\omega_\alpha$ forms a basis of $H^{1,1}_+(CY_3)$ and $\chi_{\tilde{a}}$ forms a basis of $H^{2,1}_-(CY_3)$, this does not therefore depend on the choice of the divisor $\alpha$.
By Griffith's residue formula, $\Omega=\Omega_{124}dz_1\wedge dz_2\wedge dz_4$ where $\Omega_{124}=\frac{1}{\frac{\partial P(z_1,z_2,z_3,z_4)}{\partial z_3}}=\frac{1}{3z_3^2-\psi z_1z_2z_4}$. From $P(z_1,z_2,z_3,z_4)=0$, one obtains:
\begin{eqnarray}
\label{eq:z_3}
& &  z_3\sim \frac{\psi z_1z_2z_4}{\left(-\left(z_1^{18}+z_2^{18}+z_4^2-\phi z_1^6z_2^6\right)+\sqrt{\left(\psi z_1z_2z_4\right)^3+\left(z_1^{18}+z_2^{18}+z_4^2-\phi z_1^6z_2^6\right)^2}\right)^{\frac{1}{3}}}\nonumber\\
& & \hskip -0.15in + \left(-\left(z_1^{18}+z_2^{18}+z_4^2-\phi z_1^6z_2^6\right)+\sqrt{\left(\psi z_1z_2z_4\right)^3+\left(z_1^{18}+z_2^{18}+z_4^2-\phi z_1^6z_2^6\right)^2}\right)^{\frac{1}{3}},
\end{eqnarray}
which for $z_{1,2}\sim {\cal V}^{\frac{1}{36}}, z_4\sim {\cal V}^{\frac{1}{6}}$ yields $z_3\sim {\cal V}^{\frac{1}{6}}$. Hence, $\Omega_{124}\sim{\cal V}^{-\frac{1}{3}}$.
The polynomial deformation coefficient $\psi$ is a complex structure deformation modulus and given that it must be of the type $z^{\tilde{a}}$, i.e., odd under the holomorphic isometric involution $\sigma:z_1\rightarrow -z_1,z_{2,4}\rightarrow z_{2,4}$, $\sigma:\psi\rightarrow-\psi$. So, given that $\sigma^*\Omega=-\Omega$, hence $\sigma:\Omega_{124}\rightarrow\Omega_{124}$. Now, $\frac{1}{2}\left({\cal P}_{\tilde{a}}\right)^{\bar j}_{\ l}\sim\frac{\left(\chi_{\tilde{a}}\right)_{{\bar 4}{\bar 2}1}}{{\bar\Omega}_{{\bar 1}{\bar 2}{\bar 4}}}\sim\frac{{\cal V}^{\frac{1}{3}}}{2}\Biggr|_{{\cal V}\stackrel{<}{\sim}10^6}\sim{\cal O}(10)$. Assuming the complex structure moduli $z^{\tilde{a}}$ are stabilized at value ${\cal O}(10)z^{\tilde{a}}\sim{\cal O}(1)$ for ${\cal V}~{\lesssim}10^6$, one sees that contribution quadratic in $z^iz^j$ goes like $(\omega_\alpha)_{i{\bar j}}(z^i{\bar z}^{\bar j})$. $\omega_{B,S}$ are Poincare-duals of $\Sigma_{B,S}$ respectively. Hence, $\omega_{B,S}=\delta (P_{\Sigma_{B,S}})dP_{\Sigma_{B,S}}\wedge \delta({\bar P}_{\Sigma_{B,S}})d{\bar P}_{\Sigma_{B,S}}$.
Therefore one can argue (\cite{gravitino_DM,D3_D7_Misra_Shukla}) that near
$
|z_{1,2}|\equiv{\cal V}^{\frac{1}{36}}M_p,|z_3|\equiv{\cal V}^{\frac{1}{6}}M_p, |a_1|\equiv{\cal V}^{-\frac{2}{9}}M_p,
|a_2|\equiv{\cal V}^{-\frac{1}{3}}M_p, |a_3|\equiv{\cal V}^{-\frac{13}{18}}M_p,|a_4|\equiv{\cal V}^{-\frac{11}{9}}M_p;
\zeta^{A=1,...,h^{0,2}_-(\Sigma_B|_{C_3})}\equiv0$ (implying rigidity of the non-rigid $\Sigma_B$); ${\cal G}^a\sim\frac{\pi}{{\cal O}(1)k^a(\sim{\cal O}(10))}M_p,
$
 one obtains a local meta-stable dS-like minimum corresponding to the positive definitive potential
$e^KG^{T_S{\bar T}_S}|D_{T_S}W|^2$ stabilizing
${\rm vol}\left(\Sigma_B\right) = \Re e ({\sigma}_B)\sim{\cal V}^{\frac{2}{3}}, {\rm vol}\left(\Sigma_S\right) = \Re e{\sigma}_S\sim{\cal V}^{\frac{1}{18}}$ such that $\Re e T_S\sim{\cal V}^{\frac{1}{18}}$.\\
In the dilute flux approximation, the gauge couplings corresponding to the gauge theories living on stacks of $D7$ branes wrapping the ``big" divisor $\Sigma_B$  will given by:
\begin{eqnarray}
\label{eq:1overgsquared}
 \frac{1}{g_{j{=SU(3)\ {\rm or}\ SU(2)}}^2}&  = & \Re(T_{B}) + ln\left(\left.P\left(\Sigma_S\right)\right|_{D3|_{\Sigma_B}}\right) + ln\left(\left.{\bar P}\left(\Sigma_S\right)\right|_{D3|_{\Sigma_B}}\right)\nonumber\\
 & & + {\cal O}\left({\rm U(1)-Flux}_j^2\right).
\end{eqnarray}
Near the aforementioned stabilized values of the open string moduli,
\begin{eqnarray}
\label{eq:Casquared}
& & \left|C_{1{\bar 1}}|a_1|^2\right| \sim {\cal V}^{\frac{2}{3}},\ \left|C_{1{\bar 2}}\left(a_1{\bar a}_2 + h.c.\right)\right| \sim {\cal V}^{\frac{1}{18}},\ \left|C_{1{\bar 3}}\left(a_1{\bar a}_3 + h.c.\right)\right| \sim {\cal V}^{\frac{2}{3}},\nonumber\\
& & \left|C_{1{\bar 4}}\left(a_1{\bar a}_4 + h.c.\right)\right| \sim {\cal V}^{\frac{2}{3}},\
\left|C_{2{\bar 2}}|a_2|^2\right| \sim {\cal V}^{-\frac{5}{9}},\
\left|C_{2{\bar 3}}\left(a_2{\bar a}_3 + h.c.\right)\right| \sim {\cal V}^{\frac{1}{18}},\nonumber\\
& & \left|C_{2{\bar 4}}\left(a_2{\bar a}_4 + h.c.\right)\right| \sim {\cal V}^{\frac{1}{18}},\
\left|C_{3{\bar 3}}|a_3|^2\right| \sim {\cal V}^{\frac{2}{3}},\
\left|C_{3{\bar 4}}\left(a_3{\bar a}_4 + h.c.\right)\right| \sim {\cal V}^{\frac{2}{3}},\nonumber\\
& & \left|C_{4{\bar 4}}|a_4|^2\right| \sim {\cal V}^{\frac{2}{3}},
\end{eqnarray}
we see that there is the possibility that 
\begin{eqnarray}
Vol(\Sigma_B)+C_{I{\bar J}}a_I{\bar a}_{\bar J} + h.c.\sim {\cal V}^{\frac{1}{18}},
\end{eqnarray}
and hence $\frac{1}{g_{j{=SU(3)\ {\rm or}\ SU(2)}}^2} \sim {\cal V}^{\frac{1}{18}}\sim {\cal O}(1)$,
   as according to equation (\ref{eq:1overgsquared}). 

The K\"{a}hler potential relevant to all the calculations in chapters {\bf 2-4} (without being careful about ${\cal O}(1)$ constant factors) is given as under \footnote{One should include the perturbative $(\alpha^\prime)^3$ correction $\sum_{(m,n)\mathbb{Z}^2/(0,0)}\frac{\chi(CY_3)}{|m + n \tau|^3}$ and the perturbative $(\alpha^\prime)^2$ correction $\sqrt{\sigma_B + {\bar\sigma}_B}$ \cite{Rummel_et_al} as shifts in the argument of the logarithm. Further, due to the presence of the mobile $D3$-brane, one needs to include a $-\gamma K_{\rm geom}, \gamma\sim\frac{1}{\cal V}$ so that one considers $a_B(\tau_B + {\bar\tau}_B - \gamma K_{\rm geom})^{\frac{3}{2}} - a_S(\tau_S + {\bar\tau}_S - \gamma K_{\rm geom}) + \sum_\beta n^0_\beta(...)$. However, as was verified in \cite{gravitino_DM} using the Donaldson's algorithm, $\gamma K_{\rm geom}\sim\frac{ln {\cal V}}{\cal V}<<\langle\sigma_S\rangle(\sim {\cal V}^{\frac{1}{18}}),\langle\sigma_B\rangle(\sim{\cal V}^{\frac{2}{3}})$; it is hence justified to drop $\gamma K_{\rm geom}$ from the K\"{a}hler potential.}:
 \begin{eqnarray}
\label{eq:K}
& &  K\sim-2 ln\left(a_B\Biggl[\frac{T_B+{\bar T}_B}{M_p} - \mu_3(2\pi\alpha^\prime)^2
\frac{\left\{|z_1|^2 + |z_2|^2 + z_1{\bar z}_2 + z_2{\bar z}_1\right\}}{M_p^2}
 +{\cal V}^{\frac{10}{9}}\frac{|a_1|^2}{M_p^2}\right.\nonumber\\
 & &+{\cal V}^{\frac{11}{18}}
 \frac{\left(a_1{\bar a}_2+h.c.\right)}{M_p^2} +{\cal V}^{\frac{1}{9}}\frac{|a_2|^2}{M_p^2} + {\cal V}^{\frac{29}{18}}
 \frac{\left(a_1{\bar a}_3+h.c.\right)}{M_p^2}+ {\cal V}^{\frac{10}{9}}
 \frac{\left(a_2{\bar a}_3+h.c.\right)}{M_p^2} \nonumber \\
 & & + {\cal V}^{\frac{19}{9}}\frac{|a_3|^2}{M_p^2} + {\cal V}^{\frac{19}{9}}\frac{\left(a_1{\bar a}_4 + a_4{\bar a}_1\right)}{M_p^2} +  {\cal V}^{\frac{29}{18}}\frac{\left(a_2{\bar a}_4 + a_4{\bar a}_2\right)}{M_p^2}+ {\cal V}^{\frac{47}{18}}\frac{\left(a_3{\bar a}_4 + a_4{\bar a}_3\right)}{M_p^2}\nonumber \\
 & & + {\cal V}^{\frac{28}{9}}\frac{|a_4|^2)}{M_p^2}
\Biggr]^{3/2}- \nonumber\\
& & \left. a_S\left(\frac{{T_S+{\bar T}_S}}{M_p}-\mu_3(2\pi\alpha^\prime)^2 \frac{\left\{|z_1|^2 + |z_2|^2 + z_1{\bar z}_2 + z_2{\bar z}_1\right\}}{M_p^2}\right)^{3/2} +\sum n^0_\beta(...)\right),
\end{eqnarray}
\vskip -0.09in
\noindent 
and ED3 generated non-perturbative superpotential  is given by \cite{nonpert,Ganor1_2}:
\begin{eqnarray}
\label{eq:W}
\begin{array}{r}
  W\sim\left({\cal P}_{\Sigma_S}\Bigr|_{D3|_{{\rm near}\ C_3\hookrightarrow\Sigma_B}}\sim z_1^{18} + z_2^{18}\right)^{n^s}\sum_{m_a}e^{i\tau\frac{m^2}{2}}e^{in^s G^am_a} e^{i n^s T_s},
\end{array}
\end{eqnarray}
\vskip -0.09in
\noindent which is like (\ref{W_pheno}) assuming $G^a, \tau$ has been stabilized. The  genus-zero Gopakumar-Vafa invariants (which for projective varieties are very large) prefix the $h^{1,1}_-$-valued real axions $b^a,c^a$. In general there are no known globally defined involutions, valid for all Calabi-Yau volumes, for which $h^{1,1}_-(CY_3)\neq0, h^{0,1}_-(\Sigma_B
)\neq0$.
However, as mentioned earlier, in the spirit of the involutive mirror symmetry
implemented a la SYZ prescription in terms of a triple of T dualities along a
local $T^3$ in the large volume limit, we argued in \cite{ferm_masses_MS},
e.g., $z_1\rightarrow-z_1$ would, restricted to $C_3$, generate non-zero
$h^{1,1}_-\left(\begin{array}{c} T^3(arg z_{1,2,3})\rightarrow{\cal M}_3(z_{1,2,3})\\
\hskip1in\downarrow \\
\hskip 0.3in M_3(|z_1|,|z_2|,|z_3|) \end{array}  \right)$. An example of holomorphic involutions near $C_3$  not requiring a
large Calabi-Yau volume has been discussed in \cite{gravitino_DM}. However, even if $h^{1,1}_-=0$, one can self-consistently stabilize $c^a,b^a$ to zero and $\sigma_s,\sigma_b$ to ${\cal V}^{\frac{1}{18}}, {\cal V}^{\frac{2}{3}}$ such that the K\"{a}hler potential continues to be stabilized at $- 2 ln {\cal V}$.

The evaluation of ``physical"/normalized Yukawa couplings, soft SUSY breaking parameters and various 3-point vertices needs the matrix generated from the mixed double derivative of the K\"{a}hler potential to be a diagonalized matrix. After diagonalization  the corresponding eigenvectors of the same are given by:
\begin{eqnarray}
\label{eq:eigenvectors}
\begin{array}{l}
  {\cal A}_4\sim a_4 + {\cal V}^{-\frac{3}{5}}a_3 + {\cal V}^{-\frac{6}{5}} a_1+{\cal V}^{-\frac{9}{5}} a_2 + {\cal V}^{-2}\left(z_1+z_2\right),\\
{\cal A}_3\sim -a_3 + {\cal V}^{-\frac{3}{5}}a_4 - {\cal V}^{-\frac{3}{5}}a_1 - {\cal V}^{-\frac{7}{5}}a_2 + {\cal V}^{-\frac{8}{5}}\left(z_1+z_2\right),\\
  {\cal A}_1\sim a_1 - {\cal V}^{-\frac{3}{5}}a_3 + {\cal V}^{-1}a_2 - {\cal V}^{-\frac{6}{5}}a_4+ {\cal V}^{-\frac{6}{5}}\left(z_1+z_2\right),\\
{\cal A}_2\sim - a_2 - {\cal V}^{-1}a_1 + {\cal V}^{-\frac{7}{5}}a_3 - {\cal V}^{-\frac{3}{5}}\left(z_1+z_2\right),\\
{\cal Z}_2\sim - \frac{\left(z_1+z_2\right)}{\sqrt 2}  - {\cal V}^{-\frac{6}{5}}a_1 + {\cal V}^{-\frac{3}{5}}a_2 + {\cal V}^{-\frac{8}{5}}a_3+ {\cal V}^{-2}a_4,\\
{\cal Z}_1\sim \frac{\left(z_1-z_2\right)}{\sqrt 2}  - {\cal V}^{-\frac{6}{5}}a_1 + {\cal V}^{-\frac{3}{5}}a_2 + {\cal V}^{-\frac{8}{5}}a_3+ {\cal V}^{-2}a_4.
\end{array}
\end{eqnarray}
and the numerical eigenvalues are estimated to be:
\begin{eqnarray}
\label{eq:eigenvals}
 && K_{{\cal Z}_1{\cal Z}_1} \sim10^{-5},K_{{\cal Z}_2{\cal Z}_2}\sim 10^{-3}, K_{{\cal A}_1{\cal A}_1}\sim 10^4,\nonumber\\
 && K_{{\cal A}_2{\cal A}_2}\sim10^{-2}, K_{{\cal A}_3{\cal A}_3}\sim 10^7, K_{{\cal A}_4{\cal A}_4}\sim 10^{12}.
\end{eqnarray}
 The system of equations (\ref{eq:eigenvectors}) are inverted, and solved for ($z_{1,2}, a_{1,2,3,4}$) in terms of (${\cal Z}_{1,2}, {\cal A}_{1,2,3,4}$) and used. 
 
 We will now consider four stacks of $D7$-branes: a stack of 3, a stack of 2 and two stacks of 1. The matter fields: L-quarks and their superpartners will be valued in the bifundamentals $(3,{\bar 2})$ under $SU(3)_c\times SU(2)_L$; the L-leptons and their superpartners will be valued in the bifundamentals
$(2,\bar{-1})$ of $SU(2)_L\times U(1)_Y$.  Before the  fluxes (\ref{eq:flux})  are turned on,
the Wilson line moduli are valued in the adjoint of $U(7)$. With the following choice of fluxes:
{\footnotesize{
 \begin{equation}
\label{eq:flux}
F = \left(\begin{array}{ccccccc}f_1 & 0 & 0 & 0 & 0 & 0&0\\
0 & f_1 & 0 & 0 & 0 & 0&0\\
0 & 0 & f_1 & 0 & 0 & 0&0\\
0 & 0 & 0 & f_2 & 0 & 0&0\\
0 & 0 & 0 & 0 & f_2 & 0&0\\
0 & 0 & 0 & 0 & 0 & f_3&0\\
0 & 0 & 0 & 0 & 0 & 0 & f_4
\end{array}\right),
\end{equation}}}
the $U(7)$ is broken down to $U(3)\times U(2)\times U(1)\times U(1)$. So, the bifundamental Wilson line super-moduli ${\cal A}_I$  will be represented as:
\begin{equation}
\label{eq:Q L_I}
{\cal A}_I=\sum a_I^{ab}e_{ab} + \sum\theta \tilde{a}_I^{ab}e_{ab},\ \left[(a,b)=1,...,7\right],
\end{equation}
where $\left(e_{ab}\right)_{ij}=\delta_{ai}\delta_{bj}$. Hence,
{\footnotesize{
  \begin{equation}
 \label{eq:e_L}
{\cal A}_1 =
 \left(\begin{array}{ccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & \tilde{\nu}_e + \theta\nu_e   & 0\\
 0 & 0 & 0 & 0 & 0 & \tilde{e} + \theta e & 0\\
 0 & 0 & 0 & \bar{\tilde{\nu}}_e + {\bar\theta}{\bar\nu}_e  &  \bar{\tilde{e}} + {\bar\theta}{\bar e} & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0
 \end{array} \right),
\end{equation}
  \begin{equation}
\label{eq:Q L}
{\cal A}_2 =
\left(\begin{array}{ccccccc}
0 & 0 & 0 & \tilde{u}  + \theta u & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & 0 & 0\\
\bar{\tilde{u}}  + {\bar\theta}{u}^\dagger &  0 & 0 & 0 & 0 & 0 & 0\\
0 &  0 & 0 & 0 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & 0 & 0
\end{array}\right),
\end{equation}
and
\begin{equation}
\label{eq:e_R}
{\cal A}_3 =
\left(\begin{array}{ccccccc}
0 & 0 & 0 & 0 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 &  0 & 0 & 0 & 0 & 0 & 0\\
0 &  0 & 0 & 0 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & 0 & \tilde{e}_R + \theta e_R \\
0 & 0 & 0 & 0 & 0 & \bar{\tilde{e}}_R + {\bar\theta}{e}_R^\dagger & 0
\end{array}\right),
\end{equation}
\begin{equation}
 \label{eq:f_R}
 {\cal A}_4 =
\left(\begin{array}{ccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & \tilde{u}_R + \theta u_R\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 &  0 & 0 & 0 \\
 \bar{\tilde{u}}_R + {\bar\theta}u_R^\dagger & 0 & 0 & 0 & 0 & 0 & 0
 \end{array} \right).
\end{equation}
}}
Unlike the ${\cal A}_I$  which correspond to matter fields
corresponding to open strings stretched between two stacks of $D7$
branes (with different two-form fluxes turned on their world
volumes), the Higgses would arise as a geometric moduli corresponding
to the fluctuations in the position of the mobile space-time filling
$D3$-brane. Now, we will see if one can construct appropriate  $a_I$ (bi-fundamental)
and $z_i$(mimicking bi-fundamental fields) such that
(\ref{eq:eigenvectors}), (\ref{eq:e_L}) - (\ref{eq:f_R}), as well as:
{\footnotesize{
\begin{equation}
\label{eq:H_u}
{\cal Z}_1=\left(\begin{array}{ccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & H_u + \theta\tilde{H}_u   & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & \bar{H}_u + {\bar\theta}\tilde{H}_u^\dagger  &  0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0
 \end{array} \right),
\end{equation}
and
\begin{equation}
\label{eq:H_d}
{\cal Z}_2=\left(\begin{array}{ccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0   & 0\\
 0 & 0 & 0 & 0 & 0 & H_d + \theta\tilde{H}_d & 0\\
 0 & 0 & 0 &0  &  \bar{H}_d + {\bar\theta}\tilde{H}_d^\dagger & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0
 \end{array} \right),
\end{equation}
}}
 are satisfied. It was shown in \cite{gravitino_DM}  the following solution:
 {\footnotesize{
\begin{eqnarray*}
\label{eq:sols_a_I}
& &    a_1 = \left(\begin{array}{ccccccc}
0 & 0 & 0 & \xi_1^{14}{\cal V}^{-\frac{7}{5}} \tilde{u}_L & 0 & 0 &
\xi_1^{17}{\cal V}^{-\frac{11}{5}} \tilde{u}_R \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\xi_1^{14}{\cal V}^{-\frac{7}{5}} {\bar{\tilde{u}}}_L & 0 & 0 & 0 & 0 &
\xi_1^{46}\left(\frac{\tilde{e}_L}{2} + {\cal V}^{-\frac{8}{5}}H_u\right) & 0 \\
0 & 0 & 0 & 0 & 0 & \xi_1^{56}{\cal V}^{-\frac{8}{5}} H_d & 0 \\
0 & 0 & 0 &{\bar\xi}_1^{46}\left( \frac{{\bar{\tilde{e}}}_L}{2} + {\cal V}^{-\frac{8}{5}}{\bar H}_u\right) &
{\bar\xi}_1^{56}{\cal V}^{-\frac{8}{5}} {\bar H}_d & 0 & -\xi_1^{67} {\cal V}^{-\frac{4}{5}} e_R
\\
{\bar\xi}_1^{17}{\cal V}^{-\frac{11}{5}} {\bar{\tilde{u}}}_R & 0 & 0 & 0 & 0 &
-{\bar\xi}_1^{67}  {\cal V}^{-\frac{4}{5}} {\bar{\tilde{e}}}_R
\end{array}\right),\nonumber\\
& &  \nonumber\\
&&  \nonumber\\
&&  \nonumber\\
& &  a_2 = \left(\begin{array}{ccccccc}
0 & 0 & 0 & 0.3\xi_2^{14} \tilde{u}_L & 0 & 0 &
\xi_2^{17}{\cal V}^{-\frac{13}{5}} \tilde{u}_R \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0.3\xi_2^{14} {\bar{\tilde{u}}}_L & 0 & 0 & 0 & 0 &
\xi_2^{46}\left(-{\cal V}^{-\frac{7}{5}}\tilde{e}_L + {\cal V}^{-\frac{4}{5}}H_u\right) & 0 \\
0 & 0 & 0 & 0 & 0 & 5\xi_2^{56}{\cal V}^{-\frac{6}{5}} H_d & 0 \\
0 & 0 & 0 &{\bar\xi}_2^{46}\left( -{\cal V}^{-\frac{7}{5}}{\bar{\tilde{e}}}_L +
  {\cal V}^{-\frac{4}{5}}{\bar H}_u\right) &
5{\bar\xi}_2^{56}{\cal V}^{-\frac{6}{5}} {\bar H}_d & 0 & -\xi_2^{67} {\cal V}^{-\frac{9}{5}} e_R
\\
{\bar\xi}_2^{17}{\cal V}^{-\frac{13}{5}} {\bar{\tilde{u}}}_R & 0 & 0 & 0 & 0 &
-{\bar\xi}_2^{67}  {\cal V}^{-\frac{9}{5}} {\bar{\tilde{e}}}_R
\end{array}\right),\nonumber\\
\end{eqnarray*}
\begin{eqnarray}
\label{eq:sols_a_I_ii}
& & a_3 = \left(\begin{array}{ccccccc}
0 & 0 & 0 & \xi_3^{14}\frac{\tilde{u}_L}{{\cal V}} & 0 & 0 &
-6\xi_3^{17} \frac{\tilde{u}_R}{{\cal V}} \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
{\bar\xi}_3^{14}\frac{{\bar{\tilde{u}}}_L}{{\cal V}} & 0 & 0 & 0 & 0 &
\xi_3^{46}\left(-{\cal V}^{-\frac{4}{5}}\tilde{e}_L + {\cal V}^{-\frac{8}{5}}H_u\right) & 0 \\
0 & 0 & 0 & 0 & 0 & \xi_3^{56}{\cal V}^{-\frac{11}{5}} H_d & 0 \\
0 & 0 & 0 &{\bar\xi}_3^{46}\left(-{\cal V}^{-\frac{4}{5}}\tilde{e}_L + {\cal V}^{-\frac{8}{5}}H_u\right) &
5{\bar\xi}_3^{56}{\cal V}^{-\frac{11}{5}} {\bar H}_d & 0 & 0.3\xi_3^{67} e_R
\\
{\bar\xi}_3^{17}{\cal V}^{-\frac{13}{5}} {\bar{\tilde{u}}}_R & 0 & 0 & 0 & 0 &
0.3{\bar\xi}_3^{67}  {\bar{\tilde{e}}}_R
\end{array}\right),\nonumber\\
& &  \nonumber\\
&&  \nonumber\\
&&  \nonumber\\
& &  a_4 = \left(\begin{array}{ccccccc}
0 & 0 & 0 & 0.08\xi_4^{14}\tilde{u}_L & 0 & 0 &
0.2\xi_4^{17} \tilde{u}_R \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0.08{\bar\xi}_4^{14}{\bar{\tilde{u}}}_L & 0 & 0 & 0 & 0 &
\xi_4^{46}{\cal V}^{-\frac{7}{5}}\tilde{e}_L & 0 \\
0 & 0 & 0 & 0 & 0 & \xi_4^{56}{\cal V}^{-\frac{14}{5}} H_d & 0 \\
0 & 0 & 0 &{\bar\xi}_4^{46}{\cal V}^{-\frac{7}{5}}{\bar{\tilde{e}}}_L &
{\bar\xi}_4^{56}{\cal V}^{-\frac{14}{5}} {\bar H}_d & 0 & -7\xi_4^{67} e_R
\\
0.2{\bar\xi}_4^{17} {\bar{\tilde{u}}}_R & 0 & 0 & 0 & 0 &
-7{\bar\xi}_4^{67}  {\bar{\tilde{e}}}_R
\end{array}\right).\nonumber\\
\end{eqnarray}
\begin{eqnarray*}
z_1=\left(\begin{array}{ccccccc}
0 & 0 & 0 & \alpha_1^{14}\frac{\tilde{u}_L}{{\cal V}} & 0 & 0 &
5\alpha_1^{17}{\cal V}^{-\frac{14}{5}} \tilde{u}_R \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
{\bar\alpha}_1^{14}\frac{{\bar{\tilde{u}}}_L}{{\cal V}} & 0 & 0 & 0 & 0 &
\alpha_1^{46}\left({\cal V}^{-\frac{9}{5}}\tilde{e}_L - \frac{H_u}{\sqrt{2}}\right) & 0 \\
0 & 0 & 0 & 0 & 0 & \alpha_1^{56} \frac{H_d}{\sqrt{2}} & 0 \\
0 & 0 & 0 &{\bar\alpha}_1^{46}\left({\cal V}^{-\frac{9}{5}}{\bar {\tilde e}}_L -
  \frac{{\bar H}_u}{\sqrt{2}}\right) &
{\bar\alpha}_1^{56} \frac{{\bar H}_d}{\sqrt{2}} & 0 & \alpha_1^{67} {\cal
  V}^{-\frac{11}{5}}e_R
\\
5{\bar\alpha}_1^{17}{\cal V}^{-\frac{14}{5}} {\bar{\tilde{u}}}_R & 0 & 0 & 0 & 0 &
{\bar\alpha}_1^{67} {\cal
  V}^{-\frac{11}{5}}  {\bar{\tilde{e}}}_R
\end{array}\right),\nonumber\\
\end{eqnarray*}
\begin{eqnarray}
\label{eq:sols z_i}
& & z_2=\left(\begin{array}{ccccccc}
0 & 0 & 0 & \alpha_2^{14}{\cal V}^{-\frac{4}{5}}{\tilde{u}_L} & 0 & 0 &
5\alpha_2^{17}{\cal V}^{-\frac{13}{5}} \tilde{u}_R \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
{\bar\alpha}_2^{14}{\cal V}^{-\frac{4}{5}}{\bar{u}_L} & 0 & 0 & 0 & 0 &
\alpha_2^{46}\left(6{\cal V}^{-\frac{8}{5}}\tilde{e}_L - \frac{H_u}{\sqrt{2}}\right) & 0 \\
0 & 0 & 0 & 0 & 0 & -\alpha_2^{56} \frac{H_d}{\sqrt{2}} & 0 \\
0 & 0 & 0 &{\bar\alpha}_2^{46}\left({\cal V}^{-\frac{8}{5}}\bar {\tilde e}_L -
  \frac{{\bar H}_u}{\sqrt{2}}\right) &
-{\bar\alpha}_2^{56} \frac{{\bar H}_d}{\sqrt{2}} & 0 &
\alpha_2^{67}\frac{{\tilde e_R}}{{\cal V}^{-2}}
\\
5{\bar\alpha}_2^{17}{\cal V}^{-\frac{13}{5}} {\bar{\tilde{u}}}_R & 0 & 0 & 0 & 0 &
{\bar\alpha}_2^{67}\frac{\bar {\tilde e_R}}{{\cal V}^{-2}}
\end{array}\right).\nonumber\\
& &
\end{eqnarray}}}
In (\ref{eq:sols_a_I_ii}) and (\ref{eq:sols z_i}), $\xi_{I,i}^{ab}$ and $\alpha_{I,i}^{ab}, 
1\leq a\leq 6, 1\leq b\leq7$ are ${\cal O}(1)$ numbers. The intersection matrix was worked out in \cite{gravitino_DM}. Assuming
that the complex structure moduli
$z^{\tilde{a}=1,...,h^{2,1}_-(CY_3)}$ are stabilized at very small
values, which is in fact already assumed in writing
(\ref{eq:sigmas_Ts}) which has been written upon inclusion of terms up
to linear in the complex structure moduli, let us define a modified
intersection matrix in the $a_I-z_i$ moduli space:
\begin{eqnarray}
\label{eq:CIJbar mod}
& & {\cal C}^{{\cal I}{\cal J}}=C^{I{\bar J}},\ {\cal I}=I, {\cal
  J}={\bar J};   {\cal C}^{{\cal I}{\cal J}}
=\mu_3\left(2\pi\alpha^\prime\right)^2\left(\omega_\alpha
\right)^{i{\bar j}},\ {\cal I}=i, {\cal
  J}={\bar j};\nonumber\\
& &  {\cal C}^{{\cal I}{\cal J}}=0,\ {\cal I}=I, {\cal
  J}={\bar j},\ {\rm etc.}.
\end{eqnarray}
Now, from (\ref{eq:sols_a_I}) and (\ref{eq:sols z_i}), one can show
that for $|z_i|\sim0.8{\cal V}^{\frac{1}{36}},\ {\cal V}\sim10^5$:
\begin{eqnarray}
\label{eq:tr-1}
& & {\cal C}^{{\cal I}\bar{\cal J}}Tr({\cal M}_{\cal I} {\cal M}_{\cal
  J}^\dagger)\sim
C^{a_1\bar{a}_1}|\tilde{e}_L|^2 + C^{a_2\bar{a}_2}|\tilde{u}_L|^2 +
C^{a_3\bar{a}_3}|\tilde{e}_R|^2
+ C^{a_4\bar{a}_4}|\tilde{u}_R|^2 \nonumber\\
&& +\mu_3\left(2\pi\alpha^\prime\right)^2|H_u|^2,
\end{eqnarray}
where ${\cal M}_{\cal I}\equiv a_I, z_i$. 

Now, using (\ref{eq:eigenvectors}), one can show that in the large volume limit:
 ${\cal C}^{{\cal A}_I\bar{\cal A}_{\bar J}}\sim C^{a_I\bar{a}_{\bar J}}$, 
 ${\cal C}^{{\cal Z}_i\bar{\cal Z}_{\bar j}}\sim {\cal C}^{z_i\bar{z}_j}$. Clubbing together the Wilson line moduli and the $D3$-brane position moduli into a single vector: ${\cal M}_{\Lambda}\equiv {\cal A}_I,{\cal Z}_i$, then one sees from (\ref{eq:e_L}) - (\ref{eq:H_d}), and (\ref{eq:tr-1}): ${\cal C}^{\Lambda\bar{\Sigma}}Tr\left({\cal M}_\Lambda{\cal M}_{\Sigma}^\dagger\right)\sim {\cal C}^{{\cal I}\bar{\cal J}}Tr({\cal M}_{\cal I} {\cal M}_{\cal
  J}^\dagger)$.
  In the large volume and rigid limit of $\Sigma_B(\zeta^A=0$ which corresponds to a local minimum), perhaps $ {\cal C}^{\Lambda\bar{\Sigma}}Tr\left({\cal M}_\Lambda{\cal M}_{\Sigma}^\dagger\right)$ is invariant under moduli transformations in the $({\cal A}_I,{\cal Z}_i)/(a_I,z_i)$-subspace of the open-string moduli space, which would imply that $C^{I{\bar J}}a_I{\bar a}_{\bar J} + \mu_3\left(\alpha^\prime\right)^2\left(\omega_B\right)_{i{\bar j}}z^i{\bar z}^{\bar j}$ for multiple  $D7$-branes, in a basis that diagonalizes $g_{{\cal M}_{\cal I}\bar{\cal M}_{\bar J}}$ at stabilized values of the open string moduli,  is replaced by (\ref{eq:tr-1}).

 The effective Yukawa couplings can be calculated using $\hat{Y}^{\rm eff}_{C_i C_j C_k}\equiv\frac{e^{\frac{K}{2}}Y^{\rm eff}_{C_i C_j C_k}}{\sqrt{K_{C_i{\bar C}_i}K_{C_j{\bar C}_j}K_{C_k{\bar C}_k}}}$, $C_i$ being an open string modulus which for us is $\delta{\cal Z}_{1,2},\delta{\cal A}_{1,2,3,4}$, where, e.g., $Y^{\rm eff}_{{\cal Z}_i{\cal A}_{1/2}{\cal A}_{3/4}}$ is the ${\cal O}({\cal Z}_i)$-coefficient in the following mass term in the ${\cal N}=1$ SUGRA action of \cite{Wess_Bagger}: $e^{\frac{K}{2}}{\cal D}_{{\bar{\cal A}}_{1/2}}D_{{\bar{\cal A}}_{3/4}}{\bar W}{\bar\chi}^{{\cal A}_{1/3}}\chi^{{\cal A}_{2/4}}$. Using inverted eigenvectors of (\ref{eq:eigenvectors}), and:
\begin{eqnarray}
\label{eq:expKover2_calD_DW}
& & e^{\frac{K}{2}} {\cal D}_{z_1} D_{z_1}W = {\cal V}^{-\frac{43}{72}},\  e^{\frac{K}{2}} {\cal D}_{z_1} D_{a_1}W = {\cal V}^{-\frac{89}{72}},\
 e^{\frac{K}{2}} {\cal D}_{z_1} D_{a_2}W = {\cal V}^{-\frac{125}{72}},\nonumber\\
& & e^{\frac{K}{2}} D_{z_1} D_{a_3}W = {\cal V}^{-\frac{25}{36}},\ e^{\frac{K}{2}} D_{z_1} D_{a_4}W = {\cal V}^{-\frac{17}{72}},\
e^{\frac{K}{2}} D_{a_1} D_{a_1}W = {\cal V}^{-\frac{71}{72}},\nonumber\\
& & e^{\frac{K}{2}} {\cal D}_{a_1} D_{a_2}W = {\cal V}^{-\frac{107}{72}},\  e^{\frac{K}{2}} {\cal D}_{a_1} D_{a_3}W = {\cal V}^{-\frac{35}{72}},\
e^{\frac{K}{2}} {\cal D}_{a_1} D_{a_4}W = {\cal V}^{\frac{1}{72}},\nonumber\\
& & e^{\frac{K}{2}} {\cal D}_{a_2} D_{a_2}W = {\cal V}^{-\frac{1}{72}},\ e^{\frac{K}{2}} {\cal D}_{a_2} D_{a_3}W = {\cal V}^{-\frac{3}{4}},\
e^{\frac{K}{2}} {\cal D}_{a_2} D_{a_4}W = {\cal V}^{-\frac{5}{9}},\nonumber\\
& & e^{\frac{K}{2}} {\cal D}_{a_3} D_{a_3}W = {\cal V}^{\frac{1}{72}},\ e^{\frac{K}{2}} {\cal D}_{a_3} D_{a_4}W = {\cal V}^{\frac{37}{72}},\  e^{\frac{K}{2}} {\cal D}_{a_4} D_{a_4}W = {\cal V}^{\frac{73}{72}},
\end{eqnarray}
 one can verify that
$e^{\frac{K}{2}}{\cal D}_{{\cal A}_I}D_{{\cal A}_J}\bar{W}\sim e^{\frac{K}{2}}{\cal D}_{a_I}D_{a_J}\bar{W}$. Now, $\left(e^{\frac{K}{2}}{\cal D}_{\bar{\lambda}}D_{\bar{\Sigma}}\bar{W}\right)\bar{\chi}_L^{{\lambda}}\chi_R^{\Sigma}=\left(e^{\frac{K}{2}}{\cal D}_{\bar{\cal I}}D_{\bar{\cal J}}\bar{W}\right)\bar{\chi}_L^{{\cal I}}\chi_R^{\cal J}$, where $\lambda/\Sigma$ index ${\cal A}_I, {\cal Z}_J$ and ${\cal I}/{\cal J}$ index $a_I,z_i$. What is interesting is that using (\ref{eq:eigenvectors}), e.g.,
\begin{eqnarray}
\label{eq:eq_mass_terms_diag_non-diag_basis}
& & \left(e^{\frac{K}{2}}{\cal D}_{\bar{\cal A}_{1,2}}D_{\bar{\cal A}_{3,4}}\bar{W}\right)\bar{\chi}_L^{{\cal A}_{1,2}}\chi_R^{{\cal A}_{3,4}}\sim\left(e^{\frac{K}{2}}{\cal D}_{\bar{a}_{1,2}}D_{\bar{a}_{3,4}}\bar{W}\right)\bar{\chi}_L^{{\cal A}_{1,2}}\chi_R^{{\cal A}_{3,4}}=\nonumber\\
&& {\hskip -0.3in} \left(\frac{\partial\bar{\cal A}_{1,2}}{\partial\bar{\cal M}_{\cal I}}\right)\left(\frac{\partial\bar{\cal A}_{3,4}}{\partial\bar{\cal M}_{\bar J}}\right) \left(e^{\frac{K}{2}}{\cal D}_{\bar{a}_{1,2}}D_{\bar{a}_{3,4}}\bar{W}\right)\bar{\chi}_L^{{\cal M}_{\cal I}}\chi_R^{{\cal M}_{\cal J}}  \sim \left(e^{\frac{K}{2}}{\cal D}_{\bar{a}_{1,2}}D_{\bar{a}_{3,4}}\bar{W}\right)\bar{\chi}_L^{{a}_{1,2}}\chi_R^{a_{3,4}}.
\end{eqnarray}
This implies that the mass terms, in the large volume limit, are invariant under diagonalization of the open string moduli, and \\
 $\bullet$\begin{equation}
\label{eq:Yhatz1a1a2} \frac{{\cal O}({\cal Z}_i)\ {\rm term\ in}\
e^{\frac{K}{2}}{\cal D}_{{\cal A}_1}D_{{\cal A}_3}W}{\sqrt{K_{{\cal Z}_i\bar{\cal Z}_i}K_{{\cal A}_1\bar{\cal A}_1}K_{{\cal A}_3\bar{\cal A}_3}}}\equiv
\hat{Y}^{\rm eff}_{{\cal Z}_i{\cal A}_1{\cal A}_3}\sim 10^{-3}\times {\cal V}^{-\frac{4}{9}},
\end{equation}
which implies that for ${\cal V}\sim 10^5, \langle {\cal Z}_i\rangle\sim 246 GeV$,
 $\langle {\cal Z}_i\rangle \hat{Y}_{{\cal Z}_1{\cal A}_1{\cal A}_3}\sim MeV$ - about the mass of the electron!\\
$\bullet$
\begin{equation}
\label{eq:Yhatz1a1a2}\frac{{\cal O}({\cal Z}_i)\ {\rm term\ in}\
e^{\frac{K}{2}}{\cal D}_{{\cal A}_2}D_{{\cal A}_4}W}{\sqrt{K_{{\cal Z}_i\bar{\cal Z}_i}K_{{\cal A}_2\bar{\cal A}_2}K_{{\cal A}_4\bar{\cal A}_4}}}\equiv
\hat{Y}^{\rm eff}_{{\cal Z}_i{\cal A}_2{\cal A}_4}\sim 10^{-\frac{5}{2}}\times {\cal V}^{-\frac{4}{9}},
\end{equation}
which implies that for ${\cal V}\sim 10^5,\langle {\cal Z}_i\rangle\sim 246 GeV$,
 $\langle z_i\rangle \hat{Y}_{{\cal Z}_i{\cal A}_1{\cal A}_2}\sim10MeV$ - close to the mass of the up quark!
\\
$~~~$There is an implicit assumption that the VEV of the $D3$-brane position moduli, identified with the neutral components of two Higgs doublets, can RG-flow down to $246 GeV$ - that the same is possible was shown in \cite{ferm_masses_MS}. The RG-flow of the effective physical Yukawas are expected to change by ${\cal O}(1)$ under an RG flow from the string scale down to the EW scale. This can be motivated by looking at RG-flows of the physical Yukawas $\hat{Y}_{\Lambda\Sigma\Delta}$ in MSSM-like models:
\begin{equation}
 \frac{d\hat{Y}_{\Lambda\Sigma\Delta}}{dt} = \gamma_{\Lambda}^\kappa\hat{Y}_{\kappa\Sigma\Delta}
+ \gamma_{\Sigma}^{\kappa}\hat{Y}_{\Lambda\kappa\Delta} + \gamma_{\Delta}^\kappa\hat{Y}_{\Lambda\Sigma\kappa},
\end{equation}
 where the anomalous dimension matrix $\gamma_\Lambda^\kappa$, at one loop, is defined as: \\
 $\gamma_\Lambda^\kappa = \frac{1}{32\pi^2}\left(\hat{Y}_{\Lambda\Psi\Upsilon}\hat{Y}^*_{\kappa\Psi\Upsilon} - 2 \sum_{(a)}g_{(a)}^2C_{(a)}(\Phi_\Lambda)\delta_{{\cal I}}^{\kappa}\right)$, $(a)$ indexes the three gauge groups and $\Lambda$, etc. index
the diagonalized basis fields ${\cal A}_I,{\cal Z}_i$. Using
(\ref{eq:W}), one can show that at $M_s$(string scale):
\begin{eqnarray}
\label{eq:Yhats}
& & \hat{Y}_{{\cal Z}_i{\cal Z}_j{\cal Z}_k}\sim{\cal
  V}^{\frac{1}{8}},\ \hat{Y}_{{\cal Z}_i{\cal Z}_i{\cal
    A}_1}\sim{\cal
  V}^{-\frac{79}{40}},\
\hat{Y}_{{\cal Z}_i{\cal Z}_i{\cal A}_2}\sim{\cal
  V}^{-\frac{31}{40}},\ \hat{Y}_{{\cal Z}_i{\cal Z}_i{\cal A}_4}\sim{\cal
  V}^{-\frac{143}{40}},\nonumber\\
& &\hat{Y}_{{\cal Z}_i{\cal Z}_i{\cal A}_3}\sim{\cal
  V}^{-\frac{107}{40}},\ \hat{Y}_{{\cal Z}_i{\cal A}_1{\cal
    A}_1}\sim{\cal
  V}^{-\frac{163}{40}},\  \hat{Y}_{{\cal Z}_i{\cal A}_1{\cal
    A}_2}\sim{\cal
  V}^{-\frac{23}{8}},\ \hat{Y}_{{\cal Z}_i{\cal A}_1{\cal
    A}_3}\sim{\cal
  V}^{-\frac{191}{40}},\nonumber\\
& & \hat{Y}_{{\cal Z}_i{\cal A}_1{\cal
    A}_4}\sim{\cal
  V}^{-\frac{227}{40}},\  \hat{Y}_{{\cal Z}_i{\cal A}_2{\cal A}_2}\sim{\cal
  V}^{-\frac{67}{40}},\ \hat{Y}_{{\cal Z}_i{\cal A}_2{\cal A}_3}\sim{\cal
  V}^{-\frac{143}{40}},\  \hat{Y}_{{\cal Z}_i{\cal A}_2{\cal A}_4}\sim{\cal
  V}^{-\frac{179}{40}}, \nonumber\\
& & \  \hat{Y}_{{\cal Z}_i{\cal A}_3{\cal A}_3}\sim{\cal
  V}^{-\frac{219}{40}},\ \hat{Y}_{{\cal Z}_i{\cal A}_3{\cal
    A}_4}\sim{\cal
  V}^{-\frac{51}{8}},\  \hat{Y}_{{\cal Z}_i{\cal A}_4{\cal
    A}_4}\sim{\cal
  V}^{-\frac{55}{8}},\ \hat{Y}_{{\cal A}_1{\cal A}_1{\cal
    A}_1}\sim{\cal V}^{-\frac{247}{40}},\nonumber\\
& & \hat{Y}_{{\cal A}_1{\cal A}_1{\cal A}_2}
\sim{\cal V}^{-\frac{199}{40}},\  \hat{Y}_{{\cal A}_1{\cal A}_1{\cal A}_3}
\sim{\cal V}^{-\frac{55}{8}},\  \hat{Y}_{{\cal A}_1{\cal A}_1{\cal A}_4}
\sim{\cal V}^{-\frac{311}{40}},\ \hat{Y}_{{\cal A}_1{\cal A}_2{\cal A}_2}\sim
\sim{\cal V}^{-\frac{151}{40}},\nonumber\\
& & \ \hat{Y}_{{\cal A}_1{\cal A}_2{\cal A}_3}
\sim{\cal V}^{-\frac{227}{40}},\ \hat{Y}_{{\cal A}_1{\cal A}_2{\cal A}_4}
\sim{\cal V}^{-\frac{263}{40}},\ \hat{Y}_{{\cal A}_2{\cal A}_4{\cal A}_5}
\sim{\cal V}^{-\frac{339}{40}},\   \hat{Y}_{{\cal A}_1{\cal A}_4{\cal A}_4}
\sim{\cal V}^{-\frac{75}{8}},\nonumber\\
& &\ \hat{Y}_{{\cal A}_2{\cal A}_2{\cal
    A}_2}\sim{\cal V}^{-\frac{103}{40}},\ \hat{Y}_{{\cal A}_2{\cal A}_2{\cal A}_3}
\sim{\cal V}^{-\frac{179}{40}},\  \hat{Y}_{{\cal A}_2{\cal A}_2{\cal A}_4}
\sim{\cal V}^{-\frac{43}{8}},\  \hat{Y}_{{\cal A}_2{\cal A}_3{\cal A}_3}
\sim{\cal V}^{-\frac{299}{60}},\nonumber\\
& &  \hat{Y}_{{\cal A}_2{\cal A}_3{\cal A}_4}
\sim{\cal V}^{-\frac{263}{40}},\  \hat{Y}_{{\cal A}_4{\cal A}_3{\cal A}_3}
\sim{\cal V}^{-\frac{367}{40}},\  \hat{Y}_{{\cal A}_1{\cal A}_3{\cal A}_3}
\sim{\cal V}^{-\frac{283}{40}},\ \hat{Y}_{{\cal A}_2{\cal A}_4{\cal A}_4}
\sim{\cal V}^{-\frac{327}{40}},\nonumber\\
& &   \hat{Y}_{{\cal A}_3{\cal A}_4{\cal A}_4}
\sim{\cal V}^{-\frac{403}{40}},\  \hat{Y}_{{\cal A}_3{\cal A}_3{\cal A}_3}
\sim{\cal V}^{-\frac{331}{40}},\ \hat{Y}_{{\cal A}_4{\cal A}_4{\cal A}_4}
\sim{\cal V}^{-\frac{439}{40}}.
\end{eqnarray}
From (\ref{eq:Yhats}), one sees that $\hat{Y}_{{\cal Z}_i{\cal
    Z}_i{\cal Z}_i}(M_s)\sim{\cal V}^{\frac{1}{8}}$ is the most
dominant physical Yukawa at the string scale. Hence,
\begin{equation}
\label{eq:anom_dimen-2}
\gamma_\Lambda^\Gamma\hat{Y}_{\Gamma\Sigma\Delta}\sim\frac{1}{32\pi^2}\hat{Y}_{\Lambda{\cal
  Z}_i{\cal Z}_i}\hat{Y}^*_{{\cal Z}_i{\cal Z}_i{\cal
  Z}_i}\hat{Y}_{{\cal Z}_i\Sigma\Delta}
-\frac{2\sum_{(a)}g_{(a)}^2C_{(a)}(\Phi_\Gamma)\delta_{\Lambda}^{\Gamma}\hat{Y}_{\Gamma\Sigma\Delta}}{32\pi^2}.
\end{equation}
Now, the first term in (\ref{eq:anom_dimen-2}) is volume suppressed as
compared to the second term at $M_s$; let us assume that the same will
be true up to the EW scale. Using the one-loop solution for
$\frac{g_{(a)}^2(t)}{16\pi^2}
=\frac{ \frac{\beta_{(a)}}{b_{(a)}}}{1 + \beta_{(a)}t}$ in
(\ref{eq:anom_dimen-2}) and therefore (\ref{eq:Yhat_RG-1}), one
obtains:
\begin{equation}
\label{eq:Yhat_sol_1}
\frac{d ln\hat{Y}_{\Lambda\Sigma\Delta}}{dt}\sim -2\left(\sum_{(a)}
\frac{C_{(a)}(\Lambda)\frac{\beta_{(a)}}{b_{(a)}}}{1 + \beta_{(a)}t}
+ \sum_{(a)}
\frac{C_{(a)}(\Sigma)\frac{\beta_{(a)}}{b_{(a)}}}{1 + \beta_{(a)}t} +
\sum_{(a)}
\frac{C_{(a)}(\Delta)\frac{\beta_{(a)}}{b_{(a)}}}{1 + \beta_{(a)}t}\right),
\end{equation}
whose solution yields:
\begin{equation}
\label{eq:Yhat_sol-2}
\hat{Y}_{\Lambda\Sigma\Delta}(t)\sim\hat{Y}_{\Lambda\Sigma\Delta}(M_s)
\prod_{(a)=1}^3\left(1 + \beta_{(a)}t\right)^{\frac{-2\left(C_{(a)}(\Lambda)
    +C_{(a)}(\Sigma) + C_{(a)}(\Delta)\right) }{b_{(a)}}}.
\end{equation}
The solution (\ref{eq:Yhat_sol-2}) justifies the assumption that all
$\hat{Y}_{\Lambda\Sigma\Delta}$s change only by ${\cal O}(1)$ as one
RG-flows down from the string to the EW scale. A similar argument for the RG-evolution of $\hat{Y}^{\rm eff}_{{\cal Z}_i{\cal A}_I{\cal A}_J}$s would proceed as follows. We will for definiteness and due to relevance to the preceding discussion on lepton and quark masses, consider $\frac{d\hat{Y}^{\rm eff}_{{\cal Z}_1{\cal A}_1{\cal A}_3}}{dt}$ and $\frac{d\hat{Y}^{\rm eff}_{{\cal Z}_1{\cal A}_2{\cal A}_4}}{dt}$. Now, 
\begin{equation}
 \frac{d\hat{Y}^{\rm eff}_{{\cal Z}_1{\cal A}_1{\cal A}_3}}{dt} = \gamma_{{\cal Z}_1}^\Lambda\hat{Y}^{\rm eff}_{\Lambda{\cal A}_1{\cal A}_3} + \gamma_{{\cal A}_1}^\Lambda\hat{Y}^{\rm eff}_{{\cal Z}_1\Lambda{\cal A}_3}
+ \gamma_{{\cal A}_3}^\Lambda\hat{Y}^{\rm eff}_{{\cal Z}_1{\cal A}_1\Lambda},
\end{equation}
 where $ \gamma_{{\cal Z}_1}^\Lambda\ni\hat{Y}_{{\cal Z}_1\Upsilon\Sigma}\hat{Y}^*_{\Lambda\Upsilon\Sigma}\sim
\hat{Y}_{{\cal Z}_1{\cal Z}_1{\cal Z}_1}\hat{Y}^*_{\Lambda{\cal Z}_1{\cal Z}_1}$, {etc.}, implying:
\begin{eqnarray}
\label{eq:Yeffzia1a3-III}
& & \frac{d\hat{Y}^{\rm eff}_{{\cal Z}_1{\cal A}_1{\cal A}_3}}{dt}\ni \hat{Y}_{{\cal Z}_1{\cal Z}_1{\cal Z}_1}\hat{Y}^*_{{\cal Z}_1{\cal Z}_1{\cal Z}_1}\hat{Y}^{\rm eff}_{{\cal Z}_1{\cal A}_1{\cal A}_3}
+ \hat{Y}_{{\cal Z}_1{\cal Z}_1{\cal Z}_1}\hat{Y}^*_{{\cal A}_1{\cal Z}_1{\cal Z}_1}\hat{Y}^{\rm eff}_{{\cal A}_1{\cal A}_1{\cal A}_3}\nonumber\\
& &
+ \hat{Y}_{{\cal Z}_1{\cal Z}_1{\cal Z}_1}\hat{Y}^*_{{\cal A}_2{\cal Z}_1{\cal Z}_1}\hat{Y}^{\rm eff}_{{\cal A}_2{\cal A}_1{\cal A}_3} \hat{Y}_{{\cal Z}_1{\cal Z}_1{\cal Z}_1}\hat{Y}^*_{{\cal A}_3{\cal Z}_1{\cal Z}_1}\hat{Y}^{\rm eff}_{{\cal A}_3{\cal A}_1{\cal A}_3}\hat{Y}_{{\cal Z}_1{\cal Z}_1{\cal Z}_1}\hat{Y}^*_{{\cal A}_4{\cal Z}_1{\cal Z}_1}\hat{Y}^{\rm eff}_{{\cal A}_4{\cal A}_1{\cal A}_3},
\end{eqnarray}
and a similar equation for $\frac{d\hat{Y}^{\rm eff}_{{\cal Z}_1{\cal A}_2{\cal A}_4}}{dt}$.
Using (\ref{eq:Yhats}) and:
\begin{eqnarray}
\label{eq:yeff_I or i a1a3 and a2a4}
& & e^{\frac{K}{2}}{\cal D}_{a_{1/2}}D_{a_{3/4}}W\ni {\cal V}^{-\frac{4}{9}}\left(z_i-{\cal V}^{\frac{1}{36}}\right) + {\cal V}^{\frac{2}{3}}\left(a_1-{\cal V}^{-\frac{2}{9}}\right)
+ {\cal V}^{-\frac{5}{6}}\left(a_2-{\cal V}^{-\frac{1}{3}}\right)\nonumber\\
& &  {\hskip 1.1in}+
{\cal V}^{\frac{1}{6}}\left(a_3-{\cal V}^{-\frac{13}{18}}\right)
+ {\cal V}^{\frac{7}{6}}\left(a_4-{\cal V}^{-\frac{11}{9}}\right),
\end{eqnarray}
and (\ref{eq:Yeffzia1a3-III}), one sees that at $M_s$:
\begin{eqnarray}
\label{eq:Yeffzia1a3+a2a4-IV}
& & \gamma_{{\cal Z}_1}^\Lambda\hat{Y}^{\rm eff}_{\Lambda{\cal A}_1{\cal A}_3} + \gamma_{{\cal A}_1}^\Lambda\hat{Y}^{\rm eff}_{{\cal Z}_1\Lambda{\cal A}_3}
+ \gamma_{{\cal A}_3}^\Lambda\hat{Y}^{\rm eff}_{{\cal Z}_1{\cal A}_1\Lambda}\ni \frac{{\cal V}^{\frac{1}{8}+\frac{1}{8} - \frac{4}{9}}}{\sqrt{K_{{\cal Z}_1\bar{\cal Z}_1}K_{{\cal A}_1\bar{\cal A}_1}K_{{\cal A}_3\bar{\cal A}_3}}}\Biggr|_{{\cal V}\sim10^5}\sim{\cal V}^{-\frac{143}{180}},\nonumber\\
& &  \gamma_{{\cal Z}_1}^\Lambda\hat{Y}^{\rm eff}_{\Lambda{\cal A}_2{\cal A}_4} + \gamma_{{\cal A}_2}^\Lambda\hat{Y}^{\rm eff}_{{\cal Z}_1\Lambda{\cal A}_4}
+ \gamma_{{\cal A}_4}^\Lambda\hat{Y}^{\rm eff}_{{\cal Z}_1{\cal A}_2\Lambda}\ni \frac{{\cal V}^{\frac{1}{8}+ \frac{1}{8} - \frac{4}{9}}}{\sqrt{K_{{\cal Z}_1\bar{\cal Z}_1}K_{{\cal A}_2\bar{\cal A}_2}K_{{\cal A}_4\bar{\cal A}_4}}}\Biggr|_{{\cal V}\sim10^5}\sim{\cal V}^{-\frac{25}{36}}.
\end{eqnarray}
Hence, at the string scale, the anomalous dimension matrix contribution is sub-dominant as compared to the gauge coupling-dependent contribution, and by a similar assumption (justified by the solution below)/reasoning:
\begin{equation}
\label{eq:Yeffhat_sol}
\hat{Y}^{\rm eff}_{\Lambda\Sigma\Delta}(t)\sim\hat{Y}^{\rm eff}_{\Lambda\Sigma\Delta}(M_s)
\prod_{(a)=1}^3\left(1 + \beta_{(a)}t\right)^{\frac{-2\left(C_{(a)}(\Lambda)
    +C_{(a)}(\Sigma) + C_{(a)}(\Delta)\right) }{b_{(a)}}}.
\end{equation}
This suggests that possibly, the fermionic superpartners of ${\cal A}_1$ and ${\cal A}_3$ correspond respectively to  $e_L$ and $e_R$ and the fermionic superpartners of ${\cal A}_2$ and ${\cal A}_4$ correspond respectively to the first generation $u_L$ and $u_R$, and ${\cal Z}_I (I=1,2)$ correspond to two Higgs doublets.\\
$~~~$For the purposes of evaluation of various interaction vertices needed to evaluate decay width of gluino in section {\bf 6}, N(LSP) decay channels as well as EDM of electron/neutron in the forthcoming chapters, we will be using the following terms (written out in four-component notation or their two-component analogs and utilizing/generalizing results of \cite{Jockers_thesis}) in the ${\cal N}=1$ gauged supergravity action of Wess and Bagger \cite{Wess_Bagger} with the understanding that $m_{{\rm moduli/modulini}}<<m_{\rm KK}\Bigl(\sim\frac{M_s}{{\cal V}^{\frac{1}{6}}}\Bigr|_{{\cal V}\sim10^{5}/10^{6}} $ $\sim10^{14}GeV\Bigr)$, $M_s=\frac{M_p}{\sqrt{{\cal V}}}\Biggr|_{{\cal V}\sim10^{5/6}}\sim10^{15}GeV$, and that for multiple $D7$-branes, the non-abelian gauged isometry group\footnote{As explained in  \cite{Jockers_thesis}, one of the two Pecci-Quinn/shift symmetries along the RR two-form axions $c^a$ and the four-form axion $\rho_B$ gets gauged due to the dualization of the Green-Schwarz term $\int_{{\bf R}^{1,3}}dD^{(2)}_B\wedge A$ coming from the KK reduction of the Chern-Simons term on $\Sigma_B\cup\sigma(\Sigma_B)$ - $D^{(2)}_B$ being an RR two-form axion. In the presence of fluxes (\ref{eq:flux}) for multiple $D7$-brane fluxes, the aforementioned Green-Schwarz is expected to be modified to $Tr\left(Q_B\int_{{\bf R}^{1,3}}dD^{(2)}_B\wedge A\right)$, which after dualization in turn modifies the covariant derivative of $T_B$ and hence the killing isometry.}, corresponding to the killing vector $6i\kappa_4^2\mu_7\left(2\pi\alpha^\prime\right)Q_B\partial_{T_B}, Q_B=\left(2\pi\alpha^\prime\right)\int_{\Sigma_B}i^*\omega_B\wedge P_-\tilde{f}$ arising due to the elimination of of the two-form axions $D_B^{(2)}$ in favor of the zero-form axions
$\rho_B$ under the KK-reduction of the ten-dimensional four-form axion \cite{Jockers_thesis} (which results in a modification of the covariant derivative of $T_B$ by an additive shift given by $6i\kappa_4^2\mu_7\left(2\pi\alpha^\prime\right)Tr(Q_B A_\mu)$)  can be identified with the SM group (i.e. $A_\mu$ is the SM-like adjoint-valued gauge field \cite{Wess_Bagger}):
\begin{eqnarray}
\label{eq:WB_gSUGRA N=1}
& & {\cal L} = g_{YM}g_{T_B {\bar{\cal J}}}Tr\left(X^{T_B}{\bar\chi}^{\bar{\cal J}}_L\lambda_{\tilde{g},\ R}\right)\nonumber\\
&& +ig_{{\cal I}\bar{\cal J}}Tr\Biggl({\bar\chi}^{\bar{\cal I}}_L\Bigl[\slashed{\partial}\chi^{\cal I}_L+\Gamma^i_{Mj}\slashed{\partial} a^M\chi^{\cal J}_L \frac{1}{4}\left(\partial_{a_M}K\slashed{\partial} a_M - {\rm c.c.}\right)\chi^{\cal I}_L\Bigr] \Biggr)\nonumber\\
&&
 +\frac{e^{\frac{K}{2}}}{2}\left({\cal D}_{\bar{\cal I}}D_{\cal J}\bar{W}\right)Tr\left(\chi^{\cal I}_L\chi^{\cal J}_R\right) + g_{T_B\bar{T}_B}Tr\left[\left(\partial_\mu T_B - A_\mu X^{T_B}\right)\left(\partial^\mu T_B - A^\mu X^{T_B}\right)^\dagger\right]  \nonumber\\
&&
+ g_{T_B{\cal J}}Tr\left(X^{T_B}A_\mu\bar{\chi}^{\cal J}_L\gamma^\nu\gamma^\mu\psi_{\nu,\ R}\right) + \bar{\psi}_{L,\ \mu}\sigma^{\rho\lambda}\gamma^\mu\lambda_{\tilde{g},\ L}F_{\rho\lambda} + \bar{\psi}_{L,\ \mu}\sigma^{\rho\lambda}\gamma^\mu\lambda_{\tilde{g},\ L}W^+_\rho W^-_\lambda\nonumber\\
 & & + Tr\left[\bar{\lambda}_{\tilde{g},\ L}\slashed{A}\left(6\kappa_4^2\mu_7(2\pi\alpha^\prime)Q_BK + \frac{12\kappa_4^2\mu_7(2\pi\alpha^\prime)Q_Bv^B}{\cal V}\right) \lambda_{\tilde{g},\ L}\right]\nonumber\\
 & & + \frac{e^K G^{T_B\bar{T}_B}}{\kappa_4^2}6i\kappa_4^2(2\pi\alpha^\prime)Tr\left[Q_BA^\mu\partial_\mu
 \left(\kappa_4^2\mu_7(2\pi\alpha^\prime)^2C^{I\bar{J}}a_I\bar{a}_{\bar J}\right)\right] -\frac{f_{ab}}{4}F^a_{\mu\nu}F^{b\ mu\nu}  \nonumber\\
 & &+ \frac{1}{8}f_{ab}\epsilon^{\mu\nu\rho\lambda}F^a_{\mu\nu}F^b_{\rho\lambda} - \frac{i\sqrt{2}}{4} g \partial_{i/I}f_{ab} Tr\left(\frac{12\kappa_4^2\mu_7(2\pi\alpha^\prime)Q_B^av^B}{\cal V}{\bar\lambda}_{\tilde{g},L}^b\chi^{i/I}_R\right) + {\rm h.c.}\nonumber\\
 & & - \frac{\sqrt{2}}{4}\partial_{i/I}f_{ab}Tr\left({\bar\lambda}_{\tilde{g},R}^a\sigma^{\mu\nu}\chi^{i/I}_L\right)F_{\mu\nu}^b + {\rm h.c.}.
\end{eqnarray}
To evaluate the contribution of various 3-point interaction vertices in context of ${\cal N}=1$ gauged supergravity defined above, one needs to evaluate the full moduli space metric in fluctuations linear in different kind of moduli corresponding to different SM particles. The expansion of moduli space metric, its inverse and derivatives w.r.t to each moduli in terms of fluctuations linear in $z_i\rightarrow z_1 + {\cal V}^\frac{1}{36}{M_p}, a_1\rightarrow a_1 + {\cal V}^{-\frac{2}{9}}{M_p},a_2\rightarrow a_2 + {\cal V}^-{\frac{1}{3}}{M_p}, a_3\rightarrow a_3 + {\cal V}^{-\frac{13}{18}}{M_p},a_3\rightarrow a_3 + {\cal V}^{-\frac{11}{9}}{M_p}$ are given in an appendix  of \cite{gravitino_DM}. 
%One can show that near (\ref{eq:near_slag_i}) along which $|z_1|$ and $|z_2|$ are on the same footing.
\vskip -0.5in
\section{Computation of Soft Terms}
We briefly describe evaluation of various soft supersymmetric as well as supersymmetry breaking parameters in the model involving four-Wilson line moduli. The various soft terms are calculated by power series expansion of  superpotential as well as K\"{a}hler potential,
\begin{eqnarray}
\label{eq:KWexp}
&& W= {\hat W}(\Phi) + \mu(\Phi) {\cal Z}_I {\cal Z}_{J}+ \frac{1}{6} Y_{IJK}(\Phi){\cal M}^{I}{\cal M}^{J} {\cal M}^{K}+...,\nonumber\\
 && K = {\hat K}(\Phi,\bar\Phi) + K_{I {\bar J}}(\Phi,\bar\Phi){\cal M}^{I}{\cal M}^{\bar J} + Z(\Phi,\bar\Phi){\cal M}^{I}{\cal M}^{\bar J}+....,
 \end{eqnarray}
where ${\cal M}^{I}=({\cal Z}^{I},{\cal A}^{I}).$
The soft SUSY breaking parameters are calculated by expanding ${\cal N}=1$ supergravity potential, $V= e^{K}\left(K^{I \bar J}D_{I}W D_{\bar J}{\bar W}- 3 \left|W\right|^2\right)$, in the powers of matter fields ${\cal M}^{I}$, after expanding superpotential as well as K\"{a}hler potential as according to equation (\ref{eq:KWexp}).
%in order to evaluate the gaugino masses,
In gravity-mediated supersymmetry breaking, SUSY gets spontaneously broken in bulk sector by giving a vacuum expectation value to auxiliary F-terms. Hence, to begin with, one needs to evaluate the bulk $F$-terms which in turn entails evaluating the bulk metric. Writing the K\"{a}hler sector of the K\"{a}hler potential as:
 \begin{eqnarray}
&& K\sim-2 ln\left[\left(\sigma_B + \bar{\sigma}_B - \gamma K_{\rm geom}\right)^{\frac{3}{2}} - \left(\sigma_S + \bar{\sigma}_S - \gamma K_{rm geom}\right)^{\frac{3}{2}}\right.\nonumber\\
  && \left. + \sum_{\beta\in H_2^-(CY_3)}n^0_\beta\sum_{(n,m)} cos\left( i n k\cdot(G - \bar{G})g_s + m k\cdot (G + \bar{G}) \right)\right],
  \end{eqnarray} 
  and working near $sin \left( i n k\cdot(G - \bar{G})g_s + m k\cdot (G + \bar{G}) \right)=0$ - corresponding to a local minimum - generates the following components of the bulk metric: 
 \begin{equation}G_{m\bar{n}}\sim
\left(\begin{array}{cccc} {\cal V}^{-\frac{37}{36}} & {\cal V}^{-\frac{59}{36}} & 0 & 0\\
{\cal V}^{-\frac{59}{36}} & {\cal V}^{-\frac{4}{3}} & 0 & 0 \\
0 & 0 & {\cal O}(1) & {\cal O}(1) \\
0 & 0 & {\cal O}(1) & {\cal O}(1)
\end{array}\right),
\end{equation}
which therefore produces the following inverse: 
\begin{equation}
G^{m\bar{n}}\sim\left(\begin{array}{cccc} {\cal V}^{\frac{37}{36}} & {\cal V}^{\frac{13}{18}} & 0 & 0 \\
{\cal V}^{\frac{13}{18}} & {\cal V}^{\frac{4}{3}} & 0 & 0 \\
0 & 0 & {\cal O}(1) & {\cal O}(1) \\
0 & 0 & {\cal O}(1) & {\cal O}(1)
\end{array}\right).
\end{equation}
After spontaneous SUSY breaking, the gravitino mass is given by:
\begin{equation}
m_{3/2}= e^{K}\left|W\right|^2\sim {\cal V}^{-\frac{n^s}{2}-1}M_p.
\end{equation}
 Given that bulk $F$-terms are defined as \cite{softsusy2}: $F^m=e^{\frac{K}{2}}G^{m\bar{n}}D_{\bar{n}}\bar{W}$, one obtains:
\begin{equation}
\label{eq:bulk_F}
F^{\sigma_S}\sim{\cal V}^{-\frac{n^s}{2} + \frac{1}{36}}M_p^2,\ F^{\sigma_B}\sim{\cal V}^{-\frac{n^s}{2} - \frac{5}{18}}M_p^2,\ F^{G^a}\sim{\cal V}^{-\frac{n^s}{2}-1}M_p^2,
\end{equation}
The gaugino mass is given as:
\begin{equation}
\label{eq:gaugino_mass}
m_{\tilde{g}}=\frac{F^m\partial_m T_B}{Re T_B}\lesssim{\cal V}^{\frac{2}{3}}m_{3/2}.
\end{equation}
The analytic form of scalar masses obtained via spontaneous symmetry breaking is given as \cite{softsusy2}: 
$m^{2}_{I}= (m^{2}_{\frac{3}{2}} +V_{0}) - F^{\bar m} F^{n} {\partial_{\bar m}}{\partial_n}\log K_{I {\bar I}}$.
These were calculated in \cite{gravitino_DM} to yield
\begin{equation}
\label{eq:mass_Zi}
m_{{\cal Z}_i}\sim {\cal V}^{\frac{59}{72}}m_{3/2}, m_{{\cal A}_1}\sim\sqrt{{\cal V}}m_{3/2},
\end{equation}
implying a universality in the open moduli masses.
 
Further in \cite{gravitino_DM}, we showed  that the universality in the trilinear $A$-couplings \cite{softsusy2},
\begin{equation}
\label{ew:A}
A_{{\cal I}{\cal J}{\cal K}}=F^m\left(\partial_mK + \partial_m ln Y_{{\cal I}{\cal J}{\cal K}}
+ \partial_m ln\left(K_{{\cal I}\bar{\cal I}}K_{{\cal J}\bar{\cal J}}K_{{\cal K}\bar{\cal K}}\right)\right),
\end{equation}
that was seen in the case of the $D3$-brane position moduli and a single Wilson line modulus in \cite{D3_D7_Misra_Shukla}, is preserved even for the current four-Wilson-line moduli setup and

\begin{equation}
\label{eq:A-univ}
A_{{\cal I}{\cal J}{\cal K}}\sim{\cal V}^{\frac{37}{36}}m_{3/2}\sim\hat{\mu}_{{\cal Z}_1{\cal Z}_2}.
\end{equation}
The physical higgsino mass parameter $\hat{\mu}_{{\cal Z}_1{\cal Z}_2}$ turned out to be given by:
\begin{equation}
\label{eq:muhat_Z1Z2}
\hat{\mu}_{{\cal Z}_1{\cal Z}_2}=\frac{e^{\frac{K}{2}}\mu_{{\cal Z}_1{\cal Z}_2}}{\sqrt{K_{{\cal Z}_1\bar{\cal Z}_1}K_{{\cal Z}_2\bar{\cal Z}_2}}}\sim{\cal V}^{\frac{19}{18}}m_{3/2}.
\end{equation}
 Further,
\begin{eqnarray}
\label{eq:muhatB_Z1Z2}
& & \left(\hat{\mu}B\right)_{{\cal Z}_1{\cal Z}_2}=\frac{e^{-i arg(W)+\frac{K}{2}}}{\sqrt{K_{{\cal Z}_1\bar{\cal Z}_1}K_{{\cal Z}_2\bar{\cal Z}_2}}}F^m\left(\partial_mK \mu_{{\cal Z}_1{\cal Z}_2} + \partial_m\mu_{{\cal Z}_1{\cal Z}_2} - \mu_{{\cal Z}_1{\cal Z}_2}\partial_m ln\left(K_{{\cal Z}_1\bar{\cal Z}_1}K_{{\cal Z}_2\bar{\cal Z}_2}\right)\right)\nonumber\\
& &  \sim\hat{\mu}_{{\cal Z}_1{\cal Z}_2}\left(F^m\partial_mK+F^{\sigma_S} - F^m\partial_m ln\left(K_{{\cal Z}_1\bar{\cal Z}_1}K_{{\cal Z}_2\bar{\cal Z}_2}\right)\right) \sim{\cal V}^{\frac{19}{18}+\frac{37}{36}}m^2_{3/2}\sim\hat{\mu}^2_{{\cal Z}_1{\cal Z}_2},
\end{eqnarray}
an observation which will be very useful in obtaining a light Higgs of mass $125 \ GeV$.
\section{Realizing Large Volume $\mu$-split SUSY}
In the previous section, we calculated masses of position moduli which we have identified with Higgs doublets as according to the argument given below equation (\ref{eq:Yeffhat_sol}) at string scale. In order to obtain the possibility of getting a light Higgs at electroweak scale using the fine-tuning argument of \cite{HamidSplitSUSY}, in this section, we first analyse the contribution of masses of Higgs doublets obtained after SUSY breaking at electroweak scale.  The Higgs doublets are defined as:
\beqn
\label{massmat}
&& H_{1}=D_{h_{11}} H_{u} +D_{h_{12}}H_{d}, H_{2}=D_{h_{21}}H_{u} +D_{h_{22}} H_{d}.
\eeqn
where $D_h=\left(\begin{array}{ccccccc}
\cos \frac{\theta_h}{2} & -\sin \frac{\theta_h}{2} e^{-i\phi_{h}}\\
\sin \frac{\theta_h}{2} e^{i\phi_{h}} & \cos \frac{\theta_h}{2}
 \end{array} \right),
D_{h}^\dagger M_{h}^2 D_h={\rm diag}(M^{2}_{H_1},M^{2}_{H_2})$, 
and $\tan \theta_h=
\frac{2|M_{h_{21}}^2|}{M_{h_{11}}^2-M_{h_{22}}^2}$ for a particular range of ${{-\pi}\over {2}} \leq  \theta_h \leq {{\pi}\over {2}}$.

The Higgs masses after soft supersymmetry breaking is given by $(m_{Z_i}^{2}+\hat{\mu}_{Z_i}^{2})^{1/2}$ (where $m_{Z_i}$'s correspond to  mobile $D3$- Brane position moduli masses (to be identified with soft Higgs scalar mass parameter)) and the Higgsino mass is given by  $\hat{\mu}_{Z_i}$. However, due to lack of universality in moduli masses but universality in trilinear $A_{ijk}$ couplings, we use solution of RG flow equation for moduli masses as given in \cite{Nath+Arnowitt}. Using the same,
\begin{equation}
\label{eq:heavy_H_I}
m_{{\cal Z}_{1}}^{2}(t)=m_{o}^{2}(1+\delta_1)+m_{1/2}^{2} g(t)+\frac{3}{5}S_0p,
\end{equation}
where  
\begin{equation}
S_0=Tr(Ym^2)=m_{{\cal Z}_2}^2-m_{{\cal Z}_1}^2+\sum_{i=1}^{n_g}(m_{\tilde q_L}^2-2
m_{\tilde u_R}^2 +m_{\tilde d_R}^2 - m_{\tilde l_L}^2 + m_{\tilde e_R}^2),
\end{equation} where all the masses are at the string scale and
 $n_g$ is the number of generations. $p$ is defined by
%\begin{equation}
%\label{eq:p_def}
$p=\frac{5}{66}[1-(\frac{\tilde\alpha_1(t)}
{\tilde\alpha_1(M_s)})]$
%\end{equation}
where  $\tilde\alpha_1\equiv g_1^2/(4\pi)^2$ and  $g_1$ is the
$U(1)_Y$ gauge coupling constant. Further,
\begin{equation}
\label{eq:light_H_I}
 m_{{\cal Z}_{2}}^{2}(t) = m_0^2\Delta_{{\cal Z}_2} + m_{1/2}^{2}e(t) + A_{o}m_{1/2}f(t) + m_{o}^{2}h(t) -k(t)A_{o}^{2} - \frac{3}{5}S_0p,
\end{equation}
where $\Delta_{{\cal Z}_2}$ is given by $\Delta_{{\cal Z}_2}=\frac{(D_0-1)}{2}(\delta_2+\delta_3+\delta_4)+ \delta_2;  D_0=1-6 {\cal Y}_t \frac{F(t)}{E(t)}$.
 Here ${\cal Y}_t\equiv\hat{Y}_t^2(M_s)/(4\pi)^2$ where $\hat{Y}_t(M_s)$ is the physical top Yukawa coupling at the string scale which following \cite{Ibanez_et_al} will be set to 0.08, and $E(t)=(1+\beta_3t)^{\frac{16}{3b_3}}(1+\beta_2t)^{\frac{3}{b_2}}
(1+\beta_1t)^{\frac{13}{9b_1}}$.
   $\beta_i\equiv\alpha_i(M_s)b_i/4\pi$
($\alpha_1=(5/3)\alpha_Y$), $b_i$ are
the one loop
beta function coefficients defined  by $(b_1,b_2,b_3)=
(33/5,1,-3)$,
and $F(t)=\int_0^t E(t)dt$.

In the dilute flux approximation,
$g_1^2(M_S)=g_2^2(M_S)=g_3^2(M_S)$. To ensure $E(t)\in\bf{R}$, the $SU(3)$-valued $1+\beta_3t >0$, which for $t=57$ implies that $g_3^2(M_s)<\frac{(4\pi)^2}{3\times57}\sim{\cal O}(1)$. Hence,  $g_3^2(M_s)=0.4$ is what we will be using (see \cite{Dhuria+Misra_mu_Split_SUSY}). From (\ref{eq:heavy_H_I}) and (\ref{eq:light_H_I}), the results of scalar masses as given in section {\bf 3}, and the values of t-dependent functions given in an appendix of \cite{Dhuria+Misra_mu_Split_SUSY}, one sees that:
\begin{eqnarray}
\label{eq:heavy_H_II}
 && m_{{\cal Z}_1}^2(M_{EW})\sim m_{{\cal Z}_1}^2(M_s)+{(0.39)}{\cal V}^{\frac{4}{3}}m_{3/2}^2+\frac{1}{22}\times\frac{19\pi}{100}\times S_0,\\
\label{eq:light_H_II}
&&m_{{\cal Z}_2}^2(M_{EW})\sim  {(0.32)}{\cal V}^{\frac{4}{3}}m_{3/2}^2+{(-0.03)}n^s\hat{\mu}_{{\cal Z}_1{\cal Z}_2}{\cal V}^{\frac{2}{3}}m_{3/2}\nonumber\\
&&+{(0.96)} m_0^2-{(0.01)}(n^s)^2\hat{\mu}_{{\cal Z}_1{\cal Z}_2} -\frac{19\pi}{2200}\times S_0,
\end{eqnarray}
where we used $A_{{\cal Z}_i{\cal Z}_i{\cal Z}_i}\sim n^s\hat{\mu}_{{\cal Z}_1{\cal Z}_2}$ (\ref{eq:A-univ}).
The solution for RG flow equation for $\hat{\mu}^2$ to one loop order is given by \cite{Nath+Arnowitt}:
\begin{eqnarray}
\label{eq:muhat_I}
& &{\hskip -0.4in} \hat{\mu}^2_{{\cal Z}_i{\cal Z}_i}=-\left[m_0^2 C_1+A_0^2 C_2 +m_{\frac{1}{2}}^2C_3+m_{\frac{1}{2}}
A_0C_4-\frac{1}{2}M_Z^2 +\frac{19\pi}{2200}\left(\frac{tan^2\beta+1}{tan^2\beta-1}\right)S_0\right],
\end{eqnarray}
  wherein $C_1=\frac{1}{tan^2\beta-1}(1-\frac{3 D_0-1}{2}tan^2\beta) + 
\frac{1}{tan^2\beta-1}\Bigl(\delta_1-\delta_2tan^2\beta - \frac{ D_0-1}{2}(\delta_2 +
\delta_3+\delta_4)tan^2\beta\Bigr)$, $C_2=-\frac{tan^2\beta}{tan^2\beta-1}k(t),  C_3=-\frac{1}{tan^2\beta-1}\left(g(t)- tan^2\beta e(t)\right),~C_4=-\frac{tan^2\beta}{tan^2\beta-1}f(t)$, and the functions $e(t),f(t),g(t),k(t)$ are defined
in an appendix of \cite{Dhuria+Misra_mu_Split_SUSY}.  In the large $tan\beta$ (but less than 50)-limit, one sees that:
\begin{eqnarray}
\label{eq:muhat_II}
&& \hat{\mu}_{{\cal Z}_1{\cal Z}_2}^2\sim-\Bigl[-m_0^2-{(0.01)}(n^s)^2\hat{\mu}_{{\cal Z}_1{\cal Z}_2}^2+{(0.32)}{\cal V}^{\frac{4}{3}}m_{3/2}^2-1/2 M_{EW}^2\nonumber\\
&&+{(0.03)}{\cal V}^{\frac{2}{3}}n^s\hat{\mu}_{{\cal Z}_1{\cal Z}_2}m_{3/2} +\frac{19\pi}{2200}S_0\Bigr].
\end{eqnarray}
From (\ref{eq:light_H_II}) and (\ref{eq:muhat_II}), one therefore sees that the mass-squared of one of the two Higgs doublets, $m_{H_d}^2$, at the $EW$ scale is given by:
\begin{equation}
\label{eq:muhat_III}
  m^2_{H_d}=m^2_{{\cal Z}_2}+\hat{\mu}^2_{{\cal Z}_i{\cal Z}_i}= 2m^2_{0}-{(0.06)}{\cal V}^{\frac{2}{3}}n^s\hat{\mu}_{{\cal Z}_1{\cal Z}_2}m_{3/2}+\frac{1}{2}M_{EW}^2-\frac{19\pi}{1100}S_0.
\end{equation}
From \cite{D3_D7_Misra_Shukla}, we notice, ${\cal V}^{\frac{2}{3}}\hat{\mu}_{{\cal Z}_1{\cal Z}_2}m_{3/2}\sim m_0^2$, using which in (\ref{eq:muhat_III}), one sees that for an ${\cal O}(1)\ n^s$,
\begin{equation}
\label{eq:muhat_IV}
m^2_{H_d}(M_{EW})\sim  1.94 m_0^2 + \frac{1}{2}M_{EW}^2-\frac{19\pi}{1100}S_0.
\end{equation}
We have assumed at $ m^2_{{\cal Z}_2}(M_s)\sim m^2_0$ (implying $\delta_2=0$ but $ \delta_{1,3,4}\neq0$). 
  Further,
\begin{eqnarray}
\label{eq:heavy_Higgs}
& & m^2_{H_u}(M_{EW})=\left(m^2_{{\cal Z}_1}+\hat{\mu}_{{\cal Z}_1{\cal Z}_2}^2\right)(M_{EW})
 \sim m^2_{{\cal Z}_1}(M_s)(1+ \delta_1)+\frac{1}{2}M_{EW}^2 + m_0^2 \nonumber\\
  & & {\hskip 0.8in} -{(0.03)}{\cal V}^{\frac{2}{3}}n^s\hat{\mu}_{{\cal Z}_1{\cal Z}_2}m_{3/2}+ {(0.01)}(n^s)^2\hat{\mu}_{{\cal Z}_1{\cal Z}_2}^2  \nonumber\\
  & & {\hskip 0.8in} \sim (1.97+ \delta_1) m^2_0 +\frac{1}{2}M_{EW}^2 + {(0.01)}(n^s)^2\hat{\mu}_{{\cal Z}_1{\cal Z}_2}^2.
\end{eqnarray}
 By assuming $\left(\hat{\mu}B\right)_{{\cal Z}_1{\cal Z}_2}\sim\hat{\mu}^2_{{\cal Z}_1{\cal Z}_2}$ - see (\ref{eq:muhatB_Z1Z2}) -  to be valid at the string and EW scales, the Higgs mass matrix at the $EW$-scale can thus be expressed as:
\begin{eqnarray}
\label{eq:Higss_mass_matrix}
& & \left(\begin{array}{cc}
m^2_{H_u} & \hat{\mu}B\\
\hat{\mu}B & m^2_{H_d}\end{array}\right) \sim\left(\begin{array}{cc}
m^2_{H_u} & \xi\hat{\mu}^2\\
\xi\hat{\mu}^2 & m^2_{H_d}
\end{array}\right),
\end{eqnarray}
$\xi$ being an appropriately chosen ${\cal O}(1)$ constant - see (\ref{eq:evs_3}). The eigenvalues are given by $ \frac{1}{2}\biggl(m^2_{H_u}+m^2_{H_d}\pm\sqrt{\left(m^2_{H_u}-m^2_{H_d}\right)^2+4\xi^2\hat{\mu}^4}\biggr).$
Using equation (\ref{eq:muhat_II}), for $\delta_1 ={\cal O}(0.1)$ and ${\cal O}(1)\ n^s$, we have
\vskip -0.4in
\begin{eqnarray}
\label{eq:evs_1}
& & m^2_{H_u}+m^2_{H_d}\sim   m_0^2-0.06S_0+...  \, m^2_{H_u}-m^2_{H_d}\sim  m_0^2+0.06S_0+... \ ,\nonumber\\
& & \hat{\mu}_{{\cal H}_u{\cal H}_d}^2\sim   m_0^2 -0.03S_0+... 
\end{eqnarray}
\vskip -0.2in
Utilizing above, one sees that the eigenvalues are:
\begin{eqnarray}
\label{eq:evs_2}
& {\hskip -0.4in}m^2_{H_{1,2}}= m_0^2 -0.06S_0+.... &\pm\sqrt{\left(  m_0^2 +0.06S_0+...\right)^2+4\xi^2\left(m_0^2- 0.03S_0\right)^2}. 
\end{eqnarray}
 Considering 
 \begin{equation}
 \label{eq:evs_3}
 S_0\sim (-4.23) m_0^2, {\rm and}~~ \xi^2 \sim  {\frac{1}{5}} + \frac{1}{16}\frac{m^2_{EW}}{m_0^2},
 \end{equation}
  translates into getting  a light Higgs (corresponding to the negative sign of the square root) of the order $125 \ GeV$ and both heavy Higgs (corresponding to the positive sign of the square root) and higgsino mass parameter $\hat\mu$ of the order ${\cal V}^{\frac{59}{72}}m_{\frac{3}{2}}$.  This shows the possibility of realizing  ``$\mu$-split SUSY" scenario in the context of LVS phenomenology named as ``Large Volume $\mu$-split SUSY" scenario.
  \vskip -0.5in
 \section{Neutralino/Chargino Mass Matrix}
 In this section we work out the eigenalues and eigenvectors of the neutralino (chargino) mass matrix  
 formed by mixing neutral (charged) gaugino and neutral (charged) higgsino after electroweak symmetry breaking. In ${\cal N}=1$ gauged supergravity, the interaction vertex corresponding to Higgs-gaugino-higgsino term is given by ${\cal L}= g_{YM}g_{T^B{\cal Z}^i}X^B\tilde{H}^i\lambda^{i} + \partial_{{\cal Z}_i}T_B D^{B}\tilde{H}^i\lambda^{i} $ where $\lambda^{i}$ corresponds to gaugino (such as the Bino/Wino). Expanding the same in the fluctuations linear in $Z_i$, we have
\begin{equation}
\label{eq:gYM_ReT_II}
g_{YM}g_{T^B{\cal Z}^i}X^{B}= {\tilde f} {\cal V}^{-2}\frac{{\cal Z}_i}{M_p}, (\partial_{{\cal Z}_i}T_B) D^{B}\sim   {\tilde f} {\cal V}^{-\frac{4}{3}}\frac{{\cal Z}_i}{M_p}
\end{equation}
After giving a VEV to ${\cal Z}_i$, the interaction vertex corresponding to mixing between gaugino and higgsino will be given as:
\begin{equation}
\label{eq:gYM_ReT_II}
C^{\tilde \lambda^{+}-{{\tilde H}^{-}_{d}}}/C^{\tilde \lambda^{-}-{{\tilde H}^{+}_{u}}}/C^{\tilde \lambda^{0}-{{\tilde H}^{0}_{u}}/{\tilde H}^{0}_{d}}=\frac{ {\tilde f} {\cal V}^{-\frac{4}{3}}}{\sqrt{K_{{\cal Z}_i {\cal Z}_i}K_{{\cal Z}_i {\cal Z}_i}}}\sim   {\tilde f} {\cal V}^{-\frac{1}{3}}\frac{v}{M_p},{\rm where}~v=246~GeV.
\end{equation}
Using value of  $M_{{\tilde \lambda}^{0}} = {\cal V}^{\frac{2}{3}} m_{\frac{3}{2}}$, $M_{{{\tilde H}^{0}}_u/{{\tilde H}^{0}}_d}= {\cal V}^{\frac{59}{72}}m_{\frac{3}{2}}$ and $m_{\frac{3}{2}}= {\cal V}^{-2}M_p$  at electroweak scale,  yields a neutralino mass matrix\footnote{We keep both neutral gaugino (Wino as well as Bino) at the same footing, hence consider $3\times 3$ neutralino mass matrix.}:
\begin{eqnarray}
\label{eq:neut_mass}
& & \left(\begin{array}{ccc}
  {\cal V}^{-\frac{4}{3}}  &  \left(\frac{v}{M_p}\right) {\tilde f}{\cal V}^{-\frac{1}{3}} &  \left(\frac{v}{M_p}\right) {\tilde f}{\cal V}^{-\frac{1}{3}}\\
- \left(\frac{v}{M_p}\right) {\tilde f}{\cal V}^{-\frac{1}{3}}& 0 & {\cal V}^{-\frac{85}{72}}\\
- \left(\frac{v}{M_p}\right) {\tilde f}{\cal V}^{-\frac{1}{3}}& {\cal V}^{-\frac{85}{72}} & 0
\end{array}\right)M_p,
\end{eqnarray}
with eigenvalues:
\begin{eqnarray}
\label{eq:neut evalues}
& & \Biggl\{\frac{1}{V^{85/72}}, \frac{  {\cal V}^{4/3}- {\cal V}^{85/72}+\sqrt{  {\cal V}^{8/3}-2  {\cal V}^{181/72}+ {\cal V}^{85/36}+4 {\tilde f}^2  v^2 {\cal V}^{109/36}}}{2
   V^{157/72}},\nonumber\\
& &  \frac{ {\cal V}^{4/3}+ {\cal V}^{85/72}+\sqrt{  {\cal V}^{8/3}-2   {\cal V}^{181/72}+ {\cal V}^{85/36}+4 {\tilde f}^2  v^2 {\cal V}^{109/36}}}{2
  {\cal V}^{157/72}}\Biggr\}M_p
\end{eqnarray}
and normalized eigenvectors:
\begin{eqnarray}
\label{eq:neutralinos_i}
& & \tilde{\chi}_1^0\sim\frac{-{\tilde H}^{0}_{u}+{\tilde H}^{0}_{d}}{\sqrt{2}},~ {\rm and}~m_{{\tilde \chi}^{0}_{1}}\sim {\cal V}^{\frac{59}{72}}m_{\frac{3}{2}},\nonumber\\
& & \tilde{\chi}_2^0\sim \left(\frac{v}{  M_p}{\tilde f}{\cal V}^{\frac{5}{6}}\right){\tilde \lambda}^0+\frac{{\tilde H}^{0}_{u}+{\tilde H}^{0}_{d}}{\sqrt{2}}~ {\rm and}~m_{{\tilde \chi}^{0}_{2}}\sim {\cal V}^{\frac{59}{72}}m_{\frac{3}{2}};\ CP:-,\nonumber\\
& & \tilde{\chi}_3^0\sim-{\tilde \lambda}^0+\left(\frac{v}{M_p}{\tilde f}{\cal V}^{\frac{5}{6}}\right)\left({\tilde H}^{0}_{u}+{\tilde H}^{0}_{d}\right)~ {\rm and}~m_{{\tilde \chi}^{0}_{3}}\sim {\cal V}^{\frac{2}{3}}m_{\frac{3}{2}}.
\end{eqnarray}
For  higgsino-doublets
${\tilde H_u}=\left({\tilde H}^{0}_u , {\tilde H}^{+}_u \right), {\tilde H}_d=\left({\tilde H}^{-}_d, {\tilde H}^{0}_d \right)$,
the chargino mass matrix is given as:
\begin{equation}
 M_{{\tilde \chi}^{-}}=\left(\begin{array}{ccccccc}
  M^{2}_{{\tilde H}^{-}_{d}} & C^{\tilde \lambda^{-}-{{\tilde H}^{-}_{d}}}\\
C^{\tilde \lambda^{-}-{{\tilde H}^{-}_{d}}} &  M^{2}_{{\tilde \lambda}^{-}}
 \end{array} \right),  M_{{\tilde \chi}^{+}}=\left(\begin{array}{ccccccc}
  M^{2}_{{\tilde H}^{+}_{u}} & C^{\tilde \lambda^{+}-{{\tilde H}^{+}_{u}}}\\
C^{\tilde \lambda^{+}-{{\tilde H}^{+}_{u}}} &  M^{2}_{{\tilde \lambda}^{+}}
 \end{array} \right)
\end{equation}
Incorporating value of  $M_{{\tilde \lambda}^{+}}=M_{{\tilde \lambda}^{-}}= {\cal V}^{\frac{2}{3}} m_{\frac{3}{2}}$, $M_{{{\tilde H}^{-}}_{d}}=  M_{{{\tilde H}^{+}}_{u}}= {\cal V}^{\frac{59}{72}}m_{\frac{3}{2}}$ and $m_{\frac{3}{2}}= {\cal V}^{-2}M_p$  at electroweak scale, we have
\begin{equation}
 M_{{\tilde \chi}^{\pm}}=\left(\begin{array}{ccccccc}
  {\cal V}^{-\frac{4}{3}} & \left(\frac{v}{M_p}\right) {\tilde f}{\cal V}^{-\frac{1}{3}}\\
\left( \frac{v}{M_p}\right){\tilde f}{\cal V}^{-\frac{1}{3}}  &V^{-\frac{85}{72}}
 \end{array} \right)M_p,
\end{equation}
giving eigenvalues:
\begin{eqnarray}
\label{eq:charginoevalues}
& & \Biggl\{\frac{  {\cal V}^{4/3}+ {\cal V}^{85/72}-\sqrt{  {\cal V}^{8/3}-2  {\cal V}^{181/72}+ {\cal V}^{85/36}+4 {\tilde f}^2  v^2 {\cal V}^{109/36}}}{2
   V^{157/72}},\nonumber\\
& & \frac{ {\cal V}^{4/3}+ {\cal V}^{85/72}+\sqrt{  {\cal V}^{8/3}-2   {\cal V}^{181/72}+ {\cal V}^{85/36}+4 {\tilde f}^2  v^2 {\cal V}^{109/36}}}{2
  {\cal V}^{157/72}}\Biggr\}M_p,  \end{eqnarray}
and normalized eigenvectors:
\begin{eqnarray}
\label{eq:charginoI}
&& {\tilde \chi}^{+}_{1}= -{\tilde H}^{+}_{u}+\left(\frac{v}{M_p}{\tilde f}{\cal V}^{\frac{5}{6}}\right){\tilde \lambda}^{+}_{i},{\tilde \chi}^{-}_{1}=  -{\tilde H}^{-}_{d}+\left(\frac{v}{M_p}{\tilde f}{\cal V}^{\frac{5}{6}}\right){\tilde \lambda}^{-}_{i},~ {\rm and}~m_{{\tilde \chi}^{\pm}_{1}}\sim {\cal V}^{\frac{59}{72}}m_{\frac{3}{2}}\nonumber\\
&&  {\tilde \chi}^{+}_{2}= {\tilde \lambda}^{+}_{i} +\left(\frac{v}{M_p}{\tilde f}{\cal V}^{\frac{5}{6}}\right){\tilde H}^{+}_{u},{\tilde \chi}^{-}_{2}= {\tilde \lambda}^{-}_{i} +\left(\frac{v}{M_p}{\tilde f}{\cal V}^{\frac{5}{6}}\right) {\tilde H}^{-}_{d},~ {\rm and}~m_{{\tilde \chi}^{\pm}_{2}}\sim {\cal V}^{\frac{2}{3}}m_{\frac{3}{2}}.
\end{eqnarray}
The results of mass scales of all SM as well as superpartners are summarized in Table \ref{table:mass scales}.
 \begin{table}[htbp]
\centering
\begin{tabular}{|l|l|} \hline
Quark mass & $ M_{q}\sim O(10) MeV $\\
Lepton mass & $ M_{l}\sim {\cal O}(1) MeV $\\  \hline
Gravitino mass &  $ m_{\frac{3}{2}}\sim{\cal V}^{-\frac{n^s}{2} - 1}m_{pl}; n_s=2$ \\
Gaugino mass & $ M_{\tilde g}\sim  {\cal V}^{\frac{2}{3}}m_{\frac{3}{2}}$\\
(Lightest) Neutralino/Chargino & $ M_{{\chi^0_3}/{\chi^{\pm}_3}}\sim {\cal V}^{\frac{2}{3}}m_{\frac{3}{2}}$\\  
mass & \\
\hline
$D3$-brane position moduli  & $ m_{{\cal Z}_i}\sim {\cal V}^{\frac{59}{72}}m_{\frac{3}{2}}$ \\
(Higgs) mass & \\
Wilson line moduli & $ m_{\tilde{\cal A}_I}\sim {\cal V}^{\frac{1}{2}}m_{\frac{3}{2}}$\\
(sfermion mass ) & ${I =1,2,3,4}$\\ \hline
%& $A_{{\cal Z}_i{\cal Z}_j{\cal Z}_k}\sim n^s{\cal V}^{\frac{37}{36}}m_{\frac{3}{2}}$\\
A-terms & $A_{pqr}\sim n^s{\cal V}^{\frac{37}{36}}m_{\frac{3}{2}}$\\
& $\{p,q,r\} \in \{{{\tilde{\cal A}_I}},{{\cal Z}_i}\}$\\ \hline
Physical $\mu$-terms & $\hat{\mu}_{{\cal Z}_i{\cal Z}_j}$ \\
 (Higgsino mass) & $\sim{\cal V}^{\frac{37}{36}}m_{\frac{3}{2}}$ \\ \hline
Physical $\hat{\mu}B$-terms & $\left(\hat{\mu}B\right)_{{\cal Z}_1{\cal Z}_2}\sim{\cal V}^{\frac{37}{18}}m_{\frac{3}{2}}^2$\\ \hline
\end{tabular}
\caption{Mass scales of first generation of SM as well supersymmetric, and soft SUSY breaking parameters}
\label{table:mass scales}
\end{table}
\vskip -0.5in
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Gluino Decays}
One of the other striking feature of $\mu$-split SUSY scenario is based on longevity of gluinos
since the squarks which mediate its decay are ultra-heavy. In this spirit, we estimate the gluino decay life time at tree-level as well as one-loop level in the context of ${\cal N}=1$ gauged supergravity limit of  our ``local large volume $D3/D7$ model". Since squarks are heavier than gluino, two-body decays of gluino into squarks and quarks are kinematically forbidden at tree-level.  

 \underline{${\bf \tilde{g}\rightarrow q \ {\bar q} \ \chi^{0}_n}$}
 
We first discuss gluino three-body decays that involve the process like $\tilde{g}\rightarrow q{\bar q}\chi^{0}_n$ - $\tilde{g}$ being a gaugino, $q/{\bar q}$ being quark/anti-quark and $\chi_n$ being a neutralino. More specifically, e.g., the gluino decays into an anti-quark and an off-shell squark and the off-shell squark decays into a quark and neutralino. The eigenvalues as well as eigenvectors of neutralino are evaluated in section {\bf 5}. For gluino-decay studies, it is $\tilde{\chi}_3^0$ - largely a gaugino $\lambda^0$ with a small admixture of the higgsinos - which will be relevant. For squark-quark-neutralino vertex, we will work out squark-quark-gaugino vertex and also the squark-quark-higgsino vertex, and then add these contributions.
\begin{figure}
 \begin{center}
\begin{picture}(300,170)(50,0)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\Text(90,130)[]{$\tilde{g}$}
%\ArrowLine(110,120)(160,120)
\Line(60,120)(110,120)
\Gluon(60,120)(110,120){5}{4}
\ArrowLine(110,120)(140,150)
\Text(147,150)[]{${q}_I$}
\DashArrowLine (130,90)(110,120){4}
\Text(107,100)[]{$\tilde{q}_i$}
\ArrowLine(160,120)(130,90)
\Text(167,120)[]{${\bar q_J}$}
\ArrowLine(130,90)(160,60)
\Text(167,65)[]{$\tilde{\chi}_3^0$}
\Text(110,30)[]{(a)}
%%%%%%%%%%%%%%%%%%%%%%
\Text(250,130)[]{$\tilde{g}$}
\Line(210,120)(260,120)
\Gluon(210,120)(260,120){5}{4}
\ArrowLine(290,150)(260,120)
\Text(297,150)[]{$\bar{q}_J$}
\DashArrowLine(260,120)(280,90){4}{}
\Text(257,100)[]{$\tilde{q}_j$}
\ArrowLine(280,90)(310,120)
\Text(320,120)[]{${q}_I$}
\ArrowLine(310,60)(280,90)
\Text(317,65)[]{$\tilde{\chi}_3^0$}
\Text(280,30)[]{(b)}
%%%%%%%%%%%%%%%%%%%%%%%%%
\end{picture}
\end{center}
\vskip-0.5in
\caption{Three-body gluino decay diagrams}
\label{fig:treegdec}
\end{figure}
To calculate the contribution of various interaction vertices shown in Figure~\ref{fig:treegdec} in the context of ${\cal N}=1$ gauged supergravity, one needs to consider the following terms of gauged supergravity action  of Wess and Bagger \cite{Wess_Bagger}.
\begin{eqnarray}
\label{eq:fermion+fermion+sfermion}
& & {\hskip -0.3in}{\cal L} = g_{YM}g_{\alpha {\bar J}}X^\alpha{\bar\chi}^{\bar J}\tilde{\lambda^{0}}+ig_{i{\bar J}}{\bar\chi}^{\bar J}\left[{\bar\sigma}\cdot\partial\chi^i+\Gamma^i_{Lk}{\bar\sigma}\cdot\partial a^L\chi^k
+\frac{1}{4}\left(\partial_{a_L}K{\bar\sigma}\cdot a_L - {\rm c.c.}\right)\chi^i\right] \nonumber\\
& & {\hskip -0.3in}+\frac{e^{\frac{K}{2}}}{2}\left({\cal D}_iD_JW\right)\chi^i\chi^J+{\rm h.c.},
\end{eqnarray}
where, $X^\alpha$ corresponds to the components of a killing isometry vector. From here, one notes that $X^\alpha=-6i\kappa_4^2\mu_7Q_\alpha$, where $\alpha=B, Q_\alpha=2\pi\alpha^\prime\int_{T_B}i^*\omega_\alpha\wedge P_-\tilde{f}$ where $P_-$ is a harmonic zero-form on $\Sigma_B$ taking value +1 on $\Sigma_B$ and $-1$ on $\sigma(\Sigma_B)$ - $\sigma$ being a holomorphic isometric involution as part of the Calabi-Yau orientifold - and $\tilde{f}\in\tilde{H}^2_-(\Sigma^B)\equiv{\rm coker}\left(H^2_-(CY_3)\stackrel{i^*}{\rightarrow}H^2_-(\Sigma^B)\right)$. Also,
\begin{eqnarray}
\label{eq:DdW_def}
{\cal D}_iD_jW=\partial_i\partial_jW + \left(\partial_i\partial_jK\right)W+\partial_iKD_JW +
\partial_JKD_iW - \left(\partial_iK\partial_jK\right)W - \Gamma^k_{ij}D_kW. \nonumber\\
\end{eqnarray}
The gaugino-quark-squark vertex is given as:
 $g_{YM}g_{{ J}B^{*}}X^{{*}B}{\bar\chi}^{\bar J}\lambda_{\tilde{g}}+ + \partial_{a_2}T_B D^{B}{\bar\chi}^{\bar a_1}\lambda^{0}$. Utilizing (\ref{eq:K}) and $X^{B}=-6i\kappa_4^2\mu_7Q_{B}, \kappa_4^2\mu_7\sim \frac{1}{\cal V}, g_{YM}\sim{\cal V}^{-\frac{1}{36}}, \footnote{A small note on dimensional analysis: $\kappa_4^2\mu_7\left(2\pi\alpha^\prime\right)Q_Bg_{\sigma^B{\bar a}_{\bar j}}{\bar\chi}^{\bar j}\lambda$ has dimensions $M_p^4$ - utilizing $\kappa_4^2\mu_7\sim{\cal V}^{-1}\left(2\pi\alpha^\prime\right)^{-3}$, one sees that $Q_B$ has dimensions of $\left(2\pi\alpha^\prime\right)^2M_p$. Using the definition of $Q_B$, we will estimate $Q_B$ by
${\cal V}^{\frac{1}{3}}\left(2\pi\alpha^\prime\right)^2$, where the integral of $i^*\omega_B\wedge P_-\tilde{f}$ over $\Sigma_B$ is approximated by integrals of $i^*\omega_B$ and $P_-\tilde{f}$ over two-cycles non-trivial in the cohomology of $\Sigma_B$ and estimated/parametrized as ${\cal V}^{\frac{1}{3}}\left(2\pi\alpha^\prime\right)$ and ${\tilde f}$ respectively.}Q_B\sim{\cal V}^{\frac{1}{3}}(2\pi\alpha^\prime)^2\tilde{f},$
 \begin{equation}
\label{eq:gYMgBIbar_zi_aI}
g_{YM}g_{B {\bar a}_2}\rightarrow-{\cal V}^{-\frac{5}{4}}(a_2-{\cal V}^{-\frac{1}{3}}), \partial_{a_2}T_B \rightarrow {\cal V}^{\frac{1}{9}} (a_2-{\cal V}^{-\frac{1}{3}}).  \nonumber\\
\end{equation}
 The dominant contribution to the physical gaugino-quark-squark vertex is proportional to :
\begin{equation}
\label{eq:gaugino-quark-squark1}
C^{\tilde{\lambda^{0}}{u_L}\tilde {u_L}}\sim \frac{ {\cal V}^{-\frac{11}{9}} {\tilde f}}{{\left(\sqrt{\hat{K}_{{\cal A}_2{\bar {\cal A}}_2}}\right)}{\left(\sqrt{\hat{K}_{{\cal A}_2{\bar {\cal A}}_2}}\right)}}\sim \tilde{f}\left({\cal V}^{-\frac{4}{5}}\right).
\end{equation}
The contribution of gluino-quark/antiquark-squark vertex is same as gaugino(neural)-quark/antiquark-squark, and therefore proportional to:
\begin{eqnarray}
\label{eq:G}
 G^{{q/{\bar q}}_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}= C^{\tilde{\lambda^{0}}{u_L}\tilde {u_L}}\sim \tilde{f}{\cal V}^{-\frac{4}{5}}{\tilde q}\chi^{q/ \bar q}\lambda_{\tilde{g}},\lambda_{\tilde{g}}~ {\rm corresponds~ to ~gluino}.
\end{eqnarray}
%\item
The neutralino-quark-squark vertex of Figure~\ref{fig:treegdec} is given as considering the contribution of
$$\frac{e^{\frac{K}{2}}}{2}\left({\cal D}_ID_{\bar A_2}W\right)\chi^{{\cal Z}_I}{\chi^{c^{{\cal {A}}_2}}} +ig_{{\bar {\cal Z}_I}{\bar {A_2}}}{\bar\chi}^{{\cal Z}_I}\left[{\bar\sigma}\cdot\partial+\Gamma^{{\cal A}_2}_{{\cal A}_2{\bar A_2}}{\bar\sigma}\cdot\partial {\cal A}_2{\chi^{c^{{\cal {A}}_2}}}
+\frac{1}{4}\left(\partial_{{\cal A}_2}K{\bar\sigma}\cdot {\cal A}_2 - {\rm c.c.}\right){\chi^{c^{{\cal {A}}_2}}} \right]$$
 $\chi^I$ is $SU(2)_L$ higgsino, $\chi^{A_2}$ corresponds to $SU(2)_L$ quark and ${{\cal A}_2}$ corresponds to left-handed squark,
and  $g_{{\bar I}{\bar {\cal A}_2}}=0$. In terms of undiagonalized basis, consider ${\cal D}_iD_{\bar a_2}W= \left(\partial_i\partial_{\bar a_2}K\right)W+\partial_iKD_{\bar a_2}W +
\partial_{\bar a_2}KD_iW - \left(\partial_iK\partial_{\bar a_2}K\right)W,$ where $a_2, z_i$ correspond to undiagonalized moduli fields.
 
Considering  $a_2\rightarrow a_2+{\cal V}^{-\frac{1}{3}}{M_p}$, using equations (\ref{eq:K}), (\ref{eq:W}) and picking up the component linear in  $z_1$ as well as fluctuations of $a_2$, one gets:
\begin{eqnarray}
\label{eq:DKDW32}
& & {\hskip -0.4in} e^{\frac{K}{2}}\left(\left(\partial_i\partial_{\bar a_2}K\right)W+\partial_iKD_{\bar a_2}W +
\partial_{\bar a_2}KD_iW - \left(\partial_iK\partial_{\bar a_2}K\right)W\right)  \sim ({\cal V}^{-\frac{20}{9}})z_i \delta a_2.
\end{eqnarray}
Using equation (\ref{eq:eq_mass_terms_diag_non-diag_basis}),  $e^{\frac{K}{2}}{\cal D}_i D_{{\cal A}_2}W \chi^{{\cal Z}_i}{\chi^{c^{{\cal {A}}_2}}}\sim {\cal V}^{-\frac{20}{9}}{\cal Z}_i\delta{\cal A}_2 \chi^{{\cal Z}_i}{\chi^{c^{{\cal {A}}_2}}},$
 and the contribution of physical higgsino-quark-squark vertex will be given as :
\begin{eqnarray}
\label{eq:Higgsino-quark-squark1}
& &  C^{{\tilde H^{c}}_L {u_L} \tilde {u_L}}\sim\frac{{\cal V}^{-\frac{20}{9}}\langle{\cal Z}_i\rangle}{{\sqrt{\hat{K}^{2}_{{\cal Z}_i{\bar{\cal Z}}_i}{\hat{K}_{{\cal A}_2{\bar {\cal A}}_2}}{\hat{K}_{{\cal A}_2{\bar {\cal A}}_2}}}}} \sim {\cal V}^{-\frac{4}{5}}.
\end{eqnarray}
Following equation (\ref{eq:neutralinos_I}), the neutralino-quark squark vertex will be given by:
\begin{eqnarray}
\label{eq:X}
 {\hskip -0.2in}X^{{q/{\bar q}}}_{\tilde{q}}= C^{{\chi^{0}_3} {u_L}\tilde {u_L}}\sim C^{\tilde{\lambda^{0}}{u_L}\tilde {u_L}}+ {\tilde f}{\cal V}^{\frac{5}{6}}\left(\frac{v}{m_{pl}}\right) C^{H^{c}_L {u_L} \tilde {u_L}} \sim \tilde{f}{\cal V}^{-\frac{4}{5}}{{\chi^{0}_3} {u_L}\tilde {u_L}}.
\end{eqnarray}
%\end{enumerate}
Using RG analysis of coefficients of the effective dimension-six gluino decay operators as given in
\cite{Guidice_et_al}, it was shown in \cite{Dhuria+Misra_mu_Split_SUSY} that these coefficients at the EW scale are of the same order as that at the squark mass scale.

The analytical formulae to calculate decay width for three-body tree-level gluino decay channel as given in \cite{Manuel_Toharia} is:
\begin{eqnarray}
\label{eq:neutralinowidth}
&&\Gamma(\tilde{g}\to\chi_{\rm n}^{o}q_{{}_I} \bar{q}_{{}_J} )
%% &=&{1\over 256 \pi^2 \mgss^3}\int
%% ds_{13}ds_{23}\  |{\cal{M}}(\tilde{g}\to \chi_{\rm n}^o q_{{}_I}\bar{q}_{{}_J})|_{Avg}^2\non\\
=  {g_s^2\over256 \pi^3 \mgss^3 } \sum_{i,j} \int ds_{13} ds_{23}\ {1\over2}
{\cal R}e\Big(A_{ij}(s_{23}) + B_{ij}(s_{13}) \nonumber\\
&&{\hskip 1.3in} -  2 \eps_{n} \eps_{{g}}\
C_{ij}(s_{23},s_{13})\Big), 
\end{eqnarray}
where the integrand is the square of the spin-averaged total amplitude
and $i,j=1,2,..,6$ are the indices of the squarks mediating the decay. The limits of integration in (\ref{eq:neutralinowidth}) are given in \cite{Dhuria+Misra_mu_Split_SUSY}.
The $A_{ij}$ terms in (\ref{eq:neutralinowidth}) represent the contributions from the gluino decay channel involving gluino$\rightarrow$squark+quark and squark$\rightarrow$neutralino+anti-quark, whereas
 the $B_{ij}$ terms come from channel gluino $\rightarrow$squark+anti-quark and squark$\rightarrow$neutralino+quark. The same are defined in \cite{Dhuria+Misra_mu_Split_SUSY}.
Utilizing the results as given in (\ref{eq:G}) and (\ref{eq:neutralino-quark-squark}),

{\small $A_{ij}\Bigl(Tr\left[G^{{\bar q}}_{\tilde{q}}G^{{\bar q}}_{\tilde{q}}\ ^\dagger\right]
Tr\left[X^{q}_{\tilde{q}}X^{q}_{\tilde{q}}\ ^\dagger\right]\Bigr)\sim \tilde{f^4}{\cal V}^{-\frac{16}{5}}$},
{\small $B_{ij}\Bigl(Tr\left[G^{q_{a_1}}_{\tilde{q}_{a_1}}G^{q_{a_1}}_{\tilde{q}_{a_1}}\ ^\dagger\right]
Tr\left[X^{{\bar q}_{a_1}}_{\tilde{q}_{a_1}}X^{{\bar q}_{a_1}}_{\tilde{q}_{a_1}}\ ^\dagger\right]\Bigr)$ $\sim \tilde{f^4}{\cal V}^{-\frac{16}{5}}$}, 
{\small $C\Bigl(Tr\left[G^{{\bar q}}_{\tilde{q}_{a_1}}G^{q}_{\tilde{q}}\ ^\dagger X^{q}_{\tilde{q}}X^{{\bar q}}_{\tilde{q}}\ ^\dagger\right]\Bigr)\sim \tilde{f^4}{\cal V}^{-\frac{16}{5}}$}. 

Substituting these values for various vertex elements and solving equation (\ref{eq:neutralinowidth}) by using the limits of integration as given in \cite{Dhuria+Misra_mu_Split_SUSY},  the dominating contribution of decay width  is:
\begin{eqnarray}
 \label{eq: Decay width 1}
 \hspace{-.5cm}\Gamma(\tilde{g}\to\chi_{\rm n}^{o}q_{{}_I} \bar{q}_{{}_J} )
%% &=&{1\over 256 \pi^2 \mgss^3}\int
%% ds_{13}ds_{23}\  |{\cal{M}}(\tilde{g}\to \chi_{\rm n}^o q_{{}_I}\bar{q}_{{}_J})|_{Avg}^2\non\\
&\sim&{g_s^2  \over256 \pi^3  {\cal V}^2 m_{\frac{3}{2}}^3 }\left[
{\tilde{f}^4  {\cal V}^{-\frac{16}{5}} m_{\frac{3}{2}}^4 }{\cal V}^{\frac{10}{3}}+ \tilde{f}^4{\cal V}^{-\frac{16}{5}}{\cal V}^{\frac{10}{3}} m_{\frac{3}{2}}^4 +\tilde{f}^4{\cal V}^{-\frac{16}{5}} {\cal V}^{\frac{10}{3}} m_{\frac{3}{2}}^4\right] \nonumber\\
& & {\hskip -1.1in} \sim { g_s^2\over256 \pi^3  {\cal V}^2 m_{\frac{3}{2}}^3 }\left( \tilde{f}^4{\cal V}^{-\frac{16}{5}}{\cal V}^{\frac{10}{3}} m_{\frac{3}{2}}^4  \right)\sim O(10^{-4})\tilde{f}^4{\cal V}^{-\frac{19}{5}}{M_p} \ \sim O(10^{-5})\tilde{f}^4 GeV.
 \end{eqnarray}
 \paragraph{Upper bound on dilute flux $\tilde{f}$:}
  In case of ${\cal N}=1$ gauged supergravity, the modified D-term scalar potential in presence of background $D7$ fluxes is defined as \cite{jockersetal}:
   \begin{equation}
   \label{eq:Dterm}
V_D = {\frac{108\kappa_4^2\mu_7}{{{\cal{K}}^2}{ReT_B}}}({{\cal{K}}_{Pa}}{\cal{B}}^a-{\cal{Q}_{B}}{\emph{v}}^{B})^2.
\end{equation}
The first term of $V_D$ can be minimized for ${\cal{B}}^a= 0$ and second term has extra contribution coming from additional D7-brane fluxes.
Now, the corresponding F-term scalar potential in LVS limit has been calculated in \cite{D3_D7_Misra_Shukla} as:
\begin{equation}
\label{eq:Fterm}
V_f\sim e^K G^{\sigma^{{\alpha}}{\bar{\sigma}^{\bar{\alpha}}}}D_{\sigma^{\alpha}}W^\alpha{\bar{D}_{\bar{\sigma}^{\bar{\alpha}}}}\bar{W}\sim{\cal{V}}^{19/18}m_{3/2}^2
\sim{\cal{V}}^{-3}m_{pl}^2.
\end{equation}
 In case of dilute flux approximation $V_D << V_f$. Therefore, from (\ref{eq:Dterm}) and (\ref{eq:Fterm}),
 \begin{equation}
 {\frac{108\kappa_4^2\mu_7}{{{\cal{K}}^2}{ReT_B}}}({\cal{Q}_{B}}{\emph{v}}^{B})^2 << {\cal{V}}^{-3}m_{pl}^2,
 \end{equation}
 where $Q_B\sim{\cal V}^{\frac{1}{3}}{\tilde f}\left(2\pi\alpha^\prime\right)^2M_p$, $ \kappa_4^2\mu_7\sim\frac{1}{\cal{V}}, {\cal{K}}=1/6Y$(volume of physical Calabi Yau), ${ReT_B}\sim {\cal{V}}^{2/3}$
 (volume of ``Big" Divisor) and ${\cal{V}}^{B}\sim{\cal{V}}^{1/3}$(internal volume of 2-cycle),
 solving this: $ \frac{10^{4}{\tilde f}^2{\cal{V}}^{4/3}}{{\cal{V}}^3{\cal{V}}^{2/3}}<<{\cal{V}}^{-3}$, i.e   ${\tilde f}^2<< 10^{-8}$.
 
By considering ${{\tilde f}^2}\sim{10}^{-10}$, the decay width of gluino i.e equation (\ref{eq: Decay width 1}) becomes:
$ \Gamma(\tilde{g}\to\chi_{\rm n}^{o}q_{{}_I} \bar{q}_{{}_J} )\sim O(10^{-5}){\tilde f}^4 < {\cal O}(10^{-25})GeV$.
 Further, life time of gluino is given as:
   \begin{eqnarray}
   \tau &=&\frac{\hbar}{\Gamma}\sim\frac{10^{-34} Jsec}{10^{-5}{\tilde f}^4 GeV}\sim\frac{10^{-19}}{{\tilde f}^4} > 10 \ sec.
   \end{eqnarray}
   
$\underline{\bf{\tilde{g}\rightarrow\tilde{\chi}_3^0 \ g}}$

\begin{figure}
\begin{center}
\begin{picture}(500,170)(50,0)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\Text(140,135)[]{$\tilde{g}$}
\Line(110,120)(160,120)
\Gluon(110,120)(160,120){5}{4}
%\Text(150,130)[]{$\tilde{g}$}
\ArrowLine (160,120)(190,150)
\Text(180,152)[]{$q_I$}
\DashArrowLine (190,90)(160,120){4}
\Text(170,100)[]{$\tilde{q}_R$}
\DashArrowLine (190,150)(190,90){4}
\Gluon(190,90)(230,90){5}{4}
\Text(240,90)[]{$g_\mu$}
\ArrowLine(190,150)(230,150)
\Text(240,150)[]{$\tilde{\chi}_3^0$}
\Text(190,60)[]{(a)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\ArrowLine(110,120)(160,120)
\Line(310,120)(360,120)
\Gluon(310,120)(360,120){5}{4}
\Text(340,135)[]{$\tilde{g}$}
\DashArrowLine (360,120)(390,150){4}
\Text(380,152)[]{$\tilde{q}_R$}
\ArrowLine (390,90)(360,120)
\Text(370,100)[]{$q_I$}
\ArrowLine (390,150)(390,90)
\Gluon(390,90)(430,90){5}{4}
\Text(440,90)[]{$g_\mu$}
\ArrowLine(390,150)(430,150)
\Text(440,150)[]{$\tilde{\chi}_3^0$}
\Text(390,60)[]{(b)}
\end{picture}
\end{center}
\vskip -0.7in
\caption {Diagrams contributing to one-loop two-body gluino decay.}
\label{fig:loopgdc}
\end{figure}
Relevant to Figs.~\ref{fig:loopgdc}(a) and \ref{fig:loopgdc}(b), the gluino-quark-squark vertex and the neutralino-quark-squark vertex will again be given by equations (\ref{eq:G}) and (\ref{eq:X}). The quark-quark-gluon vertex relevant to Figure~\ref{fig:loopgdc}, from \cite{Wess_Bagger} is given by:
  \begin{eqnarray}
  \label{eq:qqgl 1}
& &  g_{I{\bar J}}{\bar\chi}^{\bar J}{\bar\sigma}\cdot A\ {\rm Im}\left(X^BK + i D^B\right)\chi^I,\nonumber\\
& & \sim g_{YM}g_{{\cal A}_2 {\bar {\cal A}_2}}{\bar\chi}^{\bar {{\cal A}_2}}{\bar\sigma}\cdot A\left\{6\kappa_4^2\mu_72\pi\alpha^\prime Q_BK+\frac{12\kappa_4^2\mu_72\pi\alpha^\prime Q_Bv^B}{\cal V}\right\},
  \end{eqnarray}
   $\chi^{{\cal A}_2}$ and ${\bar\chi}^{\bar {{\cal A}_2}}$ correspond to quarks and antiquarks.
 $X=X^B\partial_B=-12i\pi\alpha^\prime\kappa_4^2\mu_7Q_B\partial_{T_B}$  corresponds to the killing isometry vector and $D$ term generated is given as: $D^B=\frac{4\pi\alpha^\prime\kappa_4^2\mu_7Q_Bv^B}{\cal V}$.
Utilizing  value of $Q_B\sim{\cal V}^{\frac{1}{3}}f\left(2\pi\alpha^\prime\right)^2M_p$, $g_{{\cal A}_2{\bar {\cal A}}_{\bar 2}}\sim{\cal V}^{-\frac{5}{9}}, v^B\sim{\cal V}^{\frac{1}{3}}, Q_B\sim{\cal V}^{\frac{1}{3}}(2\pi\alpha^\prime)^2\tilde{f}$,  it has been shown in chapter {\bf 4} that quark-quark-gluon vertex will be of ${\cal O}(1)$.

The gauge kinetic term for squark-squark-gluon vertex, relevant to Figure~\ref{fig:loopgdc}(b), will be given by $ {\frac{1}{\kappa_4^2{\cal V}^2}}G^{T_B{\bar T}_B}\tilde{\bigtriangledown}_\mu T_B\tilde{\bigtriangledown}^\mu {\bar T}_{\bar B}$.  Using the value of $G^{T_B{\bar T}_B}(EW)= {\cal V}^{\frac{7}{3}}$ (for detailed explanation, see chapter {\bf 4}), the given term generates the required squark-squark-gluon vertex as follows:
\begin{eqnarray}
\label{eq:sq sq gl}
& &  {\frac{6i\kappa_4^2\mu_72\pi\alpha^\prime Q_BG^{\sigma_B{\bar\sigma}_B}}{\kappa_4^2{\cal V}^2}}A^\mu\partial_\mu\left(\kappa_4^2\mu_7(2\pi\alpha^\prime)^2C_{2{\bar 2}}{\cal A}_2{\bar {\cal A}}_{\bar 2}\right)\nonumber\\
&& \xrightarrow[{\small \kappa_4^2\mu_7(2\pi\alpha^\prime)^2C_{2{\bar 2}}\sim{\cal V}^{\frac{1}{9}}}]{\small G^{\sigma_B{\bar\sigma}_B}\sim{\cal V}^{\frac{7}{3}},}\frac{{\cal V}^{\frac{7}{9}}\epsilon\cdot\left(2k-(p_{\tilde{\chi}_3^0}+p_{\tilde{g}})\right)}{\left(\sqrt{\hat{K}_{{\cal A}_2{\bar {\cal A}}_2}}\right)^2} \sim O({10}^{2})\tilde{f}{\cal V}^{\frac{7}{9}}\left[ 2\epsilon\cdot k-\epsilon\cdot\left(p_{\tilde{\chi}_3^0}+p_{\tilde{g}}\right)\right]\nonumber\\
&& \sim \tilde{f}{\cal V}^{\frac{53}{45}}, {\rm for~{\cal V}\sim {10}^5}.
\end{eqnarray}
In \cite{Dhuria+Misra_mu_Split_SUSY}, it has been discussed that behavior of Wilson coefficients corresponding to  two-body gluino decay does not change much upon RG evolution to EW scale.  Using the vertices calculated above relevant to Figs.~\ref{fig:loopgdc}(a) and \ref{fig:loopgdc}(b), and the Feynman rules of \cite{2comp}, one obtains for the scattering amplitude:
\begin{eqnarray}
\label{eq:M_I}
& & {\cal M}\sim\tilde{f}^3M_p \int\frac{d^4k}{\left(2\pi\right)^4} \times{\cal V}^{-\frac{4}{5}}\left(\frac{i{\bar\sigma}\cdot k}{k^2-m_q^2+i\epsilon}\right)\left({\cal V}^{-\frac{4}{5}}
\right)\left(\frac{i}{\left[\left(k-p_{\tilde{G}}\right)^2-m^2_{\tilde{q}}+i\epsilon\right]}
\right)\nonumber\\
& & \times\left({\cal V}^{\frac{53}{45}}\right)\Bigl(\frac{i}
{\left[\left(k-p_{\tilde{g}}\right)^2-m^2_{\tilde{q}}+i\epsilon\right]}\Bigr)\nonumber\\
& & + \tilde{f}^2M_p \int\frac{d^4k}{\left(2\pi\right)^4} \times {\cal V}^{-\frac{4}{5}}\Biggl(\frac{i}
{\left[\left(k+p_{\tilde{\chi}_3^0}\right)^2-m^2_{\tilde{q}}+i\epsilon\right]}\Biggr)\left({\cal V}^{-\frac{4}{5}}
\right)\left(\frac{i{\bar\sigma}\cdot k}{k^2-m_q^2+i\epsilon}\right)\nonumber\\
& & \times\Biggl(\frac{i{\bar\sigma}\cdot\left(k-p_{g_\mu}\right)}{\left[
\left(k-p_{g_\mu}\right)^2-m^2_q+i\epsilon\right]}\Biggr).
\end{eqnarray}
Using the 1-loop integrals of \cite{Pass+Velt}:
\begin{eqnarray}
\label{eq:passvelt}
& & \frac{1}{i}\int\frac{d^4k}{\left(2\pi\right)^4}\frac{\left(k_\mu,\ k_\mu k_\nu\right)}{\left(k^2-m_1^2+i\epsilon\right)
\left[\left(k+p_1\right)^2-m_2^2+i\epsilon\right]\left[\left(k+p_1+p_2\right)^2-m_3^2+i\epsilon\right]}\nonumber\\
& & =4\pi^2\Biggl[p_{1\mu}C_{11}+p_{2\mu}C_{12}, p_{1\mu}p_{1\nu}C_{21}+p_{2\mu}p_{2\nu}C_{22}+\left(p_{1\mu}p_{2\nu}+p_{1\nu}p_{2\mu}\right)C_{23}+\eta_{\mu\nu}C_{24}\Biggr];
\nonumber\\
& & (a)~m_1=m_q, m_2=m_3=m_{\tilde{q}};\ p_1=-p_{\tilde{\chi}_3^0}, p_2=-p_{g_\mu};\nonumber\\
& & (b)~m_1=m_3=m_q, m_2=m_{\tilde{q}};\ p_1=p_{\tilde{\chi}_3^0}, p_2=-p_{\tilde{g}}.
\end{eqnarray}
\vskip -0.4in
The one-loop three-point functions $C_{ij}$'s relevant for cases (a) and (b) have been calculated in \cite{Dhuria+Misra_mu_Split_SUSY} and are given as under:
\begin{eqnarray}
\label{eq: three point functions}
& & C^{(a)}_{24}= O(10^6), C^{(b)}_{24}=  O(10^6),\nonumber\\
&& C^{(a)}_0= \frac{1}{4{\pi}^2}\times 10^{-21}\sim O(1)\times {10}^{-23}~{GeV}^{-2},\nonumber\\
&&C^{(b)}_{11}=  O(10) \times {10}^{-16} {GeV}^{-2}, C^{(b)}_{12}=  O(10)\times {10}^{-16}~{GeV}^{-2},\nonumber\\
&&C^{(b)}_{21}= C^{(b)}_{22}= C^{(b)}_{23}\sim O(1) \times {10}^{-10}~{GeV}^{-2}, C^{(b)}_0= \frac{1}{4{\pi}^2}\times 10^{-21}\sim O(1)\times {10}^{-23}~{GeV}^{-2}. \nonumber\\
  \end{eqnarray}
Now, equation (\ref{eq:M_I}) can be evaluated to yield:
\begin{eqnarray}
\label{eq:M_II}
& & {\bar u}(p_{\tilde{\chi}_3^0})\Biggl(\tilde{f}^3{\cal V}^{-0.4}\Bigl[\left\{{\bar\sigma}\cdot p_{\tilde{\chi}_3^0}C^{(a)}_{11}+{\bar\sigma}\cdot p_{g_\mu}C^{(a)}_{12}\right\}(2\epsilon\cdot p_{\tilde{\chi}_3^0}) \left\{{\bar\sigma}\cdot p_{\tilde{\chi}_3^0}\epsilon\cdot p_{\tilde{\chi}_3^0}C^{(a)}_{21}\right.+\nonumber\\
&& \left.+{\bar\sigma}\cdot p_{g_\mu}\epsilon\cdot p_{\tilde{\chi}_3^0}C^{(a)}_{23}
+{\bar\sigma}\cdot\epsilon C^{(a)}_{24}\right\}\Bigr]\nonumber\\
& & + \tilde{f}^2{\cal V}^{-1.6}\Bigl[-\left\{{\bar\sigma}\cdot p_{\tilde{\chi}_3^0}C^{(b)}_{11}
+{\bar\sigma}\cdot p_{\tilde{g}}C^{(b)}_{12}\right\}{\bar\sigma}\cdot\epsilon{\bar\sigma}\cdot p_{g_\mu}+
{\bar\sigma}\cdot p_{\tilde{\chi}_3^0}{\bar\sigma}\cdot\epsilon {\bar\sigma}\cdot p_{\tilde{\chi}_3^0}C^{(b)}_{21} \nonumber\\
& & + {\bar\sigma}\cdot p_{\tilde{g}}{\bar\sigma}\cdot\epsilon {\bar\sigma}\cdot p_{\tilde{g}}C^{(b)}_{22}  -\biggl({\bar\sigma}\cdot p_{\tilde{\chi}_3^0}{\bar\sigma}\cdot\epsilon{\bar\sigma}\cdot p_{\tilde{g}} + {\bar\sigma}\cdot p_{\tilde{g}}{\bar\sigma}\cdot\epsilon {\bar\sigma}\cdot p_{\tilde{\chi}_3^0}\biggr)C^{(b)}_{23}+ \nonumber\\
&&{\bar\sigma}_\mu{\bar\sigma}\cdot\epsilon{\bar\sigma}^\mu C^{(b)}_{24}\Bigr]\Biggr)
u(p_{\tilde{g}}),
\end{eqnarray}
which equivalently could be rewritten as:
\begin{equation}
\label{eq:M_III}
 {\bar u}(p_{\tilde{\chi}_3^0})\Biggl[{\bar\sigma}\cdot{\cal A}+{\bar\sigma}\cdot p_{\tilde{\chi}_3^0}{\bar\sigma}\cdot\epsilon{\bar\sigma}\cdot{\cal B}_1 + {\bar\sigma}\cdot p_{g_\mu}
{\bar\sigma}\cdot\epsilon{\bar\sigma}\cdot{\cal B}_2 + D_3{\bar\sigma}_\mu{\bar\sigma}\cdot\epsilon{\bar\sigma}^\mu
C^{(b)}_{24} \Biggr]u(p_{\tilde{g}}),
\end{equation}
where
\vskip -0.5in
\begin{eqnarray}
\label{eq:AB1B2}
& & {\cal A}^\mu\equiv \tilde{f}^3{\cal V}^{-0.4}\left[p_{\tilde{\chi}_3^0}^\mu\epsilon\cdot p_{\tilde{\chi}_3^0}\left(2C^{(a)}_{11} + C^{(a)}_{21}\right) + p_{g_\mu}^\mu\epsilon\cdot p_{\tilde{\chi}_3^0}\left(C^{(a)}_{12} + C^{(a)}_{23}\right) + \epsilon^\mu C^{(a)}_{24}\right],\nonumber\\
& & {\cal B}_1^\mu\equiv  \tilde{f}^2{\cal V}^{-1.6}\left[-p_{g_\mu}^\mu\left(C^{(b)}_{11} + C^{(b)}_{12} + C^{(b)}_{23}-C^{(b)}_{22}\right) + p_{\tilde{\chi}_3^0}^\mu\left(C^{(b)}_{21} + C^{(b)}_{22} - 2C^{(b)}_{23}\right)\right],\nonumber\\
& & {\cal B}_2^\mu\equiv \tilde{f}^2{\cal V}^{-1.6}\left[p_{g_\mu}^\mu\left(C^{(b)}_{12}+C^{(b)}_{22}\right) + p_{\tilde{\chi}_3^0}^\mu\left( C^{(b)}_{22} - C^{(b)}_{23}\right)\right], {D_3}\equiv \tilde{f}^2{\cal V}^{-1.6}.
\end{eqnarray}
Replacing ${\bar u}(p_{\tilde{\chi}_3^0}){\bar\sigma}\cdot p_{\tilde{\chi}_3^0}$ by $m_{\tilde{\chi}_3^0}{\bar u}(p_{\tilde{\chi}_3^0})$ and ${\bar\sigma}\cdot p_{\tilde{g}}u(p_{\tilde{g}})$ by $m_{\tilde {g}}$, and using $\epsilon\cdot p_{\tilde{\chi}_3^0}=0$, (\ref{eq:M_III}) can be simplified to:
\begin{eqnarray}
\label{eq:M_IV}
&&{\cal M}\sim {\bar u}(p_{\tilde{\chi}_3^0})\left[A{\bar\sigma}\cdot\epsilon + B_1{\bar\sigma}\cdot\epsilon
{\bar\sigma}\cdot p_{\tilde{\chi}_3^0} + B_2{\bar\sigma}\cdot p_{\tilde{g}}{\bar\sigma}\cdot\epsilon +
D_1{\bar\sigma}\cdot p_{\tilde{g}}{\bar\sigma}\cdot\epsilon{\bar\sigma}\cdot p_{\tilde{\chi}_3^0}\right. \nonumber\\
&&\left. + {D_3} {\bar\sigma}_\mu{\bar\sigma}\cdot\epsilon{\bar\sigma}^\mu C^{(b)}_{24}\right]u(p_{\tilde{g}}),
\end{eqnarray}
where,
\vskip -0.5in
\begin{eqnarray}
\label{eq:AB1B2D1 defs}
&&A\equiv {\cal V}^{-0.4} \tilde{f}^3 C^{(a)}_{24} - m_{\tilde{g}}m_{\tilde{\chi}_3^0} {\cal V}^{-1.6} \tilde{f}^2\Bigl\{
 C^{(b)}_{11} + 2 C^{(b)}_{12} + C^{(b)}_{23}-C^{(b)}_{22}\Bigr\},\nonumber\\
&& B_1\equiv {\cal V}^{-1.6}\tilde{f}^2\left(C^{(b)}_{11} + 2 C^{(b)}_{12} +  C^{(b)}_{21}\right)m_{\tilde{\chi}_3^0}, B_2\equiv {\cal V}^{-1.6}\tilde{f}^2\left(C^{(b)}_{12}+C^{(b)}_{22}\right)m_{\tilde{g}},\nonumber \\
&& D_1\equiv {\cal V}^{-1.6}\tilde{f}^2\left(- C^{(b)}_{12}- C^{(b)}_{23}\right).
\end{eqnarray}
 Utilizing values of C's calculated in (\ref{eq: three point functions}),
 $   A \sim {\cal O}(10^{5})\tilde{f}^2, B_1\sim {\cal O}({10^{-7}})\tilde{f}^2{GeV}^{-2}, B_2\sim {\cal O}({10^{-7}})\tilde{f}^2{GeV}^{-2}$, $D_1\sim {\cal O}({10^{-18}})\tilde{f}^2{GeV}^{-2};{D_3}\sim {\cal V}^{-1.6}\tilde{f}^2$.
\begin{eqnarray}
\label{eq:spinavGamma}
& & {\rm and}~~  \sum_{\tilde{g}\ {\rm and}\ \tilde{\chi}_3^0\ {\rm spins}}|{\cal M}|^2
\sim Tr\Biggl(\sigma\cdot p_{\tilde{\chi}_3^0}\left[A{\bar\sigma}\cdot\epsilon + B_1{\bar\sigma}\cdot\epsilon
{\bar\sigma}\cdot p_{\tilde{\chi}_3^0} + B_2{\bar\sigma}\cdot p_{\tilde{g}}{\bar\sigma}\cdot\epsilon \right. \nonumber\\
& & \left. +
D_1{\bar\sigma}\cdot p_{\tilde{g}}{\bar\sigma}\cdot\epsilon{\bar\sigma}\cdot p_{\tilde{\chi}_3^0}  + D_3 {\bar\sigma}_\mu{\bar\sigma}\cdot\epsilon{\bar\sigma}^\mu C^{(b)}_{24}\right]\nonumber\\
& & \times\sigma\cdot p_{\tilde{g}}\left[A{\bar\sigma}\cdot\epsilon + B_1{\bar\sigma}\cdot\epsilon
{\bar\sigma}\cdot p_{\tilde{\chi}_3^0} + B_2{\bar\sigma}\cdot p_{\tilde{g}}{\bar\sigma}\cdot\epsilon +
D_1{\bar\sigma}\cdot p_{\tilde{g}}{\bar\sigma}\cdot\epsilon{\bar\sigma}\cdot p_{\tilde{\chi}_3^0} \right.\nonumber\\
&&\left. + D_3 {\bar\sigma}_\mu{\bar\sigma}\cdot\epsilon{\bar\sigma}^\mu C^{(b)}_{24}\right]^\dagger\Biggr),
\end{eqnarray}
\vskip -0.3in
which at  $p^0_{\tilde{\chi}_3^0}=\sqrt{m_{\tilde{\chi}_3^0}^2c^4+\rho^2},
p^1_{\tilde{\chi}_3^0}=p^2_{\tilde{\chi}_3^0}=p^3_{\tilde{\chi}_3^0}=\frac{\rho}{\sqrt{3}}
=\frac{1}{\sqrt{3}}\frac{c\left(m_{\tilde{g}}^2 - m_{\tilde{\chi}_3^0}^2\right)}{2m_{\tilde{g}}}$,
yields:
\begin{eqnarray}
\label{eq:trace}
& &  \frac{1}{256}{m_{\tilde{g}}}^2 \biggl[6 {m^{2}_{\tilde{g}}}({B_1}+{D_1} {m_{\tilde{g}}})^2+\left\{8
   {A_1}+16 D_3{C_{24}}+{m_{\tilde{g}}} \left(\left(5+\sqrt{3}\right) {B_1}+8 {B_2}\right. \right. \nonumber\\
   && \left. \left. +\left(5+\sqrt{3}\right) {D_1}
   {m_{\tilde{g}}}\right)\right\}^2\biggr],
   \end{eqnarray}
in the rest frame of the gluino.\\
Incorporating results of (\ref{eq:AB1B2D1 defs}) in equation (\ref{eq:trace}), one gets, 
\begin{equation}
 \sum_{\tilde{g}\ {\rm and}\ \tilde{\chi}_3^0\ {\rm spins}}|{\cal M}|^2 \sim 0.2 {D^{2}_1} m_{\tilde{g}}^6. 
 \end{equation}
 Now, using standard two-body decay results (See \cite{Griffiths_particle}), the decay width $\Gamma$ is given by the following expression: $
\Gamma=\frac{\sum_{\tilde{g}\ {\rm and}\ \tilde{\chi}_3^0\ {\rm spins}}|{\cal M}|^2\left(m_{\tilde{g}}^2-m_{\tilde{\chi}_3^0}^2\right)}{16\pi\hbar m_{\tilde{g}}^3}.$
Using value of $D_1\sim O({10^{-18}}){\tilde f}^2 \ {GeV}^{-2}$ as given above, $m_{\tilde{g}}\sim {\cal V}^{-\frac{4}{3}}{M_p} \ GeV$, and
$m^{2}_{\tilde{\chi_3^0}}\sim m^{2}_{\tilde{g}}+ \frac{m_{\tilde g} {\tilde f}^2  v^2 {\cal V}^{\frac{2}{3}}}{m_{pl}}$ ${GeV}^{2}$, two-body decay width is given as:
\begin{equation}
\label{eq:Gamma1}
\Gamma=  \frac{(0.2) {D_1^2} m_{\tilde {g}}^6} {16\pi m_{\tilde{g}}^3} \sim \frac{O({10}^{-2}) \tilde{f}^4.{10^{-36}}.{m_{\tilde {g}}}^6 (2\frac{m_{\tilde g} {\tilde f}^2  v^2 {\cal V}^{\frac{2}{3}}}{m_{pl}})} {m_{\tilde{g}}^3}\sim{10}^{-4} \tilde{f}^4 GeV.
\end{equation}
Considering $\tilde{f} < {10}^{-5}$ as calculated above, $\Gamma < {10}^{-24}$ GeV.  Life time of gluino is given as:
   \begin{eqnarray}
   \tau &=&\frac{\hbar}{\Gamma}\sim\frac{10^{-34} Jsec}{10^{-4}{\tilde f}^4 GeV}\sim\frac{10^{-20}}{{\tilde f}^6} sec > {10}^{10}sec.
 \end{eqnarray}
\underline{${\bf \tilde{g}\rightarrow\tilde{G} \ q \ {\bar q}}$}\\
We now consider the three-body decay of the gluino into goldstino and a quark and an anti-quark: $\tilde{g}\rightarrow\tilde{G}+q+{\bar q}$. The Feynman diagrams corresponding to this particular decay are shown in Figure~\ref{fig:gludecgoldstno}.
\begin{figure}
\begin{center}
\begin{picture}(250,180)(50,0)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\Text(90,130)[]{$\tilde{g}$}
%\ArrowLine(110,120)(160,120)
\Line(60,120)(110,120)
\Gluon(60,120)(110,120){5}{4}
\Vertex(110,120){3.5}
\ArrowLine(110,120)(140,150)
\Text(149,150)[]{${q}_{a_2}$}
\DashArrowLine (130,90)(110,120){4}
\Text(107,100)[]{$\tilde{q}_{a_2}$}
\ArrowLine(160,120)(130,90)
\Text(167,120)[]{${\bar{q}_{a_2}}$}
\Line(130,90)(160,60)
\Line(128,86)(158,56)
\Vertex(129,88){3.5}
\Text(167,65)[]{${\tilde G}$}
\Text(110,30)[]{(a)}
%%%%%%%%%%%%%%%%%%%%%%
\Text(250,130)[]{$\tilde{g}$}
\Line(210,120)(260,120)
\Gluon(210,120)(260,120){5}{4}
\ArrowLine (290,150)(260,120)
\Vertex(260,120){3.5}
\Text(299,150)[]{$\bar{q}_{a_2}$}
\DashArrowLine(260,120)(280,90){4}{}
\Text(257,100)[]{$\tilde{q}_{a_4}$}
\ArrowLine(280,90)(310,120)
\Text(320,120)[]{$q_{a_2}$}
\Line(280,90)(310,60)
\Line(278,86)(308,56)
\Vertex(279,88){3.5}
\Text(317,65)[]{${\tilde G}$}
\Text(280,30)[]{(b)}
%%%%%%%%%%%%%%%%%%%%%%%%%
\end{picture}
\vskip-0.3in
\caption{Three-body gluino decay into goldstino.}
\end{center}
\label{fig:gludecgoldstno}
\end{figure}
The gluino-(anti-)quark-squark vertex will again be given by (\ref{eq:G}). The gravitino-quark-squark vertex would come from a term of type  ${\bar\psi}_\mu
\tilde{q}_Lq_L$, which in ${\cal N}=1$ gauged supergravity action of \cite{Wess_Bagger} is given by:
\begin{equation}
\label{eq:gravitino-q-sq}
-g_{I{\bar J}}\left(\partial_\mu {\bar {\cal A}}^{\bar J}\right)\chi^I\sigma^\nu{\bar\sigma}_\mu\psi_\nu - \frac{i}{2}e^{\frac{K}{2}}\left(D_IW\right)\chi^I\sigma^\mu{\bar\psi}_\mu + {\rm h.c.}.
\end{equation}
From \cite{gravitinomodexp}, the gravitino field can be decomposed into the spin-$\frac{1}{2}$ goldstino field $\tilde{G}$
via: 
$\psi_\nu=\rho_\nu + \sigma_\nu\tilde{G},\ \tilde{G}=-\frac{1}{3}\sigma^\mu\psi_\mu$,
$\rho_\nu$ being a spin-$\frac{3}{2}$ field.
Hence, the goldstino-content of (\ref{eq:gravitino-q-sq}), using $\sigma^\nu{\bar\sigma}^\mu\sigma_\nu=-2{\bar\sigma}^\nu$,
is given by: $2g_{I{\bar J}}\chi^I\left(\partial_\mu {\bar {\cal A}}^{\bar J}\right){\bar\sigma}^\mu\tilde{G} + \frac{3i}{2}e^{\frac{K}{2}}\left(D_IW\right)\chi^I\tilde{G} + {\rm h.c.}$. Utilizing
\begin{eqnarray}
\label{eq:Goldstino-s-sq_II}
& & g_{{\cal A}_2{\bar {\cal A}}_{2}}\sim{\cal V}^{-\frac{5}{9}}~ {\rm and}~ e^{\frac{K}{2}}D_{{\cal A}_2}W\Biggr|_{{\cal A}_2\rightarrow {\cal A}_{2} +{\cal V}^{-\frac{1}{3}}}\sim {\cal V}^{-\frac{37}{18}}{\cal A}_{2},
\end{eqnarray}
one obtains:
\begin{eqnarray}
\label{eq:Goldstino-s-sq_I}
& & {\hskip -0.5in}2g_{{\cal A}_{2}{\bar {\cal A}}_{2}}\chi^I\left({\bar\sigma}\cdot\frac{p_{q_{{\cal A}_2}}+ p_{\tilde{G}}}{M_p}\right){\bar\sigma}^\mu\tilde{G} + \frac{3i}{2}e^{\frac{K}{2}}\left(D_{{\cal A}_2}W\right)\chi^I\tilde{G} + {\rm h.c.}\nonumber\\
& & {\hskip -0.5in}\sim  {\cal V}^{-\frac{5}{9}}\chi^I\left(\frac{m_{G}}{M_p}\right){{\cal A}_2}\tilde{G} + {\cal V}^{-\frac{5}{9}}\chi^I\left(\frac{m_{q_{{\cal A}_2}}}{M_p}\right){{\cal A}_2}\tilde{G}+ {\cal V}^{-\frac{37}{18}}{\cal A}_2\chi^I\tilde{G} \sim {\cal V}^{-\frac{37}{18}}{\cal A}_2\chi^I\tilde{G},
\end{eqnarray}
for $m_{q_{{\cal A}_2}}\sim O(10)MeV, m_G \sim 0$ and ${\cal V}\sim 10^5.$

The physical goldstino-quark-squark vertex will be given as:
\begin{equation}
\tilde{G}^{q_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}\sim \frac{{\cal V}^{-\frac{1}{18}}{\cal A}_2\chi^I\tilde{G}}{\left(\sqrt{\hat{K}_{{\cal A}_2{\bar {\cal A}}_2}}\sqrt{\hat{K}_{{\cal A}_2{\bar {\cal A}}_2}}\right)}
\sim O({10}^{2}){\cal V}^{-\frac{37}{18}}\sim {\cal V}^{-\frac{15}{9}} ~{\rm for}~ {\cal V}\sim {10}^5.
 \end{equation}
%\Text(240,50)[]{$$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 For this particular case:-

{\small $A_{ij}\Bigl(Tr\left[G^{{\bar q}_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}G^{{\bar q}_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}\ ^\dagger\right]
Tr\left[\tilde{G}^{q_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}\tilde{G}^{q_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}\ ^\dagger\right]\Bigr)\sim \tilde{f}^2{\cal V}^{-\frac{8}{5}}.{\cal V}^{-\frac{10}{3}}\sim \tilde{f}^2{\cal V}^{-5}$},

 {\small $B_{ij}\Bigl(Tr\left[G^{q_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}G^{q_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}\ ^\dagger\right]
Tr\left[\tilde{G}^{{\bar q}_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}\tilde{G}^{{\bar q}_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}\ ^\dagger\right]\Bigr)\sim \tilde{f}^2{\cal V}^{-\frac{8}{5}}.{\cal V}^{-\frac{10}{3}}\sim \tilde{f}^2{\cal V}^{-5}$},

{\small $C\Bigl(Tr\left[G^{{\bar q}_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}G^{q_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}\ ^\dagger \tilde{G}^{q_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}\tilde{G}^{{\bar q}_{{\cal A}_2}}_{\tilde{q}_{{\cal A}_2}}\ ^\dagger\right]\Bigr)\sim \tilde{f}^2{\cal V}^{-\frac{8}{5}}.{\cal V}^{-\frac{10}{3}}\sim \tilde{f}^2{\cal V}^{-5}$}.
\vskip 0.05in
Limits of integration as given in \cite{Dhuria+Misra_mu_Split_SUSY} are:
\begin{eqnarray}
&& {\hskip -0.2in} s_{23 \max }= \left({\cal V}^{\frac{2}{3}}m_{\frac{3}{2}}-m_q\right){}^2,\ s_{23 \min }= m_q^2, s_{13 \max }= {\cal V}^{\frac{4}{3}}m_{\frac{3}{2}}^2-s_{23}, s_{13 \min }= 0.
\end{eqnarray}
where $m_{\tilde{g}}= {\cal V}^{\frac{2}{3}}m_{\frac{3}{2}} \sim {10}^{11} GeV, m_{\tilde{G}}= 0$.
Utilizing the values of vertex elements calculated above and from (\ref{eq:neutralinowidth}), we calculate decay width for gluino as:
\begin{eqnarray}
 \label{eq: Decay width goldstino}
\Gamma(\tilde{g}\to\chi_{\rm n}^{o}q_{{}_I} \bar{q}_{{}_J} )
%% &=&{1\over 256 \pi^2 \mgss^3}\int
%% ds_{13}ds_{23}\  |{\cal{M}}(\tilde{g}\to \chi_{\rm n}^o q_{{}_I}\bar{q}_{{}_J})|_{Avg}^2\non\\
&\sim&{g_s^2 \over256 \pi^3 {\cal V}^2 m_{\frac{3}{2}}^3 }\left[-
\tilde{f}^2{\cal V}^{-5} m_{\frac{3}{2}}^4 {\cal V}^{\frac{8}{3}}+  \tilde{f}^2{\cal V}^{-5}{\cal V}^{\frac{8}{3}} m_{\frac{3}{2}}^4 - \tilde{f}^2{\cal V}^{-5} {\cal V}^{\frac{8}{3}}m_{\frac{3}{2}}^4\right] \nonumber\\
& & \sim { g_s^2 \over256 \pi^3 {\cal V}^2 m_{\frac{3}{2}}^3 }( \tilde{f}^2 {\cal V}^{-5}{\cal V}^{\frac{8}{3}} m_{\frac{3}{2}}^4 ) \sim O({10}^{-4}){\cal V}^{-\frac{13}{3}}m_{\frac{3}{2}}\tilde{f}^2 \ GeV  \nonumber\\
& &< 10^{-17}\tilde{f}^2 GeV < O(10^{-25}) GeV.
 \end{eqnarray}
 \vskip -0.3in
The life time of gluino is given as:
   \begin{eqnarray}
   \tau &=&\frac{\hbar}{\Gamma}\sim\frac{10^{-34} Jsec}{10^{-17}f^2 GeV}\sim\frac{10^{-7}}{f^2}> 10^{3}sec.
   \end{eqnarray}
\begin{figure}
\begin{center}
\begin{picture}(1000,170)(50,0)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\Text(140,135)[]{$\tilde{g}$}
%\ArrowLine(110,120)(160,120)
\Line(110,120)(160,120)
\Vertex(160,120){3.5}
\Gluon(110,120)(160,120){5}{4}
\DashArrowLine (160,120)(190,150){4}
\Text(180,152)[]{$\tilde{q}_L$}
\ArrowLine(190,90)(160,120)
\Text(170,100)[]{${q_I}$}
\ArrowLine(190,150)(190,90)
\Vertex(190,90){3.5}
\Gluon(190,90)(230,90){5}{4}
\Text(240,90)[]{$g_\mu$}
\Vertex(190,148){3.5}
\Line(190,150)(230,150)
\Line(190,146)(230,146)
\Text(235,150)[]{$\psi_\mu$}
\Text(180,40)[]{(a)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\ArrowLine(110,120)(160,120)
\Line(310,120)(360,120)
\Vertex(360,120){3.5}
\Gluon(310,120)(360,120){5}{4}
\Text(340,135)[]{$\tilde{g}$}
\ArrowLine (360,120)(390,150)
\Text(380,152)[]{$q_I$}
\DashArrowLine (390,90)(360,120){4}
\Text(370,100)[]{$\tilde{q}_L$}
\DashArrowLine (390,150)(390,90){4}
\Vertex(390,90){3.5}
\Gluon(390,90)(430,90){5}{4}
\Text(440,90)[]{$g_\mu$}
\Vertex(390,148){3.5}
\Line(390,150)(430,150)
\Line(390,146)(430,146)
\Text(440,150)[]{$\psi_\mu$}
\Text(380,40)[]{(b)}
\end{picture}
 \end{center}
 \vskip -0.7in
\caption{One-loop gluino decay into goldstino and gluon}
\label{fig:treedecgold}
\end{figure}
   \underline{${\bf \tilde{g}\rightarrow g_\mu \ \tilde{G}}$}
   
The matrix element for two-body decay of the gluino into a goldstino and a gluon (see Figure~\ref{fig:treedecgold}) is given as:
\begin{eqnarray}
\label{eq:MGold_I}
& & {\cal M}\sim {\tilde{f}}^2\int\frac{d^4k}{\left(2\pi\right)^4} \times{\cal V}^{-\frac{4}{5}}\left(\frac{i{\bar\sigma}\cdot k}{k^2-m_q^2+i\epsilon}\right)\left({\cal V}^{-\frac{15}{9}}\right)\left(\frac{i}{\left[\left(k-p_{\tilde{G}}\right)^2-m^2_{\tilde{q}}+i\epsilon\right]}
\right)\nonumber\\
& & \times\left({\cal V}^{\frac{53}{45}}\epsilon\cdot\left(2k-p_{\tilde{G}}-p_{\tilde{g}}\right)\right)\left(\frac{i}
{\left[\left(k-p_{\tilde{g}}\right)^2-m^2_{\tilde{q}}+i\epsilon\right]}\right) +\nonumber\\
& &{\tilde{f}}\int\frac{d^4k}{\left(2\pi\right)^4} \times{\cal V}^{-\frac{4}{5}}\left(\frac{i}
{\left[\left(k+p_{\tilde{G}}\right)^2-m^2_{\tilde{q}}+i\epsilon\right]}\right)\left({\cal V}^{-\frac{15}{9}}\right)\left( {\bar\sigma}\cdot\epsilon\right)\nonumber\\
& & \times\left(\frac{i{\bar\sigma}\cdot\left(k-p_{g_\mu}\right)}{\left[
\left(k-p_{g_\mu}\right)^2-m^2_q+i\epsilon\right]}\right).
\end{eqnarray}
As discussed in \cite{Dhuria+Misra_mu_Split_SUSY}, the Wilson coefficients corresponding to gluino-goldstino- gluon coupling do not change much upon RG evolution to EW scale. Going through an analysis similar to the ${\tilde g} \rightarrow \tilde{\chi}_3^0  g$, it was shown in \cite{gravitino_DM}:
\begin{eqnarray}
\label{eq:spinavGammaGold}
& &  \sum_{\tilde{g}\ {\rm and}\ \tilde{G}\ {\rm spins}}|{\cal M}|^2
\sim   Tr\biggl(\sigma\cdot p_{\tilde{G}}\Bigl[A_2{\bar\sigma}\cdot\epsilon + B_3{\bar\sigma}\cdot p_{\tilde{g}}{\bar\sigma}\cdot\epsilon + D_2{\bar\sigma}\cdot p_{\tilde{g}}{\bar\sigma}\cdot\epsilon{\bar\sigma}\cdot p_{\tilde{G}} \nonumber\\
& & + D_4{\bar\sigma}_\mu{\bar\sigma}\cdot\epsilon{\bar\sigma}^\mu C^{(b)}_{24}\Bigr] \nonumber\\
&& {\hskip -0.2in}  \times\sigma\cdot p_{\tilde{g}}\left[A_2{\bar\sigma}\cdot\epsilon + B_3{\bar\sigma}\cdot p_{\tilde{g}}{\bar\sigma}\cdot\epsilon + D_2{\bar\sigma}\cdot p_{\tilde{g}}{\bar\sigma}\cdot\epsilon{\bar\sigma}\cdot p_{\tilde{G}} + D_4{\bar\sigma}_\mu{\bar\sigma}\cdot\epsilon{\bar\sigma}^\mu C^{(b)}_{24}\right]^\dagger\biggr),
\end{eqnarray}
where  $A_2\equiv  {10}^{-6} {\tilde f}^2 $, $B_3\equiv ({10}^{-23} {\tilde f}) {GeV}^{-1}$, $D_2\equiv  ({10}^{-34} {\tilde f}) {GeV}^{-2}$, $D_4 \equiv {\cal V}^{-2.4} {\tilde f}.$
At $p^0_{\tilde{G}}=m_{\tilde{g}}/2,p^1_{\tilde{G}}=p^2_{\tilde{G}}=p^3_{\tilde{G}}=\frac{m_{\tilde{g}}}{2\sqrt{3}}$, the matrix amplitude squared becomes:
\begin{equation}
\label{eq:spinavgammaGold II}
 {m^{2}_{\tilde{g}}}\left[{D_2}^2 {m^{4}_{\tilde{g}}}+\frac{1}{6} \left(6 {A_2}+12{D_4}
   {C_{24}^{(b)}}+{m_{\tilde{g}}} \left(6 {B_3}+\left(3+\sqrt{3}\right) {D_2} {m_{\tilde{g}}}\right)\right)^2\right]\sim  \tilde{f}^4 {A_2}^2 {m^{2}_{\tilde{g}}}.
\end{equation}
So, using results from \cite{Griffiths_particle}, the decay width comes out to be equal to:
\begin{equation}
\label{eq:GammaGold}
\Gamma=\frac{ \sum_{\tilde{g}\ {\rm and}\ \tilde{G}\ {\rm spins}}|{\cal M}|^2}{16\pi\hbar m_{\tilde{g}}}\sim O({10}^{-1}) {A^{2}_2} {m_{\tilde{g}}} \sim {10}^{-2}\tilde{f}^4 \ GeV.
\end{equation}
Considering value of $\tilde{f}^2 \sim{10}^{-10}$, $\Gamma < {10}^{-22}$ GeV.  Life time of gluino is given as:
   \begin{eqnarray}
   \tau &=&\frac{\hbar}{\Gamma}\sim\frac{10^{-34} Jsec}{10^{-2}{\tilde f}^4 \ GeV}\sim\frac{10^{-21}}{{\tilde f}^4} sec > {10^{-1}}sec.
   \end{eqnarray}
   %\end{enumerate}
\section{Results and Discussion}
We have studied in detail the possibility of generating $\mu$-split SUSY scenario in the context of local type IIB Swiss-cheese orientifold (involving isometric holomorphic involution) compactifications in the L(arge) V(olume) S(cenarios). After giving details of the geometric framework, we showed the possibility of obtaining a local positive semi-definite potential for specific choice of values of VEV of position as well as Wilson line moduli and bulk moduli.  Using the modified  ${\cal N} = 1$ chiral co-ordinates due to presence of D3- and D7-branes, we constructed the form of K\"{a}hler potential and superpotential relevant to describe the phenomenological results. By evaluating all possible effective Yukawa couplings in the context of ${\cal N} = 1$ gauged supergravity, and thereafter showing that effective Yukawas change only by ${\cal O}(1)$ under RG flow evolution from string scale down to electroweak scale, we realized that Dirac mass term corresponding to fermionic superpartners of two (${\cal A}_1$ and ${\cal A}_3$) of the aforementioned four-Wilson line moduli, matched very well with the order of Dirac mass of the electron, and the Dirac mass term corresponding to fermionic superpartners of the remaining two (${\cal A}_2$ and ${\cal A}_4$) of the aforementioned four-Wilson line moduli, matched very well with the order of Dirac masses of the first generation SM-like quarks. Therefore, the fermionic superpartners of ${\cal A}_1$ and ${\cal A}_3$ could be identified, respectively with $e_L$ and $e_R$, and the fermionic superpartners of ${\cal A}_2$ and ${\cal A}_4$ could be identified, respectively with the first generation quarks: $u/d_L$ and $u/d_R$. After evaluating soft SUSY breaking parameters, Wilson line moduli masses (identified with sfermions) turned out to be very heavy at string scale.  Based on the arguments given in \cite{Sparticles_Misra_Shukla}, according to which there was an ${\cal O}(1)$ change in the value of Wilson line modulus mass under an RG flow from string scale down to EW scale, we assumed that squark/slepton masses will remain heavy at EW scale too. The highlights of this chapter are:
\begin{enumerate}
\item
By evaluating Higgs mass matrix at electroweak scale, we showed the possibility of obtaining one light Higgs of order 125 GeV at EW scale while masses of another Higgs as well as higgsino mass parameter to be very large; the primary indication of $\mu$-split SUSY.
\item
By evaluating relevant interaction vertices using ${\cal N}=1$ gauged supergravity action, we estimated life time of gluino to be very high- thus providing another concrete signature of $\mu$-split SUSY.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%The limits of integration in (\ref{eq:neutralinowidth}) are
%\begin{eqnarray}
%%\hspace{-.3cm}s_{13}^{max}(s_{23})\!\! &=&\!\! m_{q_{{}_I}}^2 + \mchi^2 +{1\over2
%  s_{23}}\left[(\mgss^2-m_{q_{{}_I}}^2-s_{23})(s_{23}-m_{q_{{}_J}}^2+\mchi^2)
 % +\lambda^{1/2}(s_{23},\mgss^2,m_{q_{{}_I}}^2)\ \lambda^{1/2}(s_{23},m_{q_{{}_J}}^2,\mchi^2)\right]\nonumber \\
%\hspace{-.3cm}s_{13}^{min}(s_{23})\!\! &=&\!\! m_{q_{{}_I}}^2 + \mchi^2 +{1\over2
%  s_{23}}\left[(\mgss^2-m_{q_{{}_I}}^2-s_{23})(s_{23}-m_{{q_{{}_J}}}^2+\mchi^2)
 % -\lambda^{1/2}(s_{23},\mgss^2,m_{q_{{}_I}}^2)\ \lambda^{1/2}(s_{23},m_{q_{{}_J}}^2,\mchi^2)\right] \nonumber\\
%\hspace{-.3cm}s_{23}^{max}\ \ \  &=& (\mgss - m_{q_{{}_I}})^2\nonumber  \\
%\hspace{-.3cm}s_{23}^{min}\ \ \  &=& (\mchi + m_{q_{{}_J}})^2
%\end{eqnarray}
%where   $\ \lambda(x,y,z)=x^2+y^2+z^2-2 xy-2xz -2yz $ and the
%kinematical variables are $s_{13}=(k_1+k_3)^2$ and $s_{23}=(k_2+k_3)^2$.
%Limits of integration as given in \cite{Dhuria+Misra_mu_Split SUSY} are:
%\begin{eqnarray}
%&& s_{23 \max }\sim {\cal V}^{\frac{4}{3}}m^{2}_{\frac{3}{2}},\ s_{23 \min }\sim {\cal V}^{\frac{4}{3}}m^{2}_{\frac{3}{2}}+ \frac{m_{\tilde g} {\tilde f}^2  v^2 {\cal V}^{\frac{2}{3}}}{m_{pl}},\nonumber\\
%&& s_{13 \max}= {\cal V}^{\frac{4}{3}}m_{\frac{3}{2}}^2-s_{23}, s_{13 \min }=  ,
%\end{eqnarray}
%v is Higgs VEV at electroweak scale.
 

==> abstract.tex <==
%Satyam Shivam Sundaram
%Jai Mata Di
%\chapter*{Abstract}
%\newpage
 \chapter*{abstract}
The first part of the thesis is devoted to investigation of important phenomenological and particle-cosmology-related issues in the context of Type IIB string compactifications. 
%We begin by motivating split supersymmetry from points of view of particle as well as string phenomenology.
After undertaking a brief review of (split) supersymmetry in the context of Beyond Standard Model Physics, we discuss the possibility of realizing ``$\mu$-split SUSY" scenario from a phenomenological model, which we show could be realizable locally as the large volume limit of a type IIB Swiss-Cheese Calabi-Yau orientifold involving a mobile space-time filling D3-brane localized at a nearly special Lagrangian three-cycle embedded in the "big" divisor (hence the local nature of the model's realization) and multiple fluxed stacks of  space-time filling D7-branes wrapping the same ``big" divisor. Naturally realizing split-SUSY scenario of N. Arkani-Hamed and S. Dimopoulos in our model, we show that the mass of one of the Higgs formed by a linear combination of two Higgs doublets (related to the D3-brane position moduli), can be produced to be of the order of 125 GeV whereas other Higgs as well as higgsino mass parameter to be very heavy- the ``$\mu$-split SUSY" scenario. The squarks'/sleptons' (the Wilson line moduli on D7-branes' world volume) masses also turn out to be very heavy.  Motivated by the fact that the gravitino appears as the Lightest Supersymmetric Particle (LSP) in our model, we explore the possibility of the gravitino as a viable cold dark matter candidate by showing its life time to be of the order of or greater than the age of the universe whereas lifetimes of decays of the co-NLSPs (the first generation squark/slepton and the lightest neutralino) to the LSP (the gravitino) turns out to be too short to disturb predictions of Big Bang Nucleosynthesis (BBN). Assuming non-thermal gravitino production mechanism,
we estimate the gravitino relic abundance to be around $0.1$ by evaluating the neutralino/slepton
annihilation cross sections and hence show that the former satisfies the requirement for a dark
matter candidate.  As another testing ground for split-SUSY scenarios, we estimate Electric Dipole Moment (EDM) of electron/neutron up to two-loops in our model. By explaining distinct ${\cal O}(1)$ CP violating phases associated with Wilson line moduli and position moduli, we show that it is possible to obtain dominant contribution of EDM of electron/neutron to be around $10^{-29}$ esu-cm at two-loop level by including heavy sfermions and a light Higgs, around $10^{-27}$ esu-cm for a two-loop Barr-Zee diagram involving W boson and SM interaction vertices, eEDM  to be around $10^{-33}$ esu-cm at one-loop by including heavy chargino and a light Higgs, and nEDM  to be around $10^{-32}$  esu-cm at one-loop by including  SM fermions and a light Higgs.  

In second part of the thesis, we obtain local M-theory uplift of Type IIB background involving non-compact (resolved) warped deformed conifold and (N) space time filling D3-branes placed on the singularity of the conifold, (M) D5-branes wrapped around compact $S^2$, and ($N_{f}$) D7-branes wrapped around non-compact four-cycle via Strominger-Yau-Zaslow's mirror symmetry prescription \cite{SYZ3_Ts}. This work is mainly concerned with the investigation of hydro/thermodynamical aspects relevant to explain the behavior of thermal QCD with fundamental quarks, as well as to demonstrate the thermodynamical stability of the M-theory uplift. The uplift gives a black M3-brane solution whose near-horizon geometry near
$\theta_{1,2}=0,\pi$-branches, preserves $1/8$ SUSY. We propose a new MQGP limit corresponding to finite-string-coupling ($g_s \lesssim 1$)- large-t'Hooft-coupling regime of M-theory in addition to the one discussed in \cite{metrics}. Interestingly, we obtain $\eta/s=1/4 \pi$ for the uplift and the diffusion constant $ D \sim1/T$ for types IIB/IIA backgrounds in the both limits. The thermodynamical stability of M-theory uplift is checked by evaluating the D = 11 Euclideanized supergravity action upto $O(R^4,|G_4|^2)$  term in the two limits, and thereafter showing the positive sign of specific heat from the finite part of the action.
 

 
 



==> empty.tex <==
\newpage
~\\
~\\

\thispagestyle{empty}
%\cleardoublepage
\addtocounter{page}{-1}

